The XMM Cluster Survey: Automating the estimation of hydrostatic mass for large samples of galaxy clusters I -- Methodology, Validation, & Application to the SDSSRM-XCS sample

We describe features of the X-ray: Generate and Analyse (XGA) open-source software package that have been developed to facilitate automated hydrostatic mass ($M_{\rm hydro}$) measurements from XMM X-ray observations of clusters of galaxies. This includes describing how XGA measures global, and radial, X-ray properties of galaxy clusters. We then demonstrate the reliability of XGA by comparing simple X-ray properties, namely the X-ray temperature and gas mass, with published values presented by the XMM Cluster Survey (XCS), the Ultimate XMM eXtragaLactic survey project (XXL), and the Local Cluster Substructure Survey (LoCuSS). XGA measured values for temperature are, on average, within 1% of the values reported in the literature for each sample. XGA gas masses for XXL clusters are shown to be ${\sim}$10% lower than previous measurements (though the difference is only significant at the $\sim$1.8$\sigma$ level), LoCuSS $R_{2500}$ and $R_{500}$ gas mass re-measurements are 3% and 7% lower respectively (representing a 1.5$\sigma$ and 3.5$\sigma$ difference). Like-for-like comparisons of hydrostatic mass are made to LoCuSS results, which show that our measurements are $10{\pm}3%$ ($19{\pm}7%$) higher for $R_{2500}$ ($R_{500}$). The comparison between $R_{500}$ masses shows significant scatter. Finally, we present new $M_{\rm hydro}$ measurements for 104 clusters from the SDSS DR8 redMaPPer XCS sample (SDSSRM-XCS). Our SDSSRM-XCS hydrostatic mass measurements are in good agreement with multiple literature estimates, and represent one of the largest samples of consistently measured hydrostatic masses. We have demonstrated that XGA is a powerful tool for X-ray analysis of clusters; it will render complex-to-measure X-ray properties accessible to non-specialists.

==> OldSections/OldSections2March23/OLDSection2.tex <==

\section{XCS Data and Cluster Samples - moved}
\label{sec:samplesanddata}

This section summarises the \xmm{} data used in this work, as well as the three samples of galaxy clusters.

\subsection{XCS cleaned data and source regions}
\label{subsec:xcsdata}
All XCS 
%comment: should this say XGA? from PG
X-ray measurements presented in this work are based on cleaned event lists produced during the XCS analysis of the \xmm{}-Newton public archive, fully described in \cite{xcsmethod}. Briefly, the initial EPIC data were processed with v14.0.0 of the \xmm{} Science Analysis Software (SAS), using EMCHAIN and EPCHAIN to generate event lists. Following this, event lists were screened for periods of high background and particle noise by generating light curves in 50s time bins for the soft (0.1–1.0~keV) and hard (12–15~keV) bands. An iterative 3$\sigma$ clipping process was then performed on the light curves; time bins falling outside this range were excluded. XCS do not currently make use of \xmm{} Reflection Grating Spectrometer (RGS) or Optical Monitor (OM) data.

Source detection is performed using a custom version of {\sc wavdetect} \citep[][]{wavdetect} called XCS Automated Pipeline Algorithm (\xapa{}). \xapa{} is run on merged EPIC (PN+MOS1+MOS2) images, with a pixel size of 4.35\arcsec, generated using events within an energy range of 0.5-2.0~keV. Once sources in an image have been located, \xapa{} then classifies them as either point or extended sources. Region lists of sources are created for each individual \xmm{} observation. Note that although the cleaned events lists were produced with SAS v14.0.0, as were the images upon which \xapa{} is run, the analyses described in this paper are based on \xmm{} products generated using SAS {\color{red} v18.0.0}.

% Finally, making sure to remove duplicate objects from parts of the sky that have been imaged multiple times by \xmm{}, the detected sources are compiled into the XCS master source list (hereafter called the MSL).
% As of {\color{red} late 2020} the XCS MSL contains 372,205 objects, with XAPA classifying 39,890 of those objects as extended sources, and 332,315 as point sources. As a galaxy cluster survey we focus mostly on the extended sources, though not all extended sources detected by XCS will be galaxy clusters. 
%comment: It's an important part of XCS, but seeing as I don't actually use the MSL in this work (just region lists), maybe not worth mentioning? from DG


\subsection{SDSSRM-XCS$_{T_{\rm{X}},\rm{vol}}$}
\label{subsec:sdssrmxcs}

The first sample used in this work is a set of optically selected galaxy clusters with available {\em XMM} data, recently described in \cite{xcsgiles}. The sample was constructed by selecting clusters from the redMaPPer analysis of Sloan Digital Sky Survey (SDSS) observations \citep[][]{redmappersdss}. The final sample is made up of clusters within $0.1<z<0.35$ (approximately the volume limited redshift range of redMaPPer used with SDSS data), and a fractional {\em XMM} X-ray temperature error of less than 25\%. This results in a sample of 150 galaxy clusters. The sample we use in this work is referred to as SDSSRM-XCS$_{T_{\rm{X}},\rm{vol}}$ in \cite{xcsgiles}, but for simplicity we refer to it simply as the SDSSRM-XCS sample.

\subsection{XXL-100-GC}
\label{subsec:xxl100gc}

The second set of clusters we utilise is the XXL-100-GC sample \citep[][]{gc100}, a sub-sample of the 100 brightest galaxy clusters detected within the XXL survey \citep[][]{xxl1}.  The sample is selected by setting a lower limit of $3\times10^{-14}~\rm{erg \:s^{-1} \:cm^{-2}}$ on the X-ray flux measured within a $1'$ aperture. The XXL survey is a large-scale \xmm{} survey that observed two contiguous regions of the sky, totalling ${\sim}50$ square degrees, made up of 542 \xmm{} observations. The XXL-100-GC sample has been used in several XXL analyses, including mass-temperature relations \citep[][]{xxlmt}, and measurements of gas masses \citep[][]{xxlbaryon}.

\subsection{LoCuSS High-$L_{\rm{X}}$}
\label{subsec:locusshighlx}

The final sample we use is the Local Cluster Substructure Survey (LoCuSS) High-$L_{\rm{X}}$, 
%comment: is high Lx needed? Sort of feels misplaced. PG
50 X-ray selected galaxy clusters from the {\em ROSAT} all sky survey (RASS) catalogues.  ICM properties have been measured using a mix of \xmm{} and \chandra{} observations, and taken from a combination of the analysis presented in \cite{locusshydro} and \cite{locusstemps}. At the time of the \cite{locusshydro} analysis, 43 of the clusters had been observed by \chandra{} and 39 by \xmm{}, with 27 of the clusters having data from both telescopes. All comparisons in this work are performed on \xmm{} measured values, to avoid the known temperature discrepancy between \xmm{} and \chandra{} analyses \citep[e.g.,][]{schellenbergertcal}. 

%So I've commented this out as I don't think it's needed (PAUL).
%This set of galaxy clusters does not extend to the low temperatures explored by the other samples we intend to analyse, as can be seen in Figure~\ref{fig:samp_sum}a. As they were specifically selected for their high X-ray luminosities this is to be expected, but means that our comparison of masses does not extend to the low-mass regime.

%comment: Should we say all this?  A referee might say while surely you can cobble together a load of low mass clusters to make a comparison.  They might say that anyway, but let's not give them the idea. PG

\subsection{Comparison of samples}
\label{subsec:compsamp}

Summary information for these samples is presented in Table~\ref{tab:samplesummary}.  Comparisons of the distributions of the X-ray temperature ($T_{X}$), redshift and X-ray luminosity ($L_{X}$) for the samples are shown in Figures~\ref{fig:samp_sum}a), b) and c) respectively.  The temperature distribution shows the XXL-100-GC mostly contains clusters below 6~keV, the SDSSRM-XCS peaks at a similar temperature to XXL-100-GC but extends to higher temperatures, and the LoCuSS High-$L_{\rm{X}}$ sample contains higher temperature clusters (similar to the tail of the SDSSRM-XCS distribution) due to its selection from highly luminous systems.  The redshift distribution for the XXL-100-GC sample contains higher redshift clusters than the other samples, however, the SDSSRM-XCS and LoCuSS High-$L_{\rm{X}}$ samples includes redshift cuts, introducing artificial limits. Finally, the luminosity distributions highlights that the XXL-100-GC is similar to the lower end of the SDSSRM-XCS distribution, whereas the LoCuSS High-$L_{\rm{X}}$ sample is similar to the high luminosity tail of SDSSRM-XCS. 

% {\color{red} I USE XGA FOR THIS SO SHOULD IT BE HERE? - A search through the \xmm{} science archive shows that {\color{red} 46} of the LoCuSS High-L$_{\rm{x}}$ clusters have now been observed by \xmm{}}. As we will not use \chandra{} data in this work we do not perform the same check through the \chandra{} archive.

% The full LoCuSS sample of 165 clusters was derived from the RASS catalogues by applying the cuts to various values; 0.15 < $z$ < 0.3, $n_{H}$ < $7\times 10^{20}\rm{cm}^{-2}$, and $-70^{\circ}$ < $\delta$ < $70^{\circ}$. The High-$L_{\rm{x}}$ sample was then selected from this larger sample by a harsher cut on the allowed declination values ($-25^{\circ}$ < $\delta$ < $65^{\circ}$), and a cut on the cluster luminosities measured within the $0.1-2.4$keV band ($L_{\rm{X}}$E($z$)$^{-2.7}$ $\geq$ $4.2\times10^{44}\rm{erg\:s^{-1}}$).

%comment:no segue KR


==> OldSections/OldSections2March23/OLDSection3.tex <==

\section{The X-ray: Generate and Analyse software package - moved}
%this section is to explain why XGA is needed, to compare/contrast with XCS3P, and to give technical details that are not in the XGA paper
\label{sec:xga}

In this section we provide a brief overview of the basics of X-ray Generate and Analysis \citep[\xga\footnote{\href{https://github.com/DavidT3/XGA}{X-ray: Generate and Analyse GitHub}};][]{xgapaper}, including source matching, generation of images, generation of masks to remove contaminating sources, and the measurement of galaxy cluster temperatures and luminosities. Using the samples described in Section~\ref{sec:samplesanddata}, we show that \xga{} produces simple X-ray observables (e.g., \tx{} and \lx{}) consistent with previous measurements.  Additional comparisons are made in Section~\ref{sec:radxga} \xga{} related to the measurement of gas density and temperature radial profiles, where we detail the \xga{} process of determining hydrostatic masses. All  analyses performed in this work used \xga{} {\color{red} v0.4.1, \texttt{SAS} v18.0.0, {\sc Xspec} v12.11}.

%comment: NOT OUT YET BUT WILL BE THE VERSION I RELEASE WITH THIS WORK I SUSPECT | Double check all of these before actually making public | DT

\subsection{Summary of \xga{} - moved}
\label{subsec:xgaintro}

%comment: not sure this should be a sub-section, but could be shorted a bit and be in the 3.0 part before each subsection is described. Something we need to be careful of is avoiding repetition with the XGA paper. And if something is in here that is not in there, we need to explain why. make it clearer that the XGA paper does not have any technical details, but can mention there is a useful flow chart KR

\xga{} is an open-source Python module developed by XCS, and recently described in \cite{xgapaper}. It is a generalised X-ray analysis tool, capable of investigating any X-ray source that has been observed by \xmm{}, with different analyses implemented for specific types of astrophysical source. 

%comment: Avoid double footnote, looks weird in pdf PG

%\footnote{\href{http://xga.readthedocs.io/}{X-ray: Generate and Analyse Documentation}}

%comment: Considering we give the citation to the paper, which contains links to the documentation, I don't think this footnote is needed. PG

\xga{} is based around the declaration of source objects, which are software proxies for actual astrophysical objects; they have physical properties associated with them, such as position, redshift, nH, luminosity, and more, dependent on the type of object they are. There are general source types for generic point and extended sources, and more specific classes for sources like galaxy clusters or stars. The type of source declared will affect what analyses can be performed, for instance attempting to measure the hydrostatic mass of an AGN source would not be allowed.

%comment: much of this [para above] feels unnecessary PG

Almost every aspect of the generation and analysis routines implemented in \xga{} are configurable by the user. This ranges from being able to define the cosmology that is used for analysis, to deciding how spectra should be binned on generation, to setting the energy range that a spectral fit should be performed in. This allows us to recreate many of the analysis choices employed by previous work, simply by changing arguments passed to \xga{} functions.

\subsection{Selecting \xmm{} data - moved}
\label{subsec:dataselect}

%comment: make sure the headings link to what is in the flow chart in the XGA paper to make it easy to cross reference KR

Once a galaxy cluster source 
% I struggle with "source" in this context. Maybe we can define a clearer technical term, e.g. \tt{source}^{XGA} KR
has been declared, valid \xmm{} observations with an aimpoint within 30\arcmin of the cluster coordinates are located; an observation is discarded if less than 70\% of the initial $R_{500}$ region 
%comment: I may have to alter this slightly for a couple of the SDSS clusters DT
falls on the detectors. The SDSSRM-XCS sample contains 99 (66\%) objects with at least one on-axis observation, the XXL-100-GC sample contains 33 (34\%; lower because of the contiguous survey nature of XXL), and LoCuSS High-$L_{\rm{X}}$ 43 (96\%).  All observations were inspected for flaring that were not removed through cleaning, as well as for other data problems;
%comment: Is this an important point that needs to be defined? PG
we found and rejected 47 such observations.
%comment: Add link to the notes in the GitHub I think? PG
Our final analysis of the three samples makes use of ${\sim}400$ unique \xmm{} observations.
%comment: Link to the ObsID file in the GitHub repo


%During the source setup process an nH value for the cluster coordinates is found from the full-sky HI survey by the \cite{nh} using the HEASoft \texttt{nh} command, the chosen cosmology is used to make sure analysis radii (such as $R_{500}$) are available in kpc and degrees, then image World Coordinate System (WCS) information is used to make radii available in pixel units.
%comment: I've removed this for now as I don't think it is needed. PG

% {\color{red} Data from all scientific observation modes\footnote{\href{https://xmm-tools.cosmos.esa.int/external/xmm_user_support/documentation/dfhb/node71.html}{XMM-Newton Observation Modes}} are used, including small window data - DON'T KNOW IF THIS WILL REMAIN TRUE, I SHOULD ADD AN OPTION TO TURN IT OFF}.

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\columnwidth]{images/SDSSXCS-408-rt.png}
%    \caption[]{An \xmm{} 0.5-2.0~keV stacked ratemap of the galaxy cluster A1413 (contained in the SDSSRM-XCS sample). A mask to remove contaminating 
%comment: I'd like there to be a blow up of one part in the corner, to demonstrate that region outlines don't overlap between obsids KR
%sources has been applied. Masks are built from sources identified by {\sc xapa}, with point sources highlighted by red sources and extended sources given by green ellipses.  The appearance of overlapping regions highlights that the mask is composed of all regions identified in all observations available for a cluster.  The solid line cross-hair indicates the X-ray peak measured by \xga{}, the dashed line cross-hair indicates the original input coordinate. 
%comment: Is this really needed?  It's very hard to see the different between the two crosshairs. PG
%Solid circle indicates the input $R_{500}$ from \cite{xcsgiles}, with the dashed annulus indicating the background region.}
%    \label{fig:immask}
%\end{figure}

%\begin{figure}
%comment: not sure I'll keep it DT | don't think we need it KR | how about appendix? PG
%    \centering
%    \includegraphics[width=1.0\columnwidth]{images/region_editor.jpg}
%    \caption[]{An example of an \xga{} region editor window, taken from an \href{https://github.com/DavidT3/XCS-Mass-Paper-I/blob/main/images/region_editor.gif}{animated example} of the manual adjustment process for SDSSRM-103. A manual region (in white) is being added to account for a bright poorly removed point source which is exhibiting strong PSF spoking. {\color{red} preliminary}}
%    \label{fig:regeditor}
%\end{figure}

%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/sdssxcs_Tx_Lxb_Lx52_comp.pdf}
%    \caption[XCS3P vs XGA 500]{Comparisons between results measured using the existing XCS pipeline, and those measured using the new \xga{} package. a) The \xga{} APEC temperatures versus the \texttt{XCS3P} APEC temperatures within $R_{500}$ for the SDSSRM-XCS sample, a clear 1:1 relation with a small amount of scatter is evident, as would be expected in this case. b) Shows the equivalent comparison for the 0.5-2.0~keV X-ray luminosity measured within $R_{500}$, with a similarly tight relation between the two measurements. c) Shows the comparison for the bolometric X-ray luminosity measured within $R_{500}$, and is very similar to the soft-band comparison.}
%    \label{fig:xcstemplumcomp}
%\end{figure*}

%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/sdssxcs_Tx_Lxb_Lx52_r2500_comp.pdf}
%    \caption[XCS3P vs XGA 2500]{Comparisons between results measured using the existing XCS pipeline, and those measured using the new \xga{} package. a) The \xga{} APEC temperatures versus the \texttt{XCS3P} APEC temperatures within $R_{2500}$for the SDSSRM-XCS sample; they agree very well with less scatter than the $R_{500}$ comparison. b) Shows the equivalent comparison for the 0.5-2.0~keV X-ray luminosity measured within $R_{2500}$, with a similarly tight relation between the two measurements. c) Shows the comparison for the bolometric X-ray luminosity measured within $R_{2500}$ which is again very similar to the soft-band.}
%    \label{fig:xcstemplumcompr2500}
%\end{figure*}

\subsection{Generating and interacting with X-ray imaging data - moved}
\label{subsec:xgaphot}

%comment: : I am not comfortable with "photometric" in this context. It might be the correct term, but since it is usually for optical images, we'd need to put in an explanation of that the first time it comes up KR
%comment:  can we just call it "X-ray imaging" data PG

In order to produce imaging data, \xga{} interfaces with the \texttt{SAS} \texttt{evselect} (used to generate images) and \texttt{eexpmap} (used to generate exposure maps) tools. Once a source (or a sample of sources) has been defined, images, exposure maps, and ratemaps (an image divided by an exposure map) in any energy range can be generated in bulk (and in parallel). By default, \xga{} uses the 0.5-2.0~keV energy band. Imaging data are loaded into instances of specific \xga{} product classes; \href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.phot.Image}{\texttt{Image}}, \href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.phot.ExpMap}{\texttt{ExpMap}}, and \href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.phot.RateMap}{\texttt{RateMap}}. \xga{}'s photometric classes provide convenience functions for viewing (e.g., Figure~\ref{fig:immask}), conversion of coordinates using WCS and extracting values at specific coordinates. In addition, \xga{} also supports creating `combined' images, exposure maps, and ratemaps, from multiple {\em XMM} observations using the \texttt{SAS} tool \texttt{emosaic}.  

\subsection{Identifying and removing contaminating sources - moved}
\label{subsec:xgacontam}

To identify which sources are contaminants and need to be removed from an observation, we must determine which source corresponds to the cluster of interest. During the setup stage of a galaxy cluster object, \xga{} searches the XCS region files for each observation to find source regions that match the cluster coordinates.
%comment: I feel as though this should go in section 3.2? PG | I think I remember flip-flopping about where to put this - I think the only reason I didn't was because I wanted to segue into the manual adjustment part, which I wanted to put after the interacting with X-ray imaging data part DT | Actually, think about it again, I think it is fine here.  We are talking about somewhat different things i.e., finding observations compared to finding sources. PG

If the input cluster coordinates fall within an extended source, it is considered a match. A cluster is considered detected if there is a match in at least one observation's region list. We then search for point regions within 0.15R$_{500}$ of the cluster coordinates, as they could be an indication of a bright cool core, and make sure that they are not removed as contaminating sources. 
%comment: Hmmm, I am not sure about this.  0.15r500 can be quite large.  I would want to double check this figure. PG
We also check for intersections between matched regions and other extended regions (from all observations) within R$_{500}$. This avoids cases where a cluster is detected in multiple observations, but the supplied coordinates do not match to regions in all of them, as \xapa{} has placed a region on a different part of the cluster. Finally, all other regions (from all observations) are designated as contaminants, and removed by masks. Figure~\ref{fig:immask} shows a stacked count-rate map generated by \xga{}, with contaminating sources masked.  Sources are identified by {\sc xapa}, with point sources highlighted by red sources and extended sources given by green ellipses.  The appearance of overlapping regions highlights that the mask is composed of all regions identified in all observations available for a cluster. 

\subsection{Manual adjustment of detection regions and inspection of data - moved}
\label{subsec:manualdetreg}

In some instances, manual adjustments to the mask regions produced by \xapa{} is required, most commonly to increase the size of a region so that contaminating emission is better removed. Poorly removed contaminant emission in either the source analysis region or background region can have a significant effect on measurements.

%particularly when the source is in the background region. As background emission is subtracted from the surface brightness profiles generated by \xga{}, and from the spectra during \texttt{XSPEC} fitting, extra emission can bias the observed emission level of the cluster significantly.
%comment:  So I have commented this out for now as not really needed. PG
Feb 9, 2023 10:30 AM

We address this by visually inspecting combined ratemaps
% Why specifically ratemaps? PG
of our galaxy cluster samples using a method in \xga{} (\texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.phot.Image.edit_regions}{edit\_regions}}) that allows us to easily interact with and modify existing regions, add new regions, adjust the scaling of the image and apply smoothing to check for sources that have been missed by \xapa{}. This is done in a graphical user interface, so the result of a new or modified region can be seen immediately. 
%comment: not needed I think PG

We overlay analysis regions on the clusters (centered on their X-ray coordinates); a circle indicating where the $R_{500}$ region lies, and an outer annulus indicating where its corresponding background region lies.
%comment:  just an outer annulus? PG
Some point source regions were adjusted so that more of their emission is removed from analysis.  In extreme cases, bright point sources introduce artefacts in the image from \xmm{}'s radial PSF spokes. Extended elliptical regions were added to remove this emission, with Figure~\ref{fig:regeditor} showing an example of this. Additionally, nearby cluster's (e.g., mergers or foreground/background clusters)
%comment: Hmmm, maybe we should discuss more.  What emission of a merger should we really exclude?  How do we determine foreground/background? PG
to the one in question had existing extended regions modified to remove more of the contaminating cluster's X-ray emission.

We modified region files for 60 (40\%) of the SDSSRM-XCS sample, 44 (44\%) of the XXL-100-GC sample, and 26 (56\%) of the LoCuSS High-$L_{\rm{X}}$ sample. 

%every cluster was inspected. The process took approximately three hours for all clusters.
%comment:  Great.  But i don't think it's needed :)

% , the effects of which can be seen in figure \ref{fig:badinterloper}.

% Optionally, XGA can be supplied with region files for the available cleaned data; we use the region files generated by XAPA, which not only detail positions of sources, but also their extent, and whether XAPA considers them to be point or extended sources. Once a set of observations for a given source has been selected, we attempt to match the user-provided coordinates to an entry in the region file of each; matching to extended regions for objects like galaxy clusters, or point regions for objects such as AGN. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{images/chopped_cluster.png}
%     \caption{A cluster with an invalid interloper extended source in the R$_{500}$ region. The crosshair indicates the user supplied coordinates, a mask that removes any data outside the R$_{500}$ region, as well as interloper sources, has been applied. The large extended region next to the crosshair that has been masked out is due an off-axis observation of this cluster causing XAPA to only enclose part of the emission for that observation. - {\color{red} placeholder until I make a better figure.}}
%     \label{fig:badinterloper}
% \end{figure}

% Again we apply further selection criteria in the case of galaxy clusters, to account for common issues that can arise with region selection.  This can happen when a cluster lies at the centre of one observation and on the outskirts of another.

%\begin{figure*}
%    \centering
 %   \includegraphics[width=1.0\textwidth]{images/xxl_Tx_Lx52_comp.pdf}
%    \caption[]{A comparison of global X-ray values measured by \xga{} and XXL analyses, for the XXL-100-GC sample. a) Shows the temperature values measured within the 300kpc, and b) shows the equivalent for the 0.5-2.0keV luminosity measurements.}
 %   \label{fig:xxltxlxcomp}
%\end{figure*}

\subsection{Generating and fitting spectra - moved}
\label{subsec:xgaspecs}
%comment: Maybe rewrite to highlight how configurable it all is, wrt spectral binning, start parameters etc DT

We use \xga{} to measure global
%comment: Don't know if I like this word for that DT
properties (\tx{} and \lx{}) of the galaxy clusters in the samples introduced in Section~\ref{sec:samplesanddata}. Spectra are extracted within analysis regions specific to each literature sample, as the original works measured properties within different apertures; 
%comment:  Do I talk about the parallelism here?
apertures are defined in the relevant subsection (Sections~\ref{subsubsec:xcs3plt}, \ref{subsubsec:xxllt}, \ref{subsubsec:locusslt}). Background spectra are extracted in annuli outside of the analysis region, with the inner and outer radii of a background spectrum dependent on the analysis aperture (see specific sample analysis sections). For example, the solid white circle centered on the cross-hairs in Figure~\ref{fig:immask} shows the $R_{500}$ measured by \cite{xcsgiles} for the cluster in question.  The dashed white circles indicate the corresponding background annulus. All spectra are centered on their literature X-ray coordinates. Spectra for each camera of each observation of a given galaxy cluster are generated.  \xga{} uses the \texttt{SAS} \texttt{evselect} tool to create the initial spectra, and then \texttt{specgroup} to re-bin each spectrum so that there are at least five counts per channel.

Once \xga{} has generated a set of spectra of a particular galaxy cluster, we use the \xga{} \texttt{XSPEC} \citep[][]{xspec} interface to fit an emission model.  We fit absorbed \cite[with \texttt{tbabs},][]{tbabs} plasma emission models \citep[APEC,][]{apec} to the spectra. 

There are multiple stages to the fitting process. Initially, we reject any spectra that have fewer than 10 noticed channels. Next, each spectrum is fitted individually following the procedure above. If the measured temperature for a spectrum is $0.01~{\rm keV} \leq T_{\rm{X}} < \: $20~keV, or if the temperature uncertainty is greater than 15~keV, that spectrum is excluded from further analysis. Finally, we simultaneously fit the remaining spectra using a \texttt{constant*tbabs*apec} model.  The $T_{\rm{X}}$ and normalisation parameters of \texttt{apec} 
%comment: other models available KR
are tied across all spectra, the redshift is frozen at the input value, metallicity is frozen at 0.3~$Z_{\odot}$, 
%comment: This is not true for all of the analyses DT
nH is frozen
%comment: ust noticed that LoCuSS let nH vary... DT | Also, do we say yet what nH value we assume? PG | Yeah I think we have done somewhere, but probably should be here too DT
at the value determined by \xga{}, and the constant factor for each spectrum is allowed to vary to account for differences in normalisation due to effective area. Temperatures and unabsorbed luminosities 
%comment: How do you determine Lx e.g., using the lumin command? PG | Using lumin yes DT
are determined from this simultaneous fit. For all fits, $T_{\rm{X}}$ is initially set to 3~keV, the normalisation is initially set to 1~cm$^{-5}$, and the constant is initially set to 1. 
%comment: Check the original works for start parameters - though I think I did and found nothing DT |  Yeah they aren't there DT | Also, this bit should be moved up a bit. PG
All fits use the \texttt{angr} abundance table \citep[][]{andgrev}.
%comment: Check the original works for abundance tables DT | XXL does use Anders and Grevasse DT | LoCuSS Martino doesn't seem to say DT

The fits 
%comment: in what ways does the method deviate from Giles? Anything that is similar can be cut down to a reference KR
are performed using the $c$-statistic \citep[][]{cash}. Each \texttt{XSPEC} operation (i.e. a fit to global spectra for a cluster) will time out if it has not been successful within 4 hours. 
%comment: need more info about this KR |  is it CPU or ellapsed? KR | why 4 hours? how often does it happen? what happens next to remedy the situation? KR

%  Previous work by XCS ({\color{red} le references}) has measured these values using a luminosity-temperature (hereafter referred to as L-T) pipeline that iteratively generates spectra, fits them, measures temperature and luminosity, then uses that temperature to estimate R$_{500}$, and repeat until the results converge. The results presented in this work do not use the existing XCS pipeline, but rather use an equivalent functionality that has been built into XGA. The behaviour of our new implementation is largely the same as the original L-T pipeline, though subtle differences in software version, calibration files, location of the central coordinate, and how interloper sources are handled will cause slightly different results to be measured. For this work we measure temperatures within a region of radius R$_{500}$ and centred on the X-ray peak coordinates, we also measure unabsorbed luminosities in that same region, as well as core-excised luminosities in the {\color{red} 0.15-1R$_{500}$ region, which have been shown to have smaller scatter compared to global luminosities.}

% For this work, the measurements are derived from spectra centred on the X-ray peak as measured by XGA, with the peak position/outer radius (and inner radius for core-excised luminosity) converted to XMM detector coordinates. Equivalent position information for all interloper sources is used to exclude their corresponding events, and a source spectrum (within the chosen region) is generated for each instrument of each observation associated with that source. An ARF is calculated for that spectra, though the same RMF is used for all spectra generated from a particular ObsID-Instrument combination, as there is very little spatial variance that can be attributed to an RMF, and they relatively computationally expensive to create. We also group the spectra {\color{red} talk about the grouping parameters, as well as the rest of the SAS expression I forgot}

%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/locuss_Txce_Lxbol_comp.pdf}
%    \caption{A comparison of global, core-excised, X-ray temperatures and luminosities measured by \xga{} and LoCuSS analyses, for a subset of the LoCuSS High-$L_{\rm{X}}$ sample. a) Shows the temperature values measured within the 0.15-1$R_{500}$ region, and b) shows the comparison for full $R_{500}$ bolometric luminosity measurements.}
%    \label{fig:locusstxlxcomp}
%\end{figure*}


\subsection{Comparing \xga{} \tx{} and \lx{} measurements to literature - moved}
\label{subsec:comptxlx}
%comment: Should this be a new section?  Just wondering as it's getting pretty long. PG | If so then 3.6 should be the start of the new section DT | I'm not sure, up to and including 3.6 is analysis, then 3.7 moves to comparison, so think it would still flow well.  Lets ask Kathy as well though.

Here we 
%comment: wouldn't it read better if all XGA technical stuff was in one section (inc. profile making and fitting) and all tests in another section? KR
directly compare \xga{} measurements of galaxy cluster temperature and luminosity to measurements from literature. We attempt to minimise the differences in analysis between \xga{} and each literature dataset; we use the same energy bands during \texttt{XSPEC} spectral fitting as the original analyses, equivalent analysis regions (e.g. 300~kpc aperture for XXL), and the same cosmologies.


\subsubsection{SDSSRM-XCS properties measured by \texttt{XCS3P}}
%comment: XCS3P uses all sub-exposures of an XMM observations, whereas the way we have setup XGA only uses one with the longest exposure time. Do I mention this? DT
\label{subsubsec:xcs3plt}

We first compare \xga{} SDSSRM-XCS properties to the analysis presented in \cite{xcsgiles}, who measured  temperatures and luminosities (0.5-2.0~keV and bolometric) within $R_{500}$ and $R_{2500}$ regions. The notebook we constructed to fully detail the \xga{} analysis is \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/sdss_comparisons.ipynb}{accessible here}. 

Published measurements were made using the \texttt{XCS3P} pipeline \citep[fully described in][]{xcsmethod, xcsgiles} that measures properties within the overdensity radii, found through an iterative process.  An initial temperature and luminosity are measured within the \xapa{} defined source 
%comment:  We may need to define this. PG
radius, then uses the temperature to estimate R$_{500}$ (or R$_{2500}$) using the $R_{\Delta}-T_{\rm{X}}$ relation of \cite{arnaudmt}, and repeats until the radius converges. To account for the background, local background annuli were constructed between 1.05-1.5$R_{500}$ or between 2-3$R_{2500}$.  \xga{} does not re-use any code from \texttt{XCS3P}, but the \xga{} analysis matches as close as possible that performed in \cite{xcsgiles} (e.g., the same source and background regions).
%comment: I would like there to be a similiarities and differences list here like there is for XXL and LOCUS KR | there are differences, e.g. in how the contaminating sources are masked KR | it would also highlight that the "cleaned event lists and region files" are the same KR 
%comment: Makes it sound as though you perform an iterative process.  I think this description is slightly overkill, and we just need to say we take the r500/r2500 radii from G22. PG

We find strong agreement between SDSSRM-XCS \tx{}, \lxl{}, and \lxb{} 
%comment:  Pretty sure a couple of them don't run, find out why DT
values measured by \xga{} and the \texttt{XCS3P} pipeline. Figure~\ref{fig:xcstemplumcomp} demonstrates a 1:1 relationship for all measured properties within $R_{500}$. Figure~\ref{fig:xcstemplumcompr2500} provides the same comparison, but for measurements made within $R_{2500}$. Again, there is a very tight agreement between the two sets of measurements.
This demonstrates that \xga{} produces results that are consistent with previous XCS work, and the small amount of scatter can be attributed to differences in software versions, rounding, and how \xga{} removes contaminating sources.

\subsubsection{XXL-100-GC}
\label{subsubsec:xxllt}

Next, we compare \xga{} luminosity and temperature measurements to the XXL-100-GC\footnote{\href{http://vizier.u-strasbg.fr/viz-bin/VizieR-3?-source=IX/49/xxl100gc}{XXL-100-GC baryonic properties VizieR table}} \citep[][]{gc100} 
%comment: Already referenced, can prob drop. PG
sample. The notebook we constructed to measure these quantities is \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/xxl_comparisons.ipynb}{accessible here}, and fully explains all analysis steps.

We attempt to minimise the difference between our \xga{} analysis and the XXL-100-GC analysis \citep[as presented in][]{xxllt}, but some variables are outside our control. The measurements of \cite{xxllt} are based on data products that have gone through a different cleaning process to XCS data \citep[][]{xxl1}. 
%comment: Is this the reference for cleaning XXL data? I should prob know :) PG
Not only that, a different source finder was used to identify and remove contaminating sources, and we do not replicate any potential manual exclusion of sources. 
Our measurements of the XXL-100-GC cluster sample \tx{} and \lx{} are centred on the coordinates reported by \cite{gc100} (derived from X-ray centroids), use the WMAP9 cosmological results, and use a 300~kpc aperture to be consistent with \cite{xxllt}. Attempting to make our analysis 
%comment:  in this list should be the aperture info, since that is a key feature of XGA (its adaptability to apertures). Currently buried in paragraph above KR
as consistent as possible with \cite{xxllt}, we:

\begin{enumerate}[leftmargin=*,labelindent=2pt, itemsep=0.5ex]
    \item[--] Measure properties from 300~kpc radius aperture spectra.
    \item[--] Perform \texttt{XSPEC} fits within an energy range of 0.4-7.0~keV.
    \item[--] Use the same cosmology as the original analysis.
    \item[--] Use a fixed metallicity of 0.3~$Z_{\odot}$ and the \cite{andgrev} abundance tables.
    \item[--] Fit an absorbed \texttt{APEC} model to the spectra.
    %comment: However, I used a wabs model. PG
\end{enumerate}

However, some differences between the analyses remain:
\begin{enumerate}[leftmargin=*,labelindent=2pt, itemsep=0.5ex]
    \item[--] Original work by \cite{xxllt} used \cite{xxlnh} nH measurements, \xga{} uses \cite{nh} values; they have been shown to be consistent\footnote{\label{footnote:nh}\href{https://heasarc.gsfc.nasa.gov/Tools/w3nh_comp.html}{Comparisons of nH from different analyses}}.
    %comment: weird footnote wording KR
    \item[--] Further \xmm{} observations of XXL clusters may 
    %comment: we need to say definitely if this is the case KR
    have been taken since the original analysis.
    \item[--] XXL will have different 
    %comment:  rephrase KR
    cleaned event lists and region files.
    \item[--] The background measurement technique used in the XXL analysis is significantly different to the method currently used by \xga{}. A background annulus centered on the aimpoint of the \xmm{} observation is used, with a width determined by the diameter of the analysis region of the galaxy cluster \citep[see Figure~1 of][]{xxllt}. We use a background annulus local background with width 1000-1500~kpc centered on the galaxy cluster. 
\end{enumerate}

From these spectral fits we measure $T_{\rm{X}, 300~kpc}$ and unabsorbed $L^{\rm{0.5-2.0}}_{\rm{X}, 300~kpc}$. In line with \cite{xxllt} we do not include XLSSC-504 in our analysis due its unconstrained temperature errors. Two (XLSSC-61 and XLSSC-527) of the XXL-100-GC clusters do not pass the \xga{} cleaning step where at least 70\% of the $R_{500}$ region must be present on an observation, and as such we do not measure a temperature or luminosity for those clusters. Likewise we do not measure a temperature or luminosity for XLSSC-11, as due to its very low redshift there are difficulties generating the required spectral products.
%comment: This is going to have some extra investigation because it is quite weird - it worked at one point I'm sure DT

The comparison in Figure~\ref{fig:xxltxlxcomp} demonstrates good agreement between our \xga{} based analysis, and the original XXL measurements. The temperature measurements are generally consistent with a 1:1 relation, though many have large uncertainty values. This is likely due to a combination of the difference in analysis as detailed above. 
%comment: Do I mention the short exposures of XXL as another factor here? Its sort of hard to argue in a way, as I have access to exactly the same data that Paul did, but equally maybe it could be that any poorly adjusted region has a larger impact because of the overall lack of photons? DT
The luminosity measurements of our analysis are in agreement with the XXL work, though there appears to be a slight divergence at higher luminosities. One plausible explanation is the difference in our background methods.  Since we are using a fixed background annulus there will be more cluster emission present in the background region for larger clusters, hence, more cluster emission will be removed for those systems. Luminosity depends mainly on the normalisation of the spectral fit models, and as such exhibits a stronger dependence on choice of background. 
This reanalysis of the XXL-100-GC cluster sample, and its good agreement with the original results published by \cite{xxllt}, shows that \xga{} is a reliable tool that produces measurements of global cluster quantities consistent with existing results. 

\subsubsection{LoCuSS High-$L_{\rm{X}}$}
\label{subsubsec:locusslt}

% As \cite{locusshydro} reported which \xmm{} observations were used for their measurements, we shall measure properties in two ways; a) using only those observations, in an attempt to perform an analysis as close to the original as possible, and b) using all available data.

Finally, we perform a reanalysis of the LoCuSS High-$L_{\rm{X}}$ and again directly compare \xga{} measured \tx{} and \lx{} values to those from the original analysis. The notebook we constructed to measure these quantities is \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/locuss_comparisons.ipynb}{accessible here}, and fully explains all analysis steps.

The temperatures which we compare to 
%comment: Cite private communication with Graham? DT | Do you need to, are they not published? PG
for these clusters are core-excised (measured within 0.15-1R$_{500}$), though the luminosities are not.
%comment: Strange, how come?  Just not available? PG
The $R_{500}$ values we use are those presented in \cite{locusshydro}. Comparing to core-excised temperatures allows us to demonstrate and test \xga{}'s ability to measure core-excised galaxy cluster properties. We attempt to minimise differences between analyses, but the same caveats with respect to event cleaning and source regions apply as in Section~\ref{subsubsec:xxllt}. The cluster spectra are centered on RASS positions 
%comment: I assume they are centered in X-ray positions, looking at the images they certainly seem to be DT |  Really, that seems strange. PG
reported in \cite{locusshydro}. 

We attempt to match LoCuSS analysis 
%comment: in this list should be the aperture info, since that is a key feature of XGA (its adaptability to apertures). Currently buried in paragraph above KR
choices by adjusting the settings with which we run \xga{}:
\begin{enumerate}[leftmargin=*,labelindent=2pt, itemsep=0.5ex]
    \item[--] We perform \texttt{XSPEC} fits within an energy range of 0.7-10.0~keV.
    %comment: Is that what they use?  Again, somewhat of a strange decision.  Do they not chop out energy ranges effected by fluorescence lines. PG
    \item[--] Use the same cosmology as the original analysis.
    \item[--] Metallicity is left free to vary during XSPEC fits.
\end{enumerate}

Some differences between our analysis and the original remain:
\begin{enumerate}[leftmargin=*,labelindent=2pt, itemsep=0.5ex]
    \item[--] Original work by \cite{locusshydro} used \cite{locussnh} nH measurements, \xga{} uses \cite{nh} values; they have been shown to be consistent$^\ref{footnote:nh}$.
    \item[--] The original analysis left nH free in XSPEC fits, we do not.
    %comment: Probably shouldn't say that XGA is capable of this, because then they'll wonder why I didn't do it DT | if they left it free, why do they use D&L90? was that as a starting point in the fit? KR |  I am sort of wondering why don't we just leave it free as well. PG
    \item[--] Further \xmm{} observations of LoCuSS clusters may 
    %comment: you have to be definite (not "may") KR | Will certainly be true for some clusters, PG
    have been taken since the original analysis.
    \item[--] LoCuSS will have different 
    %comment: rephrase KR
    cleaned event lists and region files.
    \item[--] \cite{locusshydro} use older models (\texttt{wabs} and \texttt{mekal}). Though we have found that temperature and luminosity results are consistent with \texttt{tbabs*apec}.
    %comment: What do we mean by this?  Have you analysed 1:1 clusters with wabs x mekal and tbabs x apec? PG
\end{enumerate}

At the time of the original analysis, 39 of the LoCuSS High-$L_{\rm{X}}$ 
%comment: What about clusters with newer additional observations. PG
clusters had an \xmm{} observation. During our analysis we found that 45 of the clusters now have \xmm{} observations, though we cannot use the new observations to provide direct comparisons to literature.
%comment: this doesn't sell the fact that we have extra data KR
 
Figures~\ref{fig:locusstxlxcomp} a) and b) highlight the comparison in temperatures and luminosities respectively, between \xga{} and LoCuSS. The comparison of core-excised temperatures demonstrates a good 1:1 agreement. The scatter is attributed to the differences in analysis techniques. Some clusters in the LoCuSS High-$L_{\rm{X}}$ sample also have had follow-up observations since the initial work by \cite{locusshydro}, which will have an effect on our results. 
%comment:  Can we not exclude this newer observations to see if the results agree better? PG
The luminosity comparison is also good, 
%comment: How can it be good and systematically offset :)
though we observe a systematic offset between original and \xga{}-measured values, with \xga{} measurements slightly lower than original LoCuSS measurements.

This comparison has further demonstrated \xga{}'s flexibility and the veracity of its global (and core-excised) luminosity and temperature measurements. The analyses and comparisons presented in Section~\ref{subsubsec:xcs3plt}, Section~\ref{subsubsec:xxllt}, and in this section have shown that \xga{} is consistent with previous work by XCS, capable of accurate fixed aperture measurements akin to those by XXL, and consistent with core-excised values as measured by LoCuSS. Additionally, we have illustrated that we can easily analyse large samples of galaxy clusters with \xga{}.

% \section{Extensions with XGA}
% \label{sec:newxgacap}

% In Section~\ref{sec:xga} we showed that \xga{} is capable of performing the same measurements as existing \texttt{XCS3P} software, and that \xga{}'s measurements are not only consistent with previous XCS work, but also with other cluster analyses from literature \citep[][]{xxllt,locusshydro}. Here, we introduce further \xga{} features that do not directly allow the measurement of hydrostatic masses, but were not present in \texttt{XCS3P}. This includes a new peak finding approach, the ability to apply PSF correction to \xmm{} images, and a simple-to-use approach to the modification of regions within an analysis.
%comment: But do not all of these features help with the hydro analysis?  Are they not centred on your peak and use the PSF correction in the gas profiles.  The manual regions I assume are used in the hydro analysis? PG | If you don't use these features, then I would move this to an Appendix. PG

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{images/pn_edgemap.png}
%     \caption{\color{red} Edge map of EPIC PN, observation 0201903501 I assume?}
%     \label{fig:pnedgemap}
% \end{figure}

%comment: This will probably be removed DT | Yeah, I would get rid of this figure. PG


% \begin{figure}
%comment: This figure should be improved DT
%     \centering
%     \includegraphics[width=1\columnwidth]{images/centre.png}
%     \caption{A demonstration of the hierarchical clustering peak finder, in a worst-case scenario where a bright point source has not been masked. Left figure indicates the X-ray peak from simply selecting the brightest pixel. Right figure shows the same cluster but with the result of the hierarchical clustering peak finder overlaid (white cross-hair) and with the point clusters overlaid (different colours, {\color{red} red} 
%comment: Change this if the colour changes in whatever updated figure you make DT
%indicates the galaxy cluster.  {\color{red} This is a bit of a naff figure} }
%     \label{fig:clusteringcentre}
% \end{figure}


% \subsection{Hierarchical clustering peak finder}
% \label{subsec:peakfinder}
%comment: Maybe should mention that the clustering criterion is another hyperparameter DT

% Finding a true central coordinate for a galaxy cluster is rarely feasible. An assumption of spherical symmetry is often made, but galaxy clusters are more often ellipsoidal, or have complex morphologies due to e.g., mergers.
% % Defining the centre of an ellipsoid which is not orthogonal or parallel to the plane it has been projected onto is not possible when you have no knowledge of the three-dimensional space.
% Different methods are used to determine a proxy for the centre of a cluster. Optical/NIR analyses often use the brightest cluster galaxy (BCG) as a proxy for the centre, but in X-ray observations the X-ray peak or centroid is used. 
%comment: This bit is a bit intro material, I would just delete. PG
%X-ray peaks have been shown to be a robust approximation of the centre of a cluster's potential well \citep[][]{sim_misscent}. In this work we generally make use of the literature coordinates, 
%comment: So if I understand, in Section 2 you have used literature RA and Dec, but for hydro analysis going forward (e.g., Sec 4) you use this peak? PG
%but for the final analysis of the SDSSRM-XCS sample in Section~\ref{sec:results} we use peak coordinates determined using our hierarchical clustering peak finder.

% Finding an X-ray peak is as simple as locating the highest valued pixel in an image. We perform peak finding on ratemaps, rather than images, to take vignetting into account; we also make sure to use combined ratemaps made up of all available \xmm{} observations, to maximise signal-to-noise.

% Peak finding can be complicated by bright pixels that aren't associated with the galaxy cluster of interest. These can be bright pixels that occur in ratemaps on the edges of \xmm{} detectors, artefacts resulting from exposure map calculations producing erroneously low values on detector edges. They can also be the remnants of poorly removed point sources, where the detection region is too small for the mask to eliminate all emission from an object (see Figure~\ref{fig:immask}). 

% We implement a new method that attempts to deal with these issues in an automated manner, it is explained in greater detail in \href{https://xga.readthedocs.io/en/latest/notebooks/techniques/hierarchical_clustering_peak_finding.html}{the \xga{} documentation}. Firstly, we use an edge detection algorithm on the {\em XMM} exposure map to find which pixels are on the edge of a detector. This is then used to generate a mask (accessible through the \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.phot.RateMap.edge_mask}{edge\_mask}} property of a \texttt{RateMap} instance) that removes any pixel on the edge of a detector; an example edge mask is shown in Figure~\ref{fig:pnedgemap}.
%comment: Remember to remove if I do remove that figure DT

% Once point sources are removed, the edge mask has been applied, and everything other than an area around the starting location of the cluster
%comment: : Do you use a starting radius e.g., within r500? PG
%has been masked out, we locate the top 5\%
%comment: Make sure that number is correct DT
%brightest pixels. A hierarchical clustering algorithm 
%comment: Does this need a reference? PG
%(using a maximum distance criterion)
%comment: Explain this and specify WHAT distance DT
%is used to group the brightest pixels into point-clusters, the largest of which is designated as the galaxy cluster. Then the pixel with the highest value in that point cluster is found, and designated as the X-ray peak.

% Figure~\ref{fig:clusteringcentre} gives an example of the results of our peak finder; on the left the brightest pixel is indicated, and on the right the pixel selected by our method. The example is in the worst case, where a bright point source was not masked.
%comment: Are you slightly misleading the truth?  I mean sure, the peak would be here, but one would at least first try and remove point sources first i.e., use our XAPA regions. PG

% This process is iterative, with the initial position set to be the literature coordinates, and the method running until the peak converges to within 15~kpc, or until 20 iterations has been reached. Figure~\ref{fig:offsets} shows the offset distributions for the three samples, where the offset is the distance (initially in pixels, converted to kpc with knowledge of the pixel degree scale, cosmology, and redshift) between the original position and the \xga{} peak.
%comment: What does said figure actually show us DT | Is this really the plot to show?  Yes, there will be an offset between the centroid and peak, but what would your peak vs other peaks be?  Maybe this isn't possible for these samples.  I would argue the plot prob isn't needed.PG

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\columnwidth]{images/samps_kpc_offset.pdf}
%     \caption{Distributions of offsets between galaxy cluster central coordinates from literature and X-ray peak coordinates measured by \xga{}.}
%comment: Maybe more detail in the caption DT
%     \label{fig:offsets}
% \end{figure}




==> OldSections/OldSections2March23/OLDSection4.tex <==

\section{Measuring gas density, temperature, and mass profiles - moved}
\label{sec:radxga}
%comment: General comment for this section - I need to discuss how errors are propagated. It's all quite simple (using posterior distributions of parameters etc), but I don't really touch on it at all DT

We wish to measure hydrostatic masses of galaxy clusters from our \xmm{} observations. The hydrostatic mass equation 
%comment:  Find something to cite, maybe the review of cluster masses from X-ray? DT Maybe somewhere with this particular version of the equation, without the dln(...)/dlnr DT
allows us to derive hydrostatic masses from knowledge of the 3D temperature and gas density profiles, 

\begin{equation}
    M(<r) = - \dfrac{k_{B}r^2}{\rho_{g}(r)\mu m_{u}G} \bigg[\rho_{g}(r)\dfrac{dT(r)}{dr} + T(r)\dfrac{d\rho_{g}(r)}{dr}\bigg],
    \label{eq:hydromass}
\end{equation}

% where $r$ is the radius within which the mass is being measured, $\rho_{g}(r)$ is the baryon mass density profile, $T(r)$ is the baryon temperature profile, {\color{red}$\mu=0.61$  is the mean molecular weight}, $m_{u}=1.66\times 10^{-24}$~g is the atomic mass unit, $G=6.67\times 10^{-11}$~m$^{3}$ kg$^{-1}$ s$^{-2}$ is the gravitational constant,and  $k_{B}=1.38\times10^{-23}$~m$^2$ kg s$^{-2}$ K$^{-1}$ is the Boltzmann constant.

where $r$ is the radius within which the mass is being measured, $\rho_{g}(r)$ is the baryon mass density profile, $T(r)$ is the temperature profile, $\mu=0.61$ is the mean molecular weight, 
%comment: Check this value, does it change with abundance table? DT |   I don't think it should, but the hydrogen/electron ratio in the density section will do DT |  I have seen other values used. PG | Vikhlinin  2006 used 0.5954 DT
$m_{u}$ is the atomic mass unit, $G$ is the gravitational constant, and $k_{B}$ is the Boltzmann constant. This is under the assumption that the cluster is spherically symmetric and in hydrostatic equilibrium. 

In this section we describe how we use \xga{} to measure gas density and temperature profiles, fit models to them, and then derive hydrostatic mass profiles from which we can obtain masses. As in Section~\ref{sec:xga} we present comparisons to measurements from literature, both of gas masses and hydrostatic masses.

\xga{} can measure various different types of radial profile for extended X-ray sources, both from X-ray images and spectra, and as such we implemented a set of classes to provide easy access to the data, model fitting, and visualisation. Specific profile classes also include other features, such as the hydrostatic mass profile's ability to measure a mass or a gas fraction. Such profiles can either be generated by \xga{} or set up from existing data, though we do not compare profiles from literature to \xga{} profiles in this work.

\subsection{Fitting models to radial profiles in \xga{} }
%comment: Should this section not be moved to after generating the profiles themselves? PG | Well I did consider that, but the section involving profile generation tend to have some mention of fitting models - in the case of density profiles the fitting of models to the SB profile is integral to the process, so I thought I'd just put it first DT
\label{subsec:radmodfit}

\begin{table*}
%comment: Some of these priors and start values might change, just will need to do a final check at some point DT | Would just the equation be better than the brief description column? | this should be in an appendix KR | if descriptions are changed to equations then this will need to be removed DT
\centering
\caption[]{{\small Summaries of the \xga{} 1D radial models used in this work (though others are implemented and available). Model names and descriptions of their use are included. The units of model parameters are given, as well as the start parameters used for initial fits. Finally details of the parameter priors used for the full MCMC fit are given, where $\mathcal{U}$[A, B] indicates a uniform distribution with limits A and B.}\label{tab:models}}
\vspace{1mm}
\begin{tabular}{c|lccc}
\hline
\hline
 Model Name & Brief description & Parameters & Start Values & Priors \\
\hline
\hline
\multirow{6}{7.5em}{\centering Double Beta} & & $\beta_{1}$ & 1 & $\mathcal{U}$[0, 3]\\ &  & $R_{\rm{core},1}$ [kpc] & 100 & $\mathcal{U}$[1, 2000] 
\\ & A simple model for the surface brightness profile, the sum of & $S_{01}$ [$\rm{ct}\rm{s^{-1}}\:\rm{arcmin}^{-2}$] & 1 & $\mathcal{U}$[0, 3]\\ & two $\beta$ models. &  $\beta_{2}$$ & 1 & $\mathcal{U}$[0, 3]\\ & & $R_{\rm{core},2}$ [kpc] & 100 & $\mathcal{U}$[1, 2000] 
%comment:  Reference maybe DT
\\ & & $S_{02}$ [$\rm{ct}\rm{s^{-1}}\:\rm{arcmin}^{-2}$] & 1 & $\mathcal{U}$[0, 3] \\
\hline
\multirow{6}{7.5em}{\centering Simplified Vikhlinin Density} & & $\beta$ & 1 & $\mathcal{U}$[0, 3]\\ &  & $R_{\rm{core}}$ [kpc] & 100 & $\mathcal{U}$[0, 2000] 
\\ & A simplified version of the \cite{vikhlininmass} density profile, as & $\alpha$ & 1 & $\mathcal{U}$[0, 3]\\ & used by \cite{simpvikhprofile}. & $R_{\rm{s}}$ [kpc] & 300 & $\mathcal{U}$[0, 2000]\\ & & $\epsilon$ & 2 & $\mathcal{U}$[0, 5] 
\\ & & $N_{0}$ [M$_{\odot}$ Mpc$^{-1}$] & $1\times10^{13}$ & $\mathcal{U}$[1, 10000]$\times10^{12}$ \\
\hline
\multirow{6}{7.5em}{\centering Simplified Vikhlinin Temperature} & & $R_{\rm{cool}}$ [kpc] & 50 & $\mathcal{U}$[10, 500]\\ &  & $a_{\rm{cool}}$ & 1 & $\mathcal{U}$[0, 5] 
\\ & A simplified version of the \cite{vikhlininmass} temperature profile, as & $T_{\rm{min}}$ [keV] & 3 & $\mathcal{U}$[0.1, 6]\\ & used by \cite{simpvikhprofile}. & $T_{0}$ [keV] & 6 & $\mathcal{U}$[0.5, 15]\\ & & $R_{\rm{T}}$ [kpc] & 200 & $\mathcal{U}$[100, 500] 
\\ & & c & 1 & $\mathcal{U}$[0, 5] \\
\hline
\end{tabular}
\end{table*}

Various aspects of this work require models to be fitted to radial data profiles. 
%comment: you haven't said how radial profiles are made yet (that can be after current 3.6) KR
For this work 
%comment:  other approaches include non linear least square, ODR,  (N>B> nLls used to set up mc walkers) KR
we make use of the \texttt{emcee} ensemble MCMC sampler which has been widely used in the astronomy community \citep[][]{emcee}. This sampler runs multiple interconnected MCMC chains to explore the parameter space. We choose to use a simple Gaussian likelihood function and uninformative uniform priors. The priors are dependant upon the particular profile being fitted, as well as the model choice, and further information can be found in table \ref{tab:models}.

All profile fitting performed for this work used an \texttt{emcee} sampler instance with 20 walkers, each taking 30000 steps. We chose to generate sets of start positions for the walkers by adapting a simple method suggested in the \texttt{emcee} documentation. We use the \texttt{SciPy} \citep[][]{scipy} implementation of the non-linear least squares (NLLS) fitting method (\texttt{curve\_fit}) to fit the model to the profile. The NLLS fits use starting values for model parameters as defined in Table~\ref{tab:models}. We then find the order of magnitude of each fit parameter. These are then perturbed by drawing an $N_{\rm{walker}}\times N_{\rm{par}}$ 
%comment: parameter definitions PG
matrix of random values from a $\mathcal{N}(0, 1)$ distribution, multiplying each random value by the order of magnitude of the respective parameter, and then adding this perturbation to the original NLLS best fit value. Before starting, the sampler checks to ensure that the start positions all fall within the allowed boundaries of the priors, and if not then they are re-drawn until they do.
% On the rare occasions that the \texttt{curve\_fit} run fails, we fall back on a maximum likelihood method where we attempt to minimise the negative log likelihood to find best fit parameters, then those parameters are perturbed in the same way to generate start positions for the walkers. 

Once the sampler run is complete, we calculate integrated autocorrelation times for the model parameters, if all autocorrelation times are more than 400 times smaller than the number of steps taken by a walker, then we find the mean autocorrelation time for all the parameters, round it up to the nearest 100, and double it to find a good number of steps to remove from each walker's chains as a burn-in period. If any of the parameters had an autocorrelation time that did not fit this criteria, then we take a brute force approach and remove the first 30\% of steps in each walker's chains. We draw 10000 random points from combined parameter chains from all walkers to create the final posterior distributions. We also measure medians of the parameter posterior distributions, as well as finding the 1$\sigma$ regions.

These fits are performed using a set of radial model classes that we have implemented in \xga{}. They provide easy access to model posterior distributions, visualisations, and predictions. \xga{} models also have implementations of useful mathematical operations such as differentiation, spherical volume integration, and inverse Abel transformation of the models \citep[using PyAbel;][]{pyabelmeth,pyabelsoft}, making use of Astropy \citep[][]{astropy1, astropy2} to provide correct units for any calculated quantities. Model instances also provide information on model parameters, support custom start parameters, and also custom priors. 

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\columnwidth]{images/a907_psf.png}
%    \caption{A figure demonstrating the image PSF correction capabilities of \xga{}. The left hand side shows a zoomed view of the original combined RateMap (stacked images from multiple observations and instruments divided by the equivalent stacked exposure maps). The right hand side shows the same zoomed view of the PSF-corrected stacked RateMap, where the individual images were all corrected separately and then stacked, then divided by the same combined exposure maps.}
%    \label{fig:a907psfcorr}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\columnwidth]{images/xxl_beta_king_1.3r500_gm_comp.pdf}
%    \caption{A one-to-one comparison of gas masses measured for the XXL-100-GC cluster sample, within $R_{500}$, by \cite{xxlbaryon} and an \xga{} reanalysis. {\color{red} $S_B$ profiles were fitted with Beta profiles, density profiles with King profiles. Contains measurements for 91 of 96 XXL-100-GC clusters analysed with \xga{}.}}
%    \label{fig:compxxlgm}
%\end{figure}

%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/locuss_1r500_gmcomp_dblbeta_svikh.pdf}
%    \caption{A one-to-one comparison of gas masses measured for the LoCuSS High-$L_{\rm{X}}$ cluster sample, within $R_{2500}$ and $R_{500}$, by \cite{locusshydro} and an \xga{} reanalysis.}
%    \label{fig:complocussgm}
%\end{figure*}

\subsection{PSF correction of \xmm{} images }
\label{subsec:psfcorr}

To measure a valid density profile from the surface brightness profile of a galaxy cluster (presented in Section~\ref{subsec:gasdensprof}), the effect of the instrument point spread function (PSF) must be accounted for. The PSF will have caused detected photons to be deflected from the position on the detector that corresponds to their true emission point on the cluster, changing the shape of the eventually measured surface brightness profile.

The \xmm{} EPIC-PN on-axis PSF has a full width half maximum of ${\sim}12.5\arcsec$, and the EPIC-MOS1 and MOS2 camera on-axis PSFs have a FWHM of ${\sim}4.3\arcsec$. The PSF of all three EPIC cameras changes size and shape depending on the position on the detector, with the PSF causing stretching of bright sources along the azimuthal direction. PSF effects are particularly noticeable for very bright point sources (causing spoking and smearing of the source), as the high photon count-rate means that enough photons arrive to trace the structure of the PSF effect, rather than the structure of the source. The \xmm{} PSFs also have a non-zero effect on observations of extended sources, especially brighter ones. Previous analyses \citep[e.g.,][]{croston,xxlbaryon} have accounted for this by constructing a mixing matrix that describes the shifting of photons between different radial bins by a 1D model of the PSF.  

We have taken a different, generalised, approach to correcting for PSF effects. Rather than apply PSF corrections in 1D after the surface brightness profile has been created, we opt to correct the image itself, from which a profile will then be generated. This approach has several advantages when compared to the mixing matrix method. The primary benefit is the ability to correct in two dimensions, especially important for off-axis clusters (where the {\em XMM} PSF becomes highly non-symmetric). It also reduces the spread of any point sources that may be contaminating the cluster of interest, making them easier to fully remove from the observation with the \xga{} generated mask. Also, as images are PSF corrected without reference to a particular source, they can be used in many different types of analysis.

We applied the widely used Richardson-Lucy algorithm, presented in both \cite{richardson} and \cite{lucy}, to individual {\em XMM} images to correct for PSF effects. Instances of the \texttt{ELLBETA} PSF model developed by \cite{readpsf} are generated using the \texttt{SAS} \texttt{psfgen} tool. An added complication is the variation of the PSF over the field of view; the Richardson-Lucy algorithm involves convolving the PSF function with the image, and when the PSF varies dependant on position there is no one to use. As such, each observation is divided into a grid of chunks, with a PSF being generated for the centre of each chunk, and each chunk being of equal size. The number of bins per side of the image is user configurable, with all corrections in this work using four bins per side, making sixteen chunks. Then, for each chunk, the whole image is convolved with that PSF (this is to avoid edge effects caused by Fast Fourier Transform convolution), and then the chunk is cut out of the convolved image and stitched into a final,  %comment: I'm not sure I follow this process. PG
overall image. This convolution process is then iterated, until a final output image for each ObsID-Instrument combination associated with a source is generated (all correction in this work uses 15 iterations). Once individual PSF-corrected images are created, stacked PSF corrected images are created in the same way uncorrected stacked images are made (Section~\ref{subsec:xgaphot}). They are then divided by the existing stacked exposure maps to create PSF-corrected stacked count-rate maps. Figure~\ref{fig:a907psfcorr} shows an example comparison of a pre- and post-correction combined count-rate map.

\subsection{Gas density profiles }
\label{subsec:gasdensprof}

%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/sbdprofs.png}
%    \caption[SB and \E profiles]{This figure shows visualisations of profiles generated by \xga{} for a galaxy cluster from the SDSSRM-XCS sample, SDSSRMXCS-134. The left hand side shows a surface brightness profile, generated from a combined image in the 0.5-2.0~keV energy band. It has been fitted with a double beta model. The right hand side shows the density profile generated from the surface brightness profile, with a simplified Vikhlinin density model fitted.}
%comment: I'm confused by the first annulus.  Why is there a gap between the first and second annuli?  Also, the first annulus seems to be centered on 1 kpc, but then goes up to 14 kpc hence:1 kpc -1 +14? PG |  Is this that bug you found? PG
%    \label{fig:sbdensprof}
%\end{figure*}

%As discussed in Section~\ref{sec:radxga}, one of the prerequisites of measuring a cluster hydrostatic mass is a radial gas density profile. Not only are the value and gradient of this profile (at a given radius) a key part of Equation~\ref{eq:hydromass}, but density profiles also give us insights into the baryon content of a cluster.
%comment: not needed? PG

% assume input centroid [ what about peak finding?] ; measure global Tx; put down annuli; subtract flat background; sum up counts per annuli, norm'd by area; invert via Abel transform; divide by APEC normalisation

In \xga{} we have implemented functionality to measure 3D density profiles 
%comment:: how does our method compare to previous in lit? KR| generally similar, except PSF correction (e.g. Croston) KR
from radial X-ray surface brightness profiles, $S_{B}(r)$. This method implicitly assumes that the cluster is spherically symmetric.  Furthermore, the analysis assumes the observed X-ray emission can be described by an \texttt{APEC} \citep[][]{apec} plasma model with galactic hydrogen column absorption provided by \texttt{tbabs} \citep[][]{tbabs}, and that emission from contaminating sources (and the X-ray background) has been properly removed.
%comment:  how is background removal done? KR

We use \xga{} to construct radial surface brightness profiles from combined (Section~\ref{subsec:xgaphot}) PSF corrected (Section~\ref{subsec:psfcorr}) ratemaps. For the XXL-100-GC and LoCuSS High-$L_{\rm{X}}$ samples the profiles are centred on the X-ray derived coordinates from literature, and for the SDSSRM-XCS sample we centre on the X-ray centroid positions from the XCS source finder \xapa{}. Galaxy cluster surface brightness profiles are generated out to $R_{500}$ (taken from literature), and an annulus of between 1.05-1.5$R_{\rm{500}}$
%comment: But not for XXL? PG
is used to measure a background level. Contaminating sources are removed prior to profile generation by applying an \xga{} generated mask to the combined image used for generation. Surface brightness profiles
%comment: at this point in counts per sec per pixel? KR
are generated by the \href{https://xga.readthedocs.io/en/latest/xga.imagetools.html\#xga.imagetools.profile.radial_brightness}{\texttt{radial\_brightness}} function, with radial bins of width 1~pixel.
%comment: : why? what about at low s:n?  [pixel scale is XCS specific] KR | should be fine for most of clusters in this paper, but might be concern for XXL KR |
\xga{} surface brightness profiles are measured in the 0.5-2.0~keV energy range by default. 
%The measured profiles are then stored in an \xga{} \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.SurfaceBrightness1D}{SurfaceBrightness1D}} instances. 
%comment: not needed? PG
We then fit the double beta model 
%comment: Make the decision on which model DT |  Beta model gas masses are way better for XXL though... DT | let's say we do this and other models are available KR
(Table~\ref{tab:models}) to the surface brightness profile data (fit method information in Section~\ref{subsec:radmodfit}, model information in Table~\ref{tab:models}). Once a profile has been parametrised, we use an inverse-Abel transform to deproject it from a 2D
%comment: are 2D profiles useful for anything else? KR
into a 3D profile, assuming spherical symmetry (this has an analytical solution for the double beta model).
%comment: reference KR
This results in a 3D radial volume emissivity profile $\epsilon(R)$, in units of photons per second per volume.

Next, we need to make use of the definition of the APEC emission model normalisation,

%comment: 


\begin{equation}
    N_{\texttt{APEC}} = \dfrac{10^{-14}}{4\pi(D_{A}(1+z))^2}\int n_e n_H dV,
	\label{eq:apecnorm}
\end{equation}
where $N_{\texttt{APEC}}$ is the normalisation of the \texttt{APEC} plasma emission model (in units of $\rm{cm}^{-5}$), $D_{A}$ is the angular diameter distance to the cluster (in units of cm), $z$ is the redshift of the cluster, $n_{e}$ and $n_{p}$ are the electron and hydrogen number densities (in units of $\rm{cm}^{-3}$). This will help infer the gas density profile by enabling a conversion between the volume emissivity profile $\epsilon(R)$, and the density profile.

We calculate a conversion factor, $K_N$, between \texttt{APEC} normalisation ($N_{\texttt{APEC}}$) and count-rate ($C_r$), where $N_{\texttt{APEC}} = K_N C_r$. To calculate the conversion factor, $K_N$, we implement an \xga{} interface to the \texttt{XSPEC} tool \texttt{FakeIt}, which can be used to simulate spectra given an emission model and an instrument response. 

This is used to generate simulated spectra for every instrument of every observation of a particular cluster (using ARFs and RMFs generated at the cluster coordinates during the generation of spectra, see Section~\ref{subsec:xgaspecs}). The simulations are performed using an \texttt{APEC} model absorbed with \texttt{tbabs}. The nH value for \texttt{tbabs} is set to the \cite{nh} value for that cluster. The spectra are simulated with a set normalisation of 1, a set temperature measured for that cluster
%comment: Not sure exactly how much a difference this makes, but when we calculated gas masses, we assumed a radial temperature profile for the cluster rather than a fixed-Tx. PG | Guess it doesn't really matter as XXL used a fixed Tx. PG
(within $R_{500}$ for LoCuSS High-\lx{}/SDSSRM-XCS, within 300~kpc for XXL-100-GC), a metallicity of 0.3~$Z_{\odot}$, and the input redshift of the cluster. The simulated spectra are all `observed' for a set exposure time of 10~ks, and are used to measure count-rates in the 0.5-2.0~keV band, which corresponds to the energy range of the ratemaps used to generate surface brightness profiles. The count-rates for each instrument of each observation are then weighted by the average effective area between 0.5-2.0~keV (drawn from the corresponding ARF) and combined into a single conversion factor $K_N$ by the \href{https://xga.readthedocs.io/en/latest/xga.sources.html\#xga.sources.extended.GalaxyCluster.norm_conv_factor}{\texttt{norm\_conv\_factor}} method of the \texttt{GalaxyCluster} class. This conversion factor is suitable for use with emissivity profiles generated from combined ratemaps.

This conversion factor, $K_N$, allows Equation~\ref{eq:apecnorm} to be written in terms of the 3D emissivity $\epsilon(R)=\frac{C_{r}(R)}{V}$ (which we can measure), and the product of the electron and hydrogen number densities $n_{e}n_{H}$ (which we can use to calculate the total gas density), 

\begin{equation}
    n_{e}(R)n_{H}(R) = \dfrac{4\pi K_{N}(D_{A}(1+z))^2C_{r}(R)}{10^{-14}V}.
    %comment: define a variable to make next eq easier to read KR
	\label{eq:halfway}
\end{equation}

At this point we must assume the ratio of electrons to hydrogen in the intra-cluster medium, so as to calculate a total gas density. We choose to use the solar abundances presented in \cite{andgrev} to calculate this ratio, $R_{eH}=1.199$. 
%comment: I stole this from pyproffit code and I still don't know how its calculated, but I would like to know DT
The total gas number density $n_{g} = n_{e}+n_{H} = (1+R_{eH})n_{H}$, is thus calculated by finding an expression for $n_{H}$ from Equation~\ref{eq:halfway}, then using $R_{eH}$ again to find $n_{e}$ and sum the two number densities. At this point the mean molecular weight $\mu=0.61$ and the atomic mass unit are used to convert number density to mass density. Thus, we calculate gas density from emissivity with quantities that we can measure, or already know;

\begin{equation}
    \rho_{\rm{gas}}(R) = \mu m_{u}(1+R_{eH})\sqrt{\dfrac{4\pi K_{N}R_{eH}\epsilon(R)(D_{A}(1+z))^2}{10^{-14}}}.
	\label{eq:dens}
\end{equation}
%comment:  does this basically boil down to: rho_c = X.(n_e . n_p)^1/2 | where X = mu.m_u.(1 + R) | PG

Once gas density
%comment: need to explain how errors are determined on each value KR
is measured using Equation~\ref{eq:dens}, it is stored in a \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.GasDensity3D}{GasDensity3D}} instance. We then use the fitting functionality discussed in Section~\ref{subsec:radmodfit} to fit simplified Vikhlinin density models (see Table~\ref{tab:models}) to the profiles. 

Once a gas density profile has been measured (and had a model fitted to it) we perform a spherical volume integral,

\begin{equation}
    M_{\rm{gas}}(<R_{\Delta}) = 4\pi \int_{0}^{R_{\Delta}} \rho_{\rm{gas}}(R)R^2 dR,
	\label{eq:volint}
\end{equation}
%comment: Double check and also write this in terms of the other quantities already defined DT
to measure a gas mass within a given radius. \xga{} can also perform this integral at a set of radii to create a cumulative gas mass profile (stored in \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.GasMass1D}{GasMass1D}}).

\subsection{Comparisons of \xga{} gas mass measurements to literature}
%comment: In both of these sections I need to specify models used for SB and density profiles, outer radii etc. | Either in the actual subsubsections, or globally if they are the same. DT
%comment:  Gas mass measurements also come from profiles, so link to the gas density profile or whichever one is the source of gas mass measurements DT

\label{subsec:compgasmasses}

We compare \xga{} measurements to previous measurements of the XXL-100-GC and LoCuSS High-$L_{\rm{X}}$ samples, similar to the comparisons we made in Section~\ref{subsec:comptxlx}. %To verify our measurements of the gas density profiles, we directly compare total gas masses measured within different apertures. 

\subsubsection{XXL-100-GC gas masses - moved}
\label{subsubsec:xxlgasmass}

We generate baryon density profiles for {\color{red} ??} clusters in the XXL-100-GC sample, with outer radii of $R_{500}$ \citep[overdensity radii measured by][]{xxlbaryon}. To maximise consistency we use the XXL measured $T_{\rm{300kpc}}$ values in the calculation of the conversion factors ($K_{N}$) between APEC normalisation ($N_{\texttt{APEC}}$) and count rate ($C_{r}$). Each cluster's neutral hydrogen column density is used in the conversion factor calculation, as is its redshift, and we assume a metallicity of 0.3~$Z_{\odot}$.  Figure~\ref{fig:compxxlgm} shows the comparison between \xga{} measured and original XXL gas masses. %The calculation of gas masses requires only a gas density profile and a radius within which to calculate, and as such comparing gas masses is an effective probe of our density profiles.

There is broad agreement between the two sets of measurements. This is encouraging considering the significant differences in density measurement between the two samples; including the PSF correction method, fitting method, and other differences mentioned in Section~\ref{subsubsec:xxllt}. We observe that the comparison isn't a perfect 1:1 relation, and that there is an offset between the two measurement sets that evolves with gas mass. An evolving offset between \xga{} and XXL \lx{} measurements was also observed in Figure~\ref{fig:xxltxlxcomp}, with the explanation for both likely being different background treatments. 

\subsubsection{LoCuSS High-$L_{\rm{X}}$ gas masses - moved}
\label{subsubsec:locussmasses}

Gas masses are also available for the LoCuSS High-$L_{\rm{X}}$ cluster sample, and we perform a comparison between the original values measured by \cite{locusshydro} and our reanalysis of the sample. LoCuSS provides an extra point of comparison, especially as the clusters also have gas masses measured within $R_{2500}$. Observations of LoCuSS High-$L_{\rm{X}}$ clusters also tend to be more massive and better observed than XXL-100-GC clusters (having dedicated pointed observations rather than being part of a survey). We estimate gas masses within the overdensity radii provided in \cite{locusshydro}
%comment: That might be a lie? DT
in order to minimise analysis differences.

Comparisons for $M^{\rm{gas}}_{\rm{500}}$ and $M^{\rm{gas}}_{\rm{2500}}$ are presented in Figure~\ref{fig:complocussgm}. We measure density profiles out to a radius of $R_{500}$. We see that the \xga{} measurements of $M^{\rm{gas}}_{2500}$ are consistently higher than their LoCuSS counterparts; we can infer that the LoCuSS analyses measure fewer baryons in the core regions of the clusters than the \xga{} does.

\subsection{Generating and fitting annular spectra with \xga{}}
\label{subsec:annspec}

%\begin{figure}
%    \centering
%    \includegraphics[width=1.\columnwidth]{images/sdssrmxcs134_annspec.png}
%    \caption{Set of annular spectra fitted folded models for SDSSRMXCS-134, performed by \texttt{XSPEC}, are shown as solid lines. Spectral data points are not included for clarity. The radius axis indicates the average of the inner and out radii of the annulus each spectra was measured from, with the zero point being the coordinate defined as the centre of the cluster.}
%    \label{fig:annspec}
%\end{figure}
%comment:  It's a bit difficult to see where the annuli appear on the plot.  Could you add shaded regions along the X-Y plane with a width equal to the annulus width? PG | Can you also plot in terms of r/r_500 PG

We wish to explore how certain spectral properties of a galaxy cluster vary with radius. As such, we implement methods to generate sets of annular spectra within radial bounds, as well as methods that attempt to find optimal bounds for the annuli. It is common practise to generate annuli with specific data quality; e.g. a minimum signal to noise or number of X-ray counts per annulus. This is to ensure that any spectra that are generated are of a sufficient quality for spectral fitting. We implement a function in \xga{} where annuli are constructed so that they have a minimum (user defined) background subtracted counts per annulus based on the combined observation of the cluster in question. We also impose a requirement of a minimum annulus width of 20\arcsec{} (also user configurable), to counter PSF effects of the extracted spectrum. Constructing the annuli is an iterative process, where initial annuli of the minimum allowed width are constructed between the cluster centre (the first annulus is a circle) and the outer radius specified for the set of annular spectra (though as the outermost radius must be an integer multiple of 20\arcsec{} the true outer radius will likely be slightly larger than what was initially specified for the cluster). These initial annuli are combined until the minimum signal-to-noise is achieved in all annuli, or until only four annuli remain. 

Annular spectra are generated using the same default settings as the global spectra detailed in Section~\ref{subsec:xgaspecs}. The set of annular spectra for a particular observation-instrument combination will (by default) have a background spectrum generated in the 1.05-1.5$R_{\rm{outer}}$ region, where $R_{\rm{outer}}$ is the outer radius of the $N^{\rm{th}}$ annulus. 
%comment: But what if R_{outer} still has cluster emission? Albeit, it will be low SNR.  For instance R_{outer} may be <R_{500} PG
To measure a temperature profile, we employ the same fitting technique that we applied to global spectra in Section~\ref{subsec:xgaspecs}; each annulus has simultaneous fits performed on all available data using the \texttt{constant*tbabs*apec} model. The same parameter start values and spectrum quality verification steps are used.

The generated spectra are stored in instances of an \xga{} product class, \href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.spec.AnnularSpectra}{\texttt{AnnularSpectra}}, as are the fit results. 
%This class simplifies access to the data and is used by other parts of \xga{} to perform spectral fits and generate radially varying profiles of fit quantities, it also includes convenient methods for visualising the data. 
Figure~\ref{fig:annspec} shows a visualisation of an example set of annular spectra for SDSSRMXCS-134 as a function of radius. It clearly illustrates the decreasing emission moving from the core of the cluster to the outskirts, as well as the flattening of the slope between ${\sim}$1-2~keV that indicates a lessening temperature.

\subsection{Three-dimensional gas temperature profiles }
\label{subsec:gastempprof}

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\columnwidth]{images/sdssrmxcs-134_tprof.pdf}
%    \caption{An example fitted three-dimensional temperature profile generated by \xga{} for a galaxy cluster in the SDSSRM-XCS sample, SDSSRMXCS-134. This visualisation was created using the view() method of the temperature profile. Data points are shown in black, and the simplified Vikhlinin temperature profile model is shown in green. This temperature profile was generated by deprojecting temperatures measured by fitting the annular spectra models shown in Figure~\ref{fig:annspec}.} 
%    \label{fig:tempprof}
%\end{figure}

The second property we must measure to calculate a cluster's hydrostatic mass is the three-dimensional temperature profile. First, we measure projected temperature profiles by generating spectra in annuli centered on the cluster coordinates, then performing spectral fits to each annulus to determine a temperature. Previous XCS work \citep[][]{xcsmethod} has indicated that around 1000 counts are required to measure well constrained temperatures (with percentage uncertainties of 10-30\%, depending on the temperature of the cluster). That means that all annuli need to have that many counts to achieve a well constrained projected temperature profile. We make use of the method described in Section~\ref{subsec:annspec} to generate annular radii, centered on the supplied cluster coordinates, that have a minimum number of counts defined by the user (3000 for the LoCuSS analysis, 1500 for the SDSSRM-XCS analysis).
%comment: why a different number of counts for SDSS?  Likely data quality issues, but should say.

Once the spectra have been generated, stored in an \href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.spec.AnnularSpectra}{\texttt{AnnularSpectra}} instance, and had \texttt{XSPEC} fits performed, the resulting projected temperature measurements (as a function of radius) are stored in an \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.ProjectedGasTemperature1D}{ProjectedGasTemperature1D}} instance.
Each projected temperature is a weighted combination of the temperatures in the three-dimensional shells of the cluster that the annulus intersects with. We opt to use the `onion-peeling' method \citep[see descriptions in e.g.,][]{onion1,onion2}. First, the volume intersections between the analysis annuli (projected back into the sky) and the spherical shells which we separate each cluster into (defined as having the same radii as the annuli) must be calculated. The volume intersections can be calculated  \citep[see Appendix A of][]{volintersec} as, 

\begin{equation}
\begin{split}
    \bm{V}_{\rm{int}} = \frac{4\pi}{3}\big[&max\{0, (\bm{R}_{\rm{so}}^{2} -  \bm{R}_{\rm{ao}}^{2})^{\frac{3}{2}}\} - max\{0, (\bm{R}_{\rm{so}}^{2} - \bm{R}_{\rm{ao}}^{2})^{\frac{3}{2}}\} +\\ & max\{0, (\bm{R}_{\rm{si}}^{2} - \bm{R}_{\rm{ao}}^{2})^{\frac{3}{2}}\} - max\{0, (\bm{R}_{\rm{si}}^{2} - \bm{R}_{\rm{ai}}^{2})^{\frac{3}{2}}\} \big],
\end{split}
\label{eq:intersec}
\end{equation}
%comment:  Maybe add the derivation to the GitHub repo DT
where $\bm{R}_{\rm{so}}$ is the matrix of shell outer radii, $\bm{R}_{\rm{ao}}$ is the matrix of annulus outer radii, $\bm{R}_{\rm{si}}$ is the matrix of shell inner radii, and $\bm{R}_{\rm{ai}}$ is the matrix of annulus inner radii. The calculation is implemented in the \xga{} function \href{https://github.com/DavidT3/XGA/blob/d8709eb1a0eb297f39ac50d4c4d9f1ad7122f9f0/xga/sourcetools/deproj.py\#L10}{\texttt{shell\_ann\_vol\_intersect}}. The $\bm{V}_{\rm{int}}$ matrix is a two dimensional matrix describing volume intersections between all combinations of annuli and three-dimensional shells.

% 

% \begin{equation}
%     \bm{V}_{\rm{int}} = \frac{4\pi}{3}(R_{\rm{out}}^{2} - R_{\rm{inn}}^{2})^{\frac{3}{2}},
% 	\label{eq:intersec}
% \end{equation}

Second, an emission measure profile (\texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.EmissionMeasure1D}{EmissionMeasure1D}}) is calculated using the \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.APECNormalisation1D.emission_measure_profile}{emission\_measure\_profile}} method of the \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.APECNormalisation1D}{APECNormalisation1D}} profile produced during the spectral fitting of the set of annular spectra. This calculation uses Equation~\ref{eq:apecnorm} and rearranges to solve for the integral. As the projected temperature measured within a given annulus is a weighted combination of the shell temperatures intersected by that annulus, we can infer the temperature of a shell \citep[for past usage see][]{onion2} with 

\begin{equation}
    \bm{T}_{\rm{shell}} = \dfrac{(\bm{V}_{\rm{int}}^{\rm{T}})^{-1} \times \bm{T}_{\rm{annulus}}\rm{\textbf{EM}}}{(\bm{V}_{\rm{int}}^{\rm{T}})^{-1} \times \rm{\textbf{EM}}}.
	\label{eq:tempdeproj}
\end{equation}
%comment: The maths does match up to that in the 2018 Ghirardini paper so its probably correct, though the expression they put in their paper has a mistake in that the T for transpose is replaced by Y DT

$\bm{T}_{\rm{shell}}$ is the matrix of spherical shell temperatures that we aim to calculate, $\bm{V}_{\rm{int}}$ is the matrix of volume intersections between all combinations of annuli and shells (see Equation~\ref{eq:intersec}), $\rm{\textbf{EM}}$ is the emission measure matrix, and $\bm{T}_{\rm{annulus}}$ is the projected temperature matrix; $\times$ represents the matrix product. Once calculated, the $\bm{T}_{\rm{shell}}$ values and uncertainties
%comment: explain how errors are measured KR
are stored in a \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.GasTemperature3D}{GasTemperature3D}} instance. 

Once three-dimensional, de-projected, gas temperature profiles have been measured, we use the methods discussed in Section~\ref{subsec:radmodfit} to model the profiles with the simplified Vikhlinin temperature model (see Table~\ref{tab:models} for more information). 
%Fitting a model enables the 




\subsection{Hydrostatic mass profiles }
%comment:  need to talk about error propagation through all of my profiles etc DT
\label{subsec:hydromassprof}

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\columnwidth]{images/sdssrmxcs-134_mprof.pdf}
%    \caption{An example hydrostatic mass profile generated for a galaxy cluster in the SDSSRM-XCS sample, SDSSRMXCS-134. This is profile was generated using the model fits to the density profile shown in the right hand side of Figure~\ref{fig:sbdensprof}, and the temperature profile shown in Figure~\ref{fig:tempprof}.}
%    \label{fig:hymprof}
%\end{figure}

Once we have measured a 3D radial density profile (details in Section~\ref{subsec:gasdensprof}) and a 3D radial temperature profile (details in Section~\ref{subsec:gastempprof}), we can use Equation~\ref{eq:hydromass} to measure hydrostatic masses. As such, \xga{} creates hydrostatic mass profiles as a function of radius (e.g. Figure~\ref{fig:hymprof}), which are stored in \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.HydrostaticMass}{HydrostaticMass}} class instances. The density and temperature profiles must have models fitted prior to the construction of a hydrostatic mass profile, with the fitting process described in Section~\ref{subsec:radmodfit} and models described in Table~\ref{tab:models}. The hydrostatic mass equation not only involves the temperature and density profile values at each radius for which a enclosed mass is measured, but also the derivatives of those profiles with respect to radius. The simplified Vikhlinin density and temperature profiles both have analytical first-derivatives, and as such these are used to calculate the slope at a given radius, rather than a numerical approximation. \xga{} models can return posterior distributions of the value of the model (or model slope) at a given radius, rather than a single value. This allows for uncertainties to be propagated from the density and temperature profile through to the mass profile.

%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/loc_sb_dblbeta_simpvikh_1r500_mc3000_hymcomp.pdf}
%    \caption{A one-to-one comparison of hydrostatic masses measured for the LoCuSS High-$L_{\rm{X}}$ cluster sample, within LoCuSS measured $R_{2500}$ and $R_{500}$ values, by \cite{locusshydro} and an \xga{} reanalysis.}
%    \label{fig:complocusshym}
%\end{figure*}

\subsection{Comparison of \xga{} hydrostatic mass measurements to the LoCuSS High-$L_{\rm{X}}$ sample}
\label{subsec:comphymasses}

As a consistency check, we use \xga{} to measure hydrostatic masses for the LoCuSS High-$L_{\rm{X}}$ sample.

To minimise differences with the original LoCuSS High-$L_{\rm{X}}$ hydrostatic mass analysis, we leave the metallicity of each annulus free to vary during the spectral fits. Density and temperature profiles are generated
%comment: Do you mean the profiles are generated out out 1.3R500, or the outer radius of the Nth annulus is 1.3R500? PG
with an outer radius of $R_{500}$, fitted with models as described in Section~\ref{subsec:gasdensprof} and Section~\ref{subsec:gastempprof}.  Mass profiles are constructed (see Section~\ref{subsec:hydromassprof}) and used to measure $M^{\rm{hy}}_{500}$ and $M^{\rm{hy}}_{2500}$. The temperature profiles are constructed with a minimum annular width of 20\arcsec, and a minimum number of background subtracted counts per annulus of 3000 (an attempt to maximise the similarity of this reanalysis with the original work). The background regions are taken from the 1.05-1.5$R_{\rm{outer}}$ annulus, where $R_{\rm{outer}}$ is the outer radius of the $N^{\rm{th}}$ annulus, which will likely be very slightly larger than $R_{500}$ (as described in Section~\ref{subsec:annspec}, the outer radius must be an integer multiple of the minimum annulus width).

Figure~\ref{fig:complocusshym} shows a comparison between the \xga{} and LoCuSS hydrostatic masses for $M^{\rm{hy}}_{2500}$ (left-hand-side) and $M^{\rm{hy}}_{500}$ (right-hand-side). We successfully measure mass profiles for 41 galaxy clusters in the LoCuSS High-$L_{\rm{X}}$ sample, 29 of which have \xmm{} hydrostatic masses measured by LoCuSS. When plotted directly against the published LoCuSS masses (specifically those measured by \xmm{}) we see a relatively good agreement for both overdensities. The agreement between the measured masses is not perfectly one-to-one; this is expected, since the number of components involved in measuring hydrostatic mass make it difficult to exactly match measurement methods between analyses. For example, \xga{} and LoCuSS take different approaches to measuring density profiles.  Furthermore, additional \xmm{} data is available for these clusters than there was at the time of the original \cite{locusshydro} analysis, which may have an effect on the constraints.

%Many of the same caveats discussed in Section~\ref{subsubsec:locusslt} (where we presented \tx{} and \lx{} comparisons for an \xga{} reanalysis of LoCuSS High-$L_{\rm{X}}$ clusters) also apply to these mass measurements. We use slightly different models than LoCuSS for the \texttt{XSPEC} fitting process, though we have found results to be consistent between them. We also use a different XSPEC fitting method, in terms of how the spectra are tied together, and our approach to the background annulus is different. 
%comment: Check that this is true DT
%Finally, there is more \xmm{} data available for these clusters now than there was at the time of the original \cite{locusshydro} analysis, which may have an effect on the constraints.

\subsection{Inspection of data and measurements}
%comment: What is this section going to be about? PG
\label{subsec:dataverif}

To ensure that the masses measured are valid, visual inspection of key data products is performed. This expands upon the visual inspection and region adjustment that was described in Section~\ref{subsec:manualdetreg}. All profile-based products that contribute to the measurement of the hydrostatic mass profiles are inspected; surface brightness, density, temperature, and finally the mass profiles.

The inspections are to look for obviously invalid or unphysical data. For instance, more complex than usual surface brightness profiles that have been poorly described by the double beta model fit to them. Temperature profiles with poor fits, very poorly constrained data points, or unphysical attributes (such as temperature increasing in the outskirts of a cluster) are flagged. Finally, mass profiles that do not appear to be strictly monotonically increasing are flagged, as each point in the mass profile represents an enclosed mass, so the mass measured at annulus $R_{j+1}$ must always be greater than at $R_{j}$. The \texttt{HydrostaticMass} class provides a method (\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.HydrostaticMass.diagnostic_view}{diagnostic\_view}) to generate a set of visualisations (a combination of Figures~\ref{fig:sbdensprof}, \ref{fig:tempprof}, and \ref{fig:hymprof}) for each cluster.


==> OldSections/OldSections30Jan2024/MethodologySection.tex <==

\section{Methodology}
\label{sec:methodology}

The overarching aim of this work is to provide an independent mass calibration for optically selected cluster samples for the purpose of cosmological parameter estimation. The masses are estimated using X-ray observations from \xmm{} under the assumptions of spherical symmetry and hydrostatic equilibrium \citep[see e.g.,][for a derivation]{1980ApJ...241..552F}, following the equation

%comment: this should go into end of Intro paragraph: say done on SDSS for now, and then on DES and LSST later? KR

\begin{equation}
    M_{\rm hydro}(<r) = - \dfrac{k_{B}r^2}{\rho_{g}(r)\mu m_{u}G} \bigg[\rho_{g}(r)\dfrac{dT(r)}{dr} + T(r)\dfrac{d\rho_{g}(r)}{dr}\bigg],
    \label{eq:hydromass}
\end{equation}
where $r$ is the radius within which the mass is being measured, $\rho_{g}(r)$ is the intracluster gas density profile, $T(r)$ is the gas temperature profile, $\mu=0.61$ is the mean molecular weight, $m_{u}$ is the atomic mass unit, $G$ is the gravitational constant, and $k_{B}$ is the Boltzmann constant. The quantities that need to be estimated from the \xmm{} data are $T(r)$ and $\rho_{g}(r)$. It is important to note that these are the 3 dimensional quantities, rather than the projected (i.e. what is observed) values. 

%comment: this is needed somewhere:  need to make it clear that we know they are not in hydro-eq. e.g. via footnote? KR

Many steps are needed to go from a raw \xmm{} observation to an estimate of $M_{\rm hydro}$.  Therefore, a secondary goal of this work is to streamline those steps into a single, self-contained pipeline. Doing so ensures the consistency of the data products and allows for computational speed-ups (e.g. by making use of multi-threading on multicore machines).
The measurement tools for $M_{\rm hydro}$ that we use herein are part of the X-ray: Generate and Analyse (\xga\footnote{\href{https://github.com/DavidT3/XGA}{\xga{} GitHub - https://github.com/DavidT3/XGA}}) software suite. \xga{} is a generalised X-ray analysis tool, capable of investigating any X-ray source that has been observed by \xmm{}. It was introduced in \cite{xgapaper} and is being used in a growing number of scientific applications \citep[e.g. ][]{denishapaper,efedsxcs,agnxga}. It is also listed on the Astrophysics Source Code Library \citep[ASCL;][]{asclxga}. This work makes use of \xga{} \verxga{} for all analyses, and to aid readability, the technical details about which parts of \xga{} are used for the different analyses in this work are described in Appendix~\ref{app:xgacommclass}.

In this section, we describe each step involved in \xga{} $M_{\rm hydro}$ measurements.
Section~\ref{subsec:xcsdata} explains the data inputs required to initiate \xga{}.
Image generation and masking of contaminating sources are described in Sections~\ref{subsec:xgaphot} and~\ref{subsec:xgacontam} respectively.  Manual checks of the data are outlined in Section~\ref{subsec:manualdetreg}.  Section~\ref{subsec:xgaspecs} details the generation and fitting of X-ray spectra.  Correcting for the {\em XMM} point-spread function (PSF) is detailed in Section~\ref{subsec:psfcorr}.  The generation of emissivity profiles, density profiles, temperature profiles and mass profiles are outlined in Sections~\ref{subsec:SBandEm},~\ref{subsec:densityProf},~\ref{subsec:gastempprof} and~\ref{subsec:hydromassprof} respectively. To illustrate the steps, we use two example clusters: \clustone{} and \clusttwo{} ($z=0.119$ and $z=0.223$ respectively). Both clusters were part of the \cite{xcsgiles} study (see Section~\ref{subsubsec:SDSSRMsim}), but have significantly different signal to noise ratios and off axis locations in their respective \xmm{} observations. Their properties are summarised in Table~\ref{tab:exampclusters}.

\begin{table*}
\begin{center}
\caption[]{{Properties of the two galaxy clusters selected as demonstration cases for \xga{}. These were selected from the SDSSRM-XCS sample presented by \cite{xcsgiles}. The coordinates are for the XCS \xapa{} defined value for the UDC$^{\ref{foot:udc}}$. This, and the $R_{2500}$ and $R_{500}$ values, in units of kpc, were taken from \cite{xcsgiles}. The redshift and richness values were taken from \cite{redmappersdss} (where the numeric value in the name is the identifier in the \cite{redmappersdss} RM catalogue). The XCS3P measured $T_{\rm X}$ and 0.5-2.0~keV $L_{\rm X}$ values are taken from \cite{xcsgiles}, and are given in $R_{2500}$ and $R_{500}$ apertures}\label{tab:exampclusters}}
\vspace{1mm}
\begin{tabular}{ccccccccccc}
\hline
\hline
Name & RA & Dec & $z_{\rm{RM}}$ & $\lambda_{\rm{RM}}$ & $R_{\rm{2500}}$ &$R_{\rm{500}}$ & $T^{\rm{XCS3P}}_{\rm{X,2500}}$ &$T^{\rm{XCS3P}}_{\rm{X,500}}$ & $L^{\rm{XCS3P, 52}}_{\rm{X,2500}}$ &$L^{\rm{XCS3P, 52}}_{\rm{X,500}}$ \\
\hline
\hline 
\clustone{} & 227.550 & 33.516 & 0.119 
& $99.80{\pm}3.74$\
& $562.3^{+7.5}_{-7.5}$ & $1237.6^{+20.1}_{-20.1}$ & $7.00^{+0.10}_{-0.10}$ & $6.70^{+0.08}_{-0.08}$ & $1.99^{+0.01}_{-0.01}$ & $2.77^{+0.01}_{-0.01}$ 
\\
\hline
\clusttwo{} & 36.455 & -5.894 & 0.223 
& $32.12{\pm}2.83$
& $321.9^{+24.4}_{-18.1}$ & $669.0^{+62.0}_{-47.9}$ & $2.89^{+0.38}_{-0.28}$ & $2.41^{+0.39}_{-0.29}$ & $0.16^{+0.01}_{-0.01}$ & $0.21^{+0.01}_{-0.01}$ \\
\hline
\end{tabular}
\end{center}
\end{table*}


\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{images/demo_clusters_RT.pdf}
    \caption[XAPA demo]{\xmm{} 0.5-2.0~keV stacked ratemaps of \clustone{} (left) and \clusttwo{} (right), which we have selected to demonstrate our methodology. Point sources are highlighted by red circles and extended sources by green ellipses.  The white cross-hair indicates the cluster centroid, and the solid circles indicate the location of $R_{2500}$ and $R_{500}$ (see Table~\ref{tab:exampclusters} for input values).   
    }
    \label{fig:xapaexample}
\end{figure*}

\subsection{Initiating \xga{}}
\label{subsec:xcsdata}

Throughout this work, we use public {\em XMM} data from the {\em XMM} Science Archive\footnote{\href{http://nxsa.esac.esa.int/nxsa-web/}{XSA - http://nxsa.esac.esa.int/nxsa-web/}} that has been pre-processed to produce cleaned event files and region lists. The region lists encode information about the source centroid, size, and shape. All pre-processing used herein relies on the the \xmm{} Cluster Survey \citep[][XCS hereafter]{xcsfoundation} methodology that is fully described in \cite{xcsmethod} and \cite{xcsgiles}. In brief, the initial EPIC (MOS and PN) data were processed with v14.0.0 of the \xmm{} Science Analysis Software \citep[SAS\footnote{\href{https://www.cosmos.esa.int/web/xmm-newton/sas}{SAS - https://www.cosmos.esa.int/web/xmm-newton/sas}};][]{sas}, using {\tt EMCHAIN} and {\tt EPCHAIN} functions to generate event lists. Following this, the event lists were screened for periods of high background 
%by generating light curves in 50 second time bins for the soft (0.1–1.0~keV) and hard (12–15~keV) bands. An iterative 3$\sigma$ clipping process was then performed on the light curves; time bins falling outside this range were excluded. 
and then individual (PN, MOS1, MOS2) and merged (PN+MOS1+MOS2) EPIC images (and corresponding exposure maps) were then generated. All images/maps have a pixel size of 4.35\arcsec. 
Next, X-ray source detection is performed using a custom version of {\sc wavdetect} \citep[][]{wavdetect} called \xapa{} (for XCS Automated Pipeline Algorithm). Once sources in an image have been located, \xapa{} classifies them as either point-like or extended sources. Region lists of sources are created for each \xmm{} observation (a given source can appear in multiple region lists if there are overlapping observations). Once all the observations have been processed, a master source list (MSL), with duplicates removed, is generated. 
To date, 12,582 observations have been processed by XCS, covering 1,068 non-overlapping square degrees of sky, and yielding 400,225 X-ray source detections in the 0.5-2.0~keV band.

%comment: we might need to define OBSID to simplify future mentions of "observations" KR

%KR: note that a region file is not a requirement - regions can be drawn on by hand, but that feature is not relevent to thiS paper

% This briefly sets the footnotes to 'symbol mode', so that we can use the dagger for a footnote
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

In addition to the XCS supplied cleaned event files and region lists, the following information is required to initiate the \xga{} analysis of a cluster: a coordinate for the cluster centre, the redshift, at least one radius to define the analysis region, and a set of values for the cosmological parameters $\Omega_M$, $\Omega_\Lambda$, and $H_0$. With regard to the cluster centre, this depends on the selection method (e.g. it could be defined by the brightest galaxy, rather than a feature in an X-ray image) and on the analysis method (e.g. it could be defined by the peak of the X-ray surface brightness or by the weighted centroid). Given this ambiguity, we henceforth refer to the user-defined coordinate (or UDC\footnote[2]{\label{foot:udc}The central coordinate input by the user, rather than a peak or centroid measured by \xga{}.}), rather than to the ``cluster centre''.

% This puts the footnote back to normal numbering
\renewcommand{\thefootnote}{\arabic{footnote}}


With regard to the analysis region radius, this can be an overdensity radius\footnote{Radius at which the average density of the enclosed cluster is equal to $\Delta\rho_{c}(z)$, where $\Delta$ is the overdensity factor and $\rho_{c}(z)$ is the critical density of the Universe at the cluster redshift.}, e.g. $R_{500}$, or a co-moving radius with no associated physical significance (e.g. 300 $h^{-1}$ kpc).
%a cosmological model from Astropy \citep[][]{astropy1,astropy2}.

 For our example clusters, \clustone{} and \clusttwo{} (and for the analysis presented in Section~\ref{sec:results}), the UDC$^{\ref{foot:udc}}$, the redshift, and the analysis region radii ($R_{2500}$, $R_{500}$) were taken from the data tables in \cite{xcsgiles}. As per \cite{xcsgiles}, the cosmological parameters were set to $\Omega_{\rm{M}}$=0.3, $\Omega_{\Lambda}$=0.7, and $H_{0}$=70 km s$^{-1}$ Mpc$^{-1}$.

 
%comment:   KR R_500 is explained in footnote, but we don't say how it was calculated in Paul's paper. Maybe not needed.

To ensure all relevant data sets are used during the analysis of a given cluster, \xga{} explores the full set of XCS processed data 
to retrieve any \xmm{} observations meeting these criteria; an aimpoint within 30\arcmin{} of the input UDC$^{\ref{foot:udc}}$, and >70\% of the chosen analysis region falling on active regions of the detectors. Two observations each were retrieved for our example clusters (Table~\ref{tab:exampclusters}), \clustone{} (0149880101 \& 0303930101) and \clusttwo{} (0404965201 \& 0677600131).

\subsection{Generating image and exposure maps}
\label{subsec:xgaphot}

Once the relevant {\em XMM} data have been retrieved, see Section~\ref{subsec:xcsdata}, \xga{} generates images, exposure maps, and ratemaps\footnote{The image divided by the exposure map.}.  For this, \xga{} interfaces with the \texttt{SAS} \texttt{evselect} and \texttt{eexpmap} tools. These images and maps are essential to the derivation of $M_{\rm{hydro}}$ as they are used during the estimate of $\rho_g(r)$, 
%comment: correct wording? KR
through the generation of surface brightness profiles (see Section~\ref{subsec:SBandEm}).  Images are also useful for inspection throughout the analysis process e.g., to check masked regions (see Section~\ref{subsec:manualdetreg}). 

We note that, in principle, the images already existing in the XCS archive (those on which \xapa{} was run) could have been used by \xga{} for the analyses herein. However, in practice, generation of fresh images is worthwhile because it simplifies the process of merging multiple observations, and gives additional freedom in the current analysis (e.g., selecting an energy range; XCS only stores images in the 0.5-2.0~keV and 2.0-10.0~keV ranges).
%we also do not anticipate that all potential users of \xga{} will have pre-generated all the images they require.

% and improves accessibility (the XCS images are currently not available via a public webserver). 

%in a user specified energy range, are generated by \xga{}. 

In Figure~\ref{fig:xapaexample}, we show the \xga{} generated \xmm{} images of our example clusters, \clustone{} and \clusttwo{}; these are the stacked images of every EPIC instrument for every usable observation of the clusters. 
%{\color{red} These images have been displayed using the \texttt{view} method of the \xga{} image class.} 
The \xapa{} (\S~\ref{subsec:xcsdata}) defined source regions are overlaid; with red (point source), green (extended source), or magenta (extended source similar in size to the PSF) outlines. The UDC$^{\ref{foot:udc}}$ is shown with a white cross. The analysis regions ($R_{2500}$ and $R_{500}$) are shown with white solid  outlines. 
Note that, in these examples, two observations have been stacked into a composite image. As each observation has its own source region list, multiple source outlines can sometimes be seen in the overlap regions.


\subsection{Automated source masking}
\label{subsec:xgacontam}

As described above (Section~\ref{subsec:xcsdata}), every XCS processed image has an associated list of detected source regions. Most of these will not be associated with the cluster of interest and need to be masked from both the image files (Section~\ref{subsec:xgaphot}), used during surface brightness fitting (Section~\ref{subsec:SBandEm}), and from the cleaned event lists (Section~\ref{subsec:xcsdata}), used during spectral analysis (Section~\ref{subsec:xgaspecs}). In almost all cases, the only source region not masked by default is the one associated with the cluster of interest (see below for two exceptions). This source is identified as the one containing the location of the UDC$^{\ref{foot:udc}}$. For the analysis herein, we apply an additional filter: the source must also have been classed as extended by the \xapa{} pipeline.  The black areas in Figure~\ref{fig:immask} (left)  show the region automatically masked for \clustone{}. This Figure is a zoom into the $3R_{500} \times 3R_{500}$ region of Figure~\ref{fig:xapaexample} (left).

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{images/demo_cluster_mask.pdf}
    \caption[image auto mask]{An \xmm{} 0.5-2.0~keV stacked ratemap of  \clustone{}. The white cross-hairs indicate the UDC$^{\ref{foot:udc}}$. 
    Left: 
    The solid circles indicate the location of $R_{2500}$ and $R_{500}$. The dashed annulus indicate 1.05-1.5$R_{500}$ (the background region used in the global spectral analysis, see Section~\ref{subsec:xgaspecs}).  An automated mask, to remove contaminating sources identified by {\sc xapa} has been applied (black areas, see Section~\ref{subsec:xgacontam}). Right: The default mask has been adjusted by hand to remove more emission from the bright point source in the top left (see Section~\ref{subsec:manualdetreg}). The solid (dashed) circles indicate the source (background) regions used during the radial spectral fitting (see Section~\ref{subsec:xgaspecs}).}
    \label{fig:immask}
\end{figure*} 

Below are two exceptions to the masking process detailed above:
\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
 
\item[--] The treatment of \xapa{} point-like sources detected within 0.15$R_{500}$ of the cluster centroid. These sources are not masked because \xapa{} occasionally misidentifies cool cores of clusters as point sources.
%comment: should we give an example in a figure? KR 
%comment: not sure if this is worth saying here, or if it muddies the water, so leaving out KR | (Alternatively, they may be AGN in the central BCG. The inclusion of contaminating, i.e. not from the ICM, flux adds to systematic errors in derived quantities and subsequent scatter in scaling relations.) 
\item[--] The treatment of overlapping \xapa{} extended source regions. If the cluster of interest was observed in two or more XMM pointings, then the associated \xapa{} extended sources may not fully overlap. This is more likely if the observations are offset from each other and/or that have differing exposure times. Therefore, if the respective source centres are within a projected distance of $<R_{500}$ of the input cluster centroid, then none of those source regions are masked. 

\end{itemize}

%comment: we have not mentioned times when XAPA breaks up a cluster on a single obsid KR this is because there are no incidences of that in this paper DT

\subsection{Manual data checks}
\label{subsec:manualdetreg}

Once the images have been generated (Section~\ref{subsec:xgaphot}) and the default masks applied (Section~\ref{subsec:xgacontam}), the next step involves manual intervention via eye-ball checks to {\em i}) identify observations that were not suitable for further analysis, {\em ii}) increase the size of masked regions if the default mask was not large enough, and {\em iii}) add masked regions for sources missed by \xapa. With regard to {\em i}), this process is similar to that described in Section~2.3 of \cite{xcsgiles}. It is used to remove, from further analysis, observations with abnormally high background levels \citep[e.g. Figure~A1(a) of][]{xcsgiles}, and those corrupted by a very bright point source\footnote{Such sources produce artefacts in the {\em XMM} images including readout streaks and ghost images of the telescope support structure.} \citep[e.g. Figure~A1(b) of][]{xcsgiles}. 
%The only difference compared to the \cite{xcsgiles} approach was that the inspection was carried out using the \xga{} visualisation tool {\color{red}XX}. 
Of the 457 \xmm{} observations identified as being relevant to the clusters in this paper, 43 were rejected entirely, and 4 had data from one or more (of the 3 EPIC) instruments rejected.

With regard to {\em ii}), occasionally the \xapa{} defined region is not large enough to encapsulate all the emission from a bright point source, or from a neighbouring (but physically distinct) extended source. This can impact subsequent analysis if the source falls in either within $R_{500}$ of the cluster UDC$^{\ref{foot:udc}}$ or within the background annulus. For the \cite{xcsgiles} analysis, this extra masking step was cumbersome and time-consuming. So, in \xga{}, a GUI was developed that makes it simple to interact with, and modify existing regions. With regard to {\em iii}), there is a rare \xapa{} failure mode whereby it fails to detect all the sources in a given observation. Using the GUI,
%{\tt edit\_regions}, 
it is easy to add new regions if a source or artefact (visible by eye in the image) has been missed by \xapa{}. 

Combined images (all observations, all instruments) for each of the galaxy clusters in this work were examined, and adjustments to regions were made. We altered or added regions for 60 (40\%) of the SDSSRM-XCS sample, 44 (44\%) of the XXL-100-GC sample, and 26 (56\%) of the LoCuSS High-\lx{} sample. Figure~\ref{fig:immask}  (right) shows part of the \xmm{} observation containing \clustone{}. This Figure highlights where a source mask has been expanded from its default (\xapa) size. 

\subsection{Generating and fitting X-ray spectra}
\label{subsec:xgaspecs}

Spectral analysis is essential to the estimation of hydrostatic masses, both for the derivation of $\rho_g(r)$ and $T(r)$. In the case of $\rho_g(r)$, only a global (cluster wide) spectral analysis is needed, whereas for $T(r)$, spectral analysis in radial bins is required. 

For the global spectral analysis of our example clusters, the analysis region (radius and UDC$^{\ref{foot:udc}}$) is defined by the user as an initiation input to \xga{} (Section~\ref{subsec:xcsdata}). A background region also needs to be defined. In the implementation of \xga{} used herein, the background region is an annulus. For our example clusters, \clustone{} and \clusttwo{} (and for the analysis presented in Section~\ref{sec:results}), the inner and outer radii of the annulus are set at 1.05R$_{500}$ and 1.5R$_{500}$ respectively.
 
For the radial analysis, \xga{} uses a series of $N$ circular source apertures with increasing radii, out to a user defined outer radius, $R_{\rm{outer}}$ and UDC$^{\ref{foot:udc}}$. The innermost aperture is a full circle, the others are annuli. The user defines a minimum annulus width (also the inner circle radius) in arcseconds, $\Delta\theta_{\rm min}$. This minimum is set to account for the PSF of the instrument. For all the cluster analyses herein, we set this to be $\Delta\theta_{\rm min}$=20\arcsec{} (roughly twice the FWHM of the \xmm{} EPIC-PN on-axis PSF, see \S~\ref{subsec:psfcorr}). 
If the specified $R_{\rm{outer}}$ value for a given cluster, when converted to units of arcseconds ($\theta_{\rm{outer}}$), is not an integer multiple of $\Delta\theta_{\rm min}$, it is adjusted (outwards) accordingly, to become $\theta_{\rm{outer}}'$. A background region is then defined and used for all the bins. For the analysis of our example clusters, \clustone{} and \clusttwo{} (and the analysis presented in Section~\ref{sec:results}), it was set to be an annulus of 1.05-1.5~$\theta_{\rm{outer}}'$. 



%comment:  what if the outer radius is still inside cluster emission? The background ring will be too small. Should there be a caveat that R_outer must be larger than R_500? PG
The widths of the bins used in the spectral analysis are set through an iterative process. This starts with determining whether $\theta_{\rm{outer}}'$ is at least $4\times\Delta\theta_{\rm min}$. If not, then the process stops (because it is not realistic to generate a $T(r)$ profile from less than 4 bins). If it is exactly $4\times\Delta\theta_{\rm min}$, then 4 bins (each of $\theta_{\rm min}$ in width) are used in the analysis. If it is $5\times\Delta\theta_{\rm min}$, then some bins may be expanded (to $2\times\Delta\theta_{\rm min}$, $3\times\Delta\theta_{\rm min}$ etc.) to improve the signal to noise. The width of a given bin expands (inwards) until either a) the user defined minimum number of background subtracted counts is reached, or b) the number of bins drops to 4.
The number of bins defined in this way will depend on the quality of the detection and on the $R_{\rm outer}$ (and hence projected size) of the cluster.

The way that the annular spectra are spatially binned can have a significant effect on the temperature profiles that are created from them, and different criteria may be used to decide on the spatial binning. The goal is to make the extraction region large enough that sufficient X-ray counts are present to constrain spectral properties (e.g. temperature), whilst maintaining a good spatial resolution.

Achieving a minimum number of counts per spectral annulus is not always sufficient to guarantee a `good' temperature profile. In an effort to mitigate potential issues, we generate two sets of temperature profiles, with different targeted counts per bin (1500 and 3000 counts). As 1500 counts should be sufficient for a well constrained $T_{\rm X}$ value \citep[see Figure~16 in][]{xcsmethod}, preference is given to profiles measured from those spectra. However, if there is a problem with the annular spectra or the profile, we may instead use the 3000 count-binned profile. Such problems include:
\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
    \item The spectral fitting process failing to converge for some annuli. Even if only one annulus failed in this manner, the entire temperature profile is unusable.
    \item Annular temperature values have very poorly constrained uncertainties, this can make the deprojection process quite unstable, and cause problems when fitting a temperature profile model to the final 3D temperature profile.
    \item Model fits to the deprojected, three-dimensional, temperature profile resulting in unphysical mass profiles, where the hydrostatic mass radial profile is not monotonically increasing. 
\end{itemize}

This only applies to the newly measured masses for the SDSSRM-XCS sample, presented in Section~\ref{sec:results}; for the masses we measure for the LoCuSS High-\lx{} sample we attempt to match the original analysis by requiring a minimum of 3000 counts. We also indicate which temperature profile each of our masses originates from.

The number of annular bins varied from $N=4$ (the defined minimum) to $N=22$ for the clusters analysed herein. For our example clusters, it was $N=17$ and $N=4$ for \clustone{} and \clusttwo{} respectively.

Once the source and background regions have been defined, spectra are generated for every camera-plus-observation combination (and in each bin for the radial analysis) of the respective galaxy cluster.  

For our example clusters, \clustone{} and \clusttwo, this corresponds to 6 (132) and 6 (24) spectra respectively for the global (radial) analyses; the annular spectra for this example were generated with a minimum of 1500 counts.

\xga{} uses the \texttt{SAS} \texttt{evselect} tool to create the initial spectra, selecting events with a FLAG value of 0, and a PATTERN of ${\leq}4$ for PN and ${\leq}12$ for MOS data. The SAS \texttt{specgroup} tool is used to re-bin each spectrum so that there is minimum number of
counts per channel (in the analysis herein, we set that to be 5, though it can be configured by the user). 

The spectral analysis requires response curves (known as ancillary response files; ARFs) to proceed. These are calculated for each spectrum individually. For this, we use a detector map generated with {\tt x} and {\tt y} bin sizes set to 200 detector coordinate pixels, and with the same event selection criteria as the spectrum, as the detector map. We preferentially select an image from another instrument, if available, e.g. a PN image for a MOS detector map, and vice versa. This helps to mitigate the effects of chip gaps.

\xga{} uses \xspec{} \citep[][]{xspec} to fit emission models to the spectra. For the analyses herein\footnote{\xga{} can use a range of other emission models if the user prefers.}, we use an absorbed plasma emission model \citep[\texttt{constant${\times}$tbabs${\times}$apec;}][]{tbabs, apec}. The multiplicative factor represented by \texttt{constant} helps to account for the difference in normalisation between spectra being fitted simultaneously. The $\rm{n_H}$ values required by \texttt{tbabs} are retrieved using the HEASoft \texttt{nh} command\footnote{\cite{nh} data are used by the \texttt{nh} tool.}. The starting metal abundance value ($Z$) is defined by the user. For the analysis herein, $Z=0.3Z_\odot$ was used.
The redshift is always fixed at the input value during \xga{} fitting. The $\rm{n_H}$ and $Z$ value can be fixed or left free depending on the use case. For our example clusters, \clustone{} and \clusttwo{}, and the analysis in Section~\ref{sec:results}, they were fixed.

The fits are performed using the $c$-statistic \citep[][]{cash} using a methodology described in detail in \cite[][section 3]{xcsgiles}. Note that not all spectra will yield fitted parameters. There are several quality checks in the \cite{xcsgiles} method that have been replicated in \xga{}. If a given spectrum fails one of those checks, then it is removed from the analysis. If all spectra related to a given analysis region are removed in this way, then no spectral parameter fits will be reported by \xga{}.
Spectral fitting results for our two example clusters are shown in Figure~\ref{fig:projtemp}.
Validation tests of the \xga{} spectral fitting process can be found in Section~\ref{sec:validation}. 

%do we need to mention that the Tx's, errors, normalisation values are saved and used later?


%comment: KR more info about the spectral method. Maybe some of it needs to go back in? Initially, we reject any spectra that have fewer than 10 noticed channels. Next, each spectrum is fitted individually. If the measured temperature for a spectrum is $0.01~{\rm keV} \leq T_{\rm{X}} < \: $20~keV, or if the temperature uncertainty is greater than 15~keV, that spectrum is excluded from further analysis. Finally, we simultaneously fit the remaining spectra using a \texttt{constant*tbabs*apec} model.  The $T_{\rm{X}}$ and normalisation parameters of \texttt{apec} are tied across all models, the redshift is frozen at the input value, metallicity is frozen at 0.3~$Z_{\odot}$, nH is frozen at the value determined by \xga{}, and the constant factor for each spectrum is allowed to vary to account for differences in normalisation due to effective area. Temperatures and unabsorbed luminosities are determined from this simultaneous fit. For all fits, $T_{\rm{X}}$ is initially set to 3~keV, the normalisation is initially set to 1~cm$^{-5}$, and the constant is initially set to 1. All fits use the \texttt{angr} abundance table \citep[][]{andgrev}.

%Each \texttt{XSPEC} operation (i.e. a fit to global spectra for a cluster) will time out if it has not been successful within 4 hours. 
%comment: don't think (above) this is needed in the paper KR

%  Previous work by XCS ({\color{red} le references}) has measured these values using a luminosity-temperature (hereafter referred to as L-T) pipeline that iteratively generates spectra, fits them, measures temperature and luminosity, then uses that temperature to estimate R$_{500}$, and repeat until the results converge. The results presented in this work do not use the existing XCS pipeline, but rather use an equivalent functionality that has been built into XGA. The behaviour of our new implementation is largely the same as the original L-T pipeline, though subtle differences in software version, calibration files, location of the central coordinate, and how interloper sources are handled will cause slightly different results to be measured. For this work we measure temperatures within a region of radius R$_{500}$ and centred on the X-ray peak coordinates, we also measure unabsorbed luminosities in that same region, as well as core-excised luminosities in the {\color{red} 0.15-1R$_{500}$ region, which have been shown to have smaller scatter compared to global luminosities.}

% For this work, the measurements are derived from spectra centred on the X-ray peak as measured by XGA, with the peak position/outer radius (and inner radius for core-excised luminosity) converted to XMM detector coordinates. Equivalent position information for all interloper sources is used to exclude their corresponding events, and a source spectrum (within the chosen region) is generated for each instrument of each observation associated with that source. An ARF is calculated for that spectra, though the same RMF is used for all spectra generated from a particular ObsID-Instrument combination, as there is very little spatial variance that can be attributed to an RMF, and they relatively computationally expensive to create. We also group the spectra {\color{red} talk about the grouping parameters, as well as the rest of the SAS expression I forgot}

\begin{figure}
    \centering
    \includegraphics[width=1.\columnwidth]{images/demo_clusters_projtemp.pdf}
    \caption[projtemp profs]{Projected temperature profile measurements for the demonstration clusters, \clustone{} (blue; upper points) and \clusttwo{} (orange; lower points). Temperatures are plotted against the central radii of the annuli they were measured within. The global temperature values measured by \xga{} within $R_{500}$ for each cluster is indicated by horizontal lines, with the shaded region representing 1$\sigma$ uncertainty.}
    \label{fig:projtemp}
\end{figure}


%each annulus has simultaneous fits performed on all available data using the \texttt{constant*tbabs*apec} model. 

%The generated spectra are stored in instances of an \xga{} product class, \href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.spec.AnnularSpectra}{\texttt{AnnularSpectra}}, as are the fit results. 
%This class simplifies access to the data and is used by other parts of \xga{} to perform spectral fits and generate radially varying profiles of fit quantities, it also includes convenient methods for visualising the data. 


\subsection{Correcting images for PSF distortion}
\label{subsec:psfcorr}

The \xmm{} EPIC-PN on-axis PSF has a full width half maximum of ${\sim}12.5\arcsec$ \citep[][]{xmmhandbook}, and the EPIC-MOS1 and MOS2 camera on-axis PSFs have a FWHM of ${\sim}4.3\arcsec$. The PSF of all three EPIC cameras changes size and shape depending on the position on the detector, with the PSF causing stretching of bright sources along the azimuthal direction \citep[e.g.][]{readpsf,xmmhandbook}.
Therefore, \xga{} has been configured to make a PSF correction to \xmm{} images. These corrections are important to our goal of estimating $M_{\rm hydro}$ because the $\rho(r)$ profiles rely on surface brightness maps (see Section~\ref{subsec:SBandEm}). The PSF correction approach deployed in \xga{} uses the Richardson-Lucy algorithm \citep[][]{richardson,lucy} combined with the \texttt{ELLBETA}\footnote{\texttt{ELLBETA} \citep{readpsf} has been implemented in \texttt{SAS} via the \texttt{psfgen} tool.}  XMM PSF model. As the \xmm{} PSFs vary with position, the de-convolution is carried out separately in a user defined  grid across the image. For the analysis here in, we used a $10\times10$ grid. Figure~\ref{fig:demopsfcorr} shows a comparison of the pre and post PSF correction combined count-rate maps for our two example clusters. 

%For more details of the \xga{} PSF correction process, see {\color{red}XX (add github link}). 

\begin{figure*}
    \centering    
\includegraphics[width=1.0\textwidth]{images/demo_cluster_psfcorr.pdf}
    \caption[PSF comparison]{
    A demonstration of the image PSF correction capabilities of \xga{}. The white cross-hair indicates the UDC$^{\ref{foot:udc}}$ of \clustone{}. The white circle indicates the $R_{500}$ aperture centered on the UDC$^{\ref{foot:udc}}$. Both images show the $2R_{500}\times2R_{500}$ region. Left: the combined RateMap before PSF correction. 
    Right: After PSF correction. Note, the individual images were corrected separately, and then stacked.}
    \label{fig:demopsfcorr}
\end{figure*}


%comment: worth saying in Discussion: XGA only pipeline that does this for XMM in community?

%comment: some of the para below could be added back in KR
%Previous analyses \citep[e.g.,][]{croston,xxlbaryon} have accounted for this by constructing a mixing matrix that describes the shifting of photons between different radial bins by a 1D model of the PSF.  We have taken a different, generalised, approach to correcting for PSF effects. Rather than apply PSF corrections in 1D after the surface brightness profile has been created, we opt to correct the image itself, from which a profile will then be generated. This approach has several advantages when compared to the mixing matrix method. The primary benefit is the ability to correct in two dimensions, especially important for off-axis clusters (where the {\em XMM} PSF becomes highly non-symmetric). It also reduces the spread of any point sources that may be contaminating the cluster of interest, making them easier to fully remove from the observation with the \xga{} generated mask. Also, as images are PSF corrected without reference to a particular source, they can be used in many different types of analysis.

%comment: re stuff below: this stuff is too technical for the paper., so suggest it is put on github. But maybe it is appendix worthy? KR
% Then, for each chunk, the whole image is convolved with that PSF (this is to avoid edge effects caused by Fast Fourier Transform convolution), and then the chunk is cut out of the convolved image and stitched into a final, overall image. This convolution process is then iterated, until a final output image for each ObsID-Instrument combination associated with a source is generated (all correction in this work uses 15 iterations). Once individual PSF-corrected images are created, stacked PSF corrected images are created in the same way uncorrected stacked images are made (Section~\ref{subsec:xgaphot}). They are then divided by the existing stacked exposure maps to create PSF-corrected stacked count-rate maps. 

\subsection{Generating surface brightness and emissivity profiles}
\label{subsec:SBandEm}

\xga{} %\href{https://xga.readthedocs.io/en/latest/xga.imagetools.html\#xga.imagetools.profile.radial_brightness}{\texttt{radial\_brightness}} function 
can be used to construct radial surface brightness (SB) profiles from combined (Section~\ref{subsec:xgaphot}) PSF corrected (Section~\ref{subsec:psfcorr}) ratemaps. For this, the region (radius and centre) over which the SB is determined is defined by the user as an initiation input to \xga{} (Section~\ref{subsec:xcsdata}). A background region also needs to be defined. In \xga{}, the background region is an annulus. For our example clusters, \clustone{} and \clusttwo{} (and for the analysis presented in Section~\ref{sec:results}), the inner and outer radii are set at 1.05R$_{500}$ and 1.5R$_{500}$ respectively.
Other sources in the respective \xmm{} observation were removed prior to profile generation using the automated and  \xga{} generated masks (see Sections~\ref{subsec:xgacontam}, and \ref{subsec:manualdetreg}). For the analyses herein, we used the default \xga{} settings radial bins of width 1~pixel and an energy range of 0.5-2.0~keV. The uncertainties on the background-subtracted SB profile are calculated by assuming Poisson errors on the counts in each annulus.
Figure~\ref{fig:sbprof} shows cluster surface-brightness profiles for \clustone{} and \clusttwo{}. 

The SB profiles are projected quantities and in instrument specific units (i.e. detected photons per second per unit area).
The next step toward our goal of measuring a $\rho(r)$ profile is to de-project them and to infer a three-dimensional profile (i.e. emitted photons per second per volume). As the true 3D distribution of ICM electrons is unknown, we have to rely on a model for the de-projection. Fitting to radial profiles using \xga{} is described in Appendix~\ref{app:radmodfit}.  We use the double beta model throughout this work, but other models are available in \xga{} (see Table~\ref{tab:models}). An advantage of the double-beta model is that there is an analytical solution for the inverse-abel transform which is used to deproject it from a 2D to a 3D profile, making the assumption of spherical symmetry. This results in a 3D radial volume emissivity profile $\epsilon(R)$.


% This makes it both more computationally efficient



\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images/demo_clusters_sb.pdf}
    \caption[SB profile]{
    Surface brightness profiles (0.5-2.0~keV) generated by \xga{} for \clustone{} (blue; upper points) and \clusttwo{} (orange; lower points). Residuals to the fit to a beta model are shown in the bottom panel.}
    \label{fig:sbprof}
\end{figure}

\subsection{Generating density profiles}
\label{subsec:densityProf}

%start paragraph with E(r) and then introduce N to make it clearer

With the emissivity profiles in hand, the next task is to convert them to gas density profiles. For this we use of the definition of the APEC emission model normalisation,

\begin{equation}
    N_{\texttt{APEC}} = \dfrac{10^{-14}}{4\pi(D_{A}(1+z))^2}\int n_e n_p dV,
    %comment: should this be n_{+ve ions} since more than H matters
	\label{eq:apecnorm}
\end{equation}
where $N_{\texttt{APEC}}$ is the normalisation of the \texttt{APEC} plasma emission model (in units of $\rm{cm}^{-5}$), $D_{A}$ is the angular diameter distance to the cluster (in units of cm), $z$ is the redshift of the cluster, $n_{e}$ and $n_{p}$ are the electron and proton number densities (in units of $\rm{cm}^{-3}$). %This will help infer the gas density profile by enabling a conversion between the volume emissivity profile, $\epsilon(R)$, and the density profile.

To make use of Equation~\ref{eq:apecnorm}, we need to calculate a conversion factor, $K_N$, between $N_{\texttt{APEC}}$ and \xmm{} count-rate ($C_r$), where $N_{\texttt{APEC}} = K_N C_r$. To calculate $K_N$, we implement an \xga{} interface to the \xspec{} tool \texttt{FakeIt}, which can be used to simulate spectra given an emission model and an instrument response.  This is used to generate simulated spectra for every camera-plus-observation combination (using ARFs and RMFs generated at the UDC$^{\ref{foot:udc}}$ during the generation of spectra, see Section~\ref{subsec:xgaspecs}). The simulations are performed using an \texttt{APEC} model absorbed with \texttt{tbabs}. The nH value for \texttt{tbabs} is set to the \cite{nh} value for that cluster. The spectra are simulated with a normalisation fixed at 1, a fixed global temperature measured for that cluster (within $R_{500}$ for LoCuSS High-\lx{}/SDSSRM-XCS, within 300~kpc for XXL-100-GC), a metallicity of 0.3~$Z_{\odot}$, and the input redshift of the cluster. The simulated spectra are all `observed' for a set exposure time of 10~ks, and are used to measure count-rates in the 0.5-2.0~keV band, which corresponds to the energy range of the ratemaps used to generate SB profiles. The count-rates for each instrument of each observation are then weighted by the average effective area between 0.5-2.0~keV (drawn from the corresponding ARF) and combined into a single conversion factor $K_N$.
%by the \href{https://xga.readthedocs.io/en/latest/xga.sources.html\#xga.sources.extended.GalaxyCluster.norm_conv_factor}{\texttt{norm\_conv\_factor}} method of the \texttt{GalaxyCluster} class. 
This conversion factor is suitable for use with emissivity profiles generated from combined ratemaps.

This conversion factor, $K_N$, allows Equation~\ref{eq:apecnorm} to be written in terms of the 3D emissivity $\epsilon(R)={C_{r}(R)}{V}^{-1}$, and the product of the electron and hydrogen number densities $n_{e}n_{p}$ (which we can use to calculate the total gas density), 

\begin{equation}
    n_{e}(R)n_{p}(R) = \dfrac{4\pi K_{N}(D_{A}(1+z))^2C_{r}(R)}{10^{-14}V}.
    %comment: why use C(r)/V in this equation instead of sticking with E(r)? KR
	\label{eq:halfway}
\end{equation}

At this point we assume the ratio of electrons to protons in the intra-cluster medium, given by $n_{e}=R_{ep}\times n_{p}$, which substituted into Equation~\ref{eq:halfway}, gives an expression for $n_{p}$ of
\begin{equation}
    n_{p}(R) = \sqrt{\dfrac{4\pi K_{N}(D_{A}(1+z))^2C_{r}(R)}{R_{ep}10^{-14}V}}.
    %comment: why use C(r)/V in this equation instead of sticking with E(r)? KR
	\label{eq:np}
\end{equation}
We choose to use the solar abundances presented in \cite{andgrev} to calculate this ratio, $R_{ep}=1.199$.
The total gas number density, $n_{g} = n_{e}+n_{p} = (1+R_{ep})n_{p}$, is thus calculated using the expression for $n_{p}$ from Equation~\ref{eq:np}. 

At this point the mean molecular weight $\mu=0.61$ and the atomic mass unit are used to convert number density to mass density. Thus, we calculate gas density from emissivity with quantities that we can measure, or already know;

\begin{equation}
    \rho_{\rm{gas}}(R) = \mu m_{u}(1+R_{ep})\sqrt{\dfrac{4\pi K_{N}\epsilon(R)(D_{A}(1+z))^2}{R_{ep}10^{-14}}}.
	\label{eq:dens}
\end{equation}

Once gas density is measured using Equation~\ref{eq:dens}, we could use the fitting functionality discussed in Appendix~\ref{app:radmodfit} to fit a parametric model to the resulting data points. However, as the density points are themselves generated from a model fit (the double-$\beta$ model, see Table~\ref{tab:models}), and that model has an analytical solution to the inverse-Abel deprojection, we choose to calculate deprojected parameter posterior distributions. This is more computationally efficient than fitting another profile, and better propagates the errors on the surface-brightness profile to the density profile. Density profiles for SDSSXCS-55 and SDSSXCS-6955 are shown in Figure~\ref{fig:densprof}.

%it is stored in a \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.GasDensity3D}{GasDensity3D}} instance. We 

\subsection{Measuring gas masses}
\label{subsec:measgasmass}

Once a gas density profile (Equation~\ref{eq:dens}) has been derived, we can use it to measure total gas masses within given radii. This is achieved through a spherical volume integral, 
\begin{equation}
    M_{\rm{gas}}(<R_{\Delta}) = 4\pi \int_{0}^{R_{\Delta}} \rho_{\rm{gas}}(R)R^2 dR,
	\label{eq:volint}
\end{equation}
and can be used to measure both total gas masses within particular radii (e.g. $R_{500}$), or to create cumulative gas mass profiles.
%(we do not use those in this work).

It is desirable to account for all significant sources of uncertainty in the calculation of gas masses.  One source of uncertainty is that on the overdensity radii within which gas mass is measured, which is not accounted for in our measurement of the density profile. Therefore, we have added an optional mechanism to account for uncertainty in the physical radius (e.g. $R_{500}$) when calculating gas mass. For this, we assume a  Gaussian posterior distribution for the radius, with the mean being the published value and the standard deviation being the published error. This radius distribution is sampled along with the model posterior distributions to create a gas mass measurement distribution, with the sampled radius for each combination of sampled model parameters acting as the outer radius within which the integral is evaluated. We have applied this method in Section~\ref{subsec:compgasmasses} where we compare \xga{} and \cite{xxlbaryon} gas mass estimates for the XXL-100-GC sample.  This is due to the fact that the gas masses measured in \cite{xxlbaryon} also account for overdensity radius uncertainty in their analysis.  We also use it in Section~\ref{sec:results} when generating new $M_{\rm{hydro}}$ estimates for SDSSRM-XCS clusters. 

To demonstrate the effect of including the uncertainty on the input radius, the measured gas mass for \clusttwo{} within $R_{500}$ ($669.0^{+62.0}_{-47.9}$ kpc; see Table~\ref{tab:exampclusters}) is $M^{\rm{gas}}_{500}= 1.155^{+0.027}_{-0.027}$ $10^{12}\: \rm{M}_{\odot}$ excluding the uncertainty on $R_{500}$, and $M^{\rm{gas}}_{500}= 1.153^{+0.089}_{-0.095}$ $10^{12}\: \rm{M}_{\odot}$ including the $R_{500}$ uncertainty. We can see that the gas mass uncertainties, when we account for radius uncertainty, are ${\sim}3$ times larger than when we don't.

\begin{figure}
    \centering \includegraphics[width=1.0\columnwidth]{images/demo_clusters_dens.pdf}
    \caption[rho profile]{Gas density models generated by \xga{} for \clustone{} (blue) and \clusttwo{} (orange). These are determined from the model fits to surface-brightness profiles shown in Figure~\ref{fig:sbprof}.}
    \label{fig:densprof}
\end{figure}


\subsection{Generating 3D temperature profiles}
\label{subsec:gastempprof}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images/demo_clusters_3dtemp.pdf}
    \caption[3D T profile]{Fitted three-dimensional temperature profile  for \clustone{} (blue; the higher temperature data points and model) and \clusttwo{} (orange; the lower temperature data points and model). Residuals to the fit to a simplified Vikhlinin model are shown in the bottom panel. 
    These temperature profiles were generated by deprojecting the temperature profiles shown in  Figure~\ref{fig:projtemp}.} 
    \label{fig:3dtempprof}
\end{figure}


%comment: refer back to initial equation
The second property we must measure to calculate a cluster's hydrostatic mass is the three-dimensional temperature profile. 
%\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.spec.AnnularSpectra}{\texttt{AnnularSpectra}} instance, 
The radial spectral analysis described in Section~\ref{subsec:xgaspecs} results in a set of projected temperature measurements (one for each of the $N$ radial bins).
%{\color{red} stored in an \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.ProjectedGasTemperature1D}{ProjectedGasTemperature1D}} instance.}
Each projected temperature is a weighted combination of the temperatures in the three-dimensional shells of the cluster that the annulus intersects with. To recover the 3D distribution, $T(r)$, we opt to use the `onion-peeling' method \citep[see descriptions in e.g.,][]{onion1,onion2}. First, the volume intersections between the analysis annuli (projected back into the sky) and the spherical shells which we separate each cluster into (defined as having the same radii as the annuli) must be calculated. The volume intersections can be calculated  \citep[see Appendix A of][]{volintersec} as, 

\begin{equation}
\begin{split}
%comment:  is this needed? could be in github info since just (?) quoting from the McLaughlin paper KR
    \bm{V}_{\rm{int}} = \frac{4\pi}{3}\big[&max\{0, (\bm{R}_{\rm{so}}^{2} -  \bm{R}_{\rm{ao}}^{2})^{\frac{3}{2}}\} - max\{0, (\bm{R}_{\rm{so}}^{2} - \bm{R}_{\rm{ao}}^{2})^{\frac{3}{2}}\} +\\ & max\{0, (\bm{R}_{\rm{si}}^{2} - \bm{R}_{\rm{ao}}^{2})^{\frac{3}{2}}\} - max\{0, (\bm{R}_{\rm{si}}^{2} - \bm{R}_{\rm{ai}}^{2})^{\frac{3}{2}}\} \big],
\end{split}
\label{eq:intersec}
\end{equation}
where $\bm{R}_{\rm{so}}$ is the matrix of shell outer radii, $\bm{R}_{\rm{ao}}$ is the matrix of annulus outer radii, $\bm{R}_{\rm{si}}$ is the matrix of shell inner radii, and $\bm{R}_{\rm{ai}}$ is the matrix of annulus inner radii. 
%The calculation is implemented in the \xga{} function \href{https://github.com/DavidT3/XGA/blob/d8709eb1a0eb297f39ac50d4c4d9f1ad7122f9f0/xga/sourcetools/deproj.py\#L10}{\texttt{shell\_ann\_vol\_intersect}}. 
The $\bm{V}_{\rm{int}}$ matrix is a two dimensional matrix describing volume intersections between all combinations of annuli and three-dimensional shells.

% 

% \begin{equation}
%     \bm{V}_{\rm{int}} = \frac{4\pi}{3}(R_{\rm{out}}^{2} - R_{\rm{inn}}^{2})^{\frac{3}{2}},
% 	\label{eq:intersec}
% \end{equation}

Second, an emission measure profile 
%(\texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.EmissionMeasure1D}{EmissionMeasure1D}}) 
is calculated using the 
%\texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.APECNormalisation1D.emission_measure_profile}{emission\_measure\_profile}} method of the \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.APECNormalisation1D}{APECNormalisation1D}} 
APEC Normalisation 1D profile produced during the spectral fitting of the set of annular spectra. This calculation uses Equation~\ref{eq:apecnorm} and rearranges to solve for the integral. As the projected temperature measured within a given annulus is a weighted combination of the shell temperatures intersected by that annulus, we can infer the temperature of a shell \citep[for past usage see][]{onion2} with 

\begin{equation}
    \bm{T}_{\rm{shell}} = \dfrac{(\bm{V}_{\rm{int}}^{\rm{T}})^{-1} \times \bm{T}_{\rm{annulus}}\rm{\textbf{EM}}}{(\bm{V}_{\rm{int}}^{\rm{T}})^{-1} \times \rm{\textbf{EM}}}.
	\label{eq:tempdeproj}
\end{equation}

$\bm{T}_{\rm{shell}}$ is the matrix of spherical shell temperatures that we aim to calculate, $\bm{V}_{\rm{int}}$ is the matrix of volume intersections between all combinations of annuli and shells (see Equation~\ref{eq:intersec}), $\rm{\textbf{EM}}$ is the emission measure matrix, and $\bm{T}_{\rm{annulus}}$ is the projected temperature matrix; $\times$ represents the matrix product.
We propagate the uncertainties from the projected temperature and emission measure profiles by generating 10000 realisations of each profile, assuming gaussian errors on each data point. We then use the profile realisations to calculate 10000 instances of the deprojected temperature profile. These distributions are used to measure 90\% confidence limits on each deprojected temperature data point. 

% Once calculated, the $\bm{T}_{\rm{shell}}$ values and uncertainties are stored in a \texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.GasTemperature3D}{GasTemperature3D}} instance. 

Once three-dimensional, de-projected, gas temperature profiles have been measured, we use the methods discussed in Section~\ref{app:radmodfit} to model the profiles with the simplified Vikhlinin temperature model
%comment: justify this choice KR
(see Table~\ref{tab:models} for more information). 
Figure~\ref{fig:3dtempprof} shows three-dimensional temperature profiles for clusters \clustone{} and \clusttwo{}, along with the corresponding 1$\sigma$ uncertainty (given by the shaded regions).


\subsection{Generating hydrostatic mass profiles}
\label{subsec:hydromassprof}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images/demo_clusters_hym.pdf}
    \caption[Hmas profile]{An example hydrostatic mass profile generated for \clustone{}. This profile was generated using the model fits to the density profile shown in Figure~\ref{fig:densprof}, and the temperature profile shown in Figure~\ref{fig:3dtempprof}.}
    \label{fig:hymprof}
\end{figure}


Once we have measured a 3D radial density profile (details in Section~\ref{subsec:densityProf}) and a 3D radial temperature profile (details in Section~\ref{subsec:gastempprof}), we can use Equation~\ref{eq:hydromass} to measure hydrostatic masses. As such, \xga{} creates hydrostatic mass profiles as a function of radius (e.g. Figure~\ref{fig:hymprof}).
%, which are stored in 

%\texttt{\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.HydrostaticMass}{HydrostaticMass}} class instances. 
%The density and temperature profiles must have models fitted prior to the construction of a hydrostatic mass profile, with the fitting process described in Section~\ref{app:radmodfit} and models described in Table~\ref{tab:models}. 
The hydrostatic mass equation not only involves the temperature and density profile values at each radius for which a enclosed mass is measured, but also the derivatives of those profiles with respect to radius. The double-king profile and temperature profiles both have analytical first-derivatives, and as such these are used to calculate the slope at a given radius, rather than a numerical approximation. 

\xga{} models can return posterior distributions of the value of the model (or model slope) at a given radius, rather than a single value. This is based on drawing randomly from the parameter posterior distributions found from the fitting process described in Section~\ref{app:radmodfit}. When calculating a hydrostatic mass at a specified radius, the temperature and density parametric models generate 10000 realisations of themselves; these realisations are then used to retrieve absolute values of $T_{\rm{3D}}$ and $\rho_{\rm{g}}$ at the specified radius, as well as $\frac{dT_{\rm{3D}}}{dr}$ and $\frac{d\rho_{\rm{g}}}{dr}$ values. As such a distribution of hydrostatic mass measurements is created for the given radius, and 90\% confidence limits are calculated.

We also implement an optional method of propagating errors on the chosen radius, to help account for uncertainties on the overdensity radii which masses are commonly calculated within. This is akin to the optional step implemented for the calculation of \xga{} gas masses at the end of Section~\ref{subsec:measgasmass}. When an uncertainty is provided along with a radius, we assume a Gaussian distribution and draw 10000 random radii. Then, when the profile realisations are generated and a distribution of hydrostatic masses are measured, the randomly drawn radii are used rather than a fixed value.  Distributions are generated for absolute values and derivatives can all take radius uncertainties into account. This is not used in our comparisons to LoCuSS $M_{\rm{hydro}}$ measurements in Section~\ref{subsec:mhydrocomp}, as radius uncertainties were not published by \cite{locusshydro}. We do include radius uncertainties in our calculation of SDSSRM-XCS cluster masses presented in Section~\ref{sec:results}.
Mass profiles for the clusters \clustone{} and \clusttwo{}, along with the corresponding 1$\sigma$ uncertainty (given by the shaded regions), are shown in Figure~\ref{fig:hymprof}.

% {\color{red} example images need to be added}

% Due to the many steps involved in the automated process of getting to a $M_{hydro}(<r)$ result using \xga{}, it is important to carry out sanity checks on the outputs.
% %To ensure that the masses measured are valid, visual inspection of key data products is performed. This expands upon the visual inspection and region adjustment that was described in Section~\ref{subsec:manualdetreg}. 
% Therefore, profile-based products that contribute to the measurement of the hydrostatic mass i.e., $\rho_{\rm gas}(r)$, $T(r)$ and $M_{hydro}(r)$ profiles, are visually inspected.  These inspections identify cases where (i) the surface brightness  profile has been poorly described by the double beta model (in the SDSSRM-XCS analysis, XX clusters removed at this step), (ii) the temperature profiles 
% %very poorly constrained data points, or 
% with unphysical attributes, such as temperature increasing in the outskirts of a cluster (XX SDSSRM-XCS clusters removed at this step), or (iii) mass profiles that do not monotonically increase (XX SDSSRM-XCS clusters removed at this step). {\color{red}Neither \clustone{} nor \clusttwo{}, show these traits, so we have included additional examples in Figure~\ref{makethisplot}. 
%  PUT EXAMPLES IN APPENDIX SECTION?}.

%The \texttt{HydrostaticMass} class provides a method (\href{https://xga.readthedocs.io/en/latest/xga.products.html\#xga.products.profile.HydrostaticMass.diagnostic_view}{diagnostic\_view}) to generate a set of visualisations (a combination of Figures~\ref{fig:sbdensprof}, \ref{fig:tempprof}, and \ref{fig:hymprof}) for each cluster.



==> OldSections/OldSections30Jan2024/ResultsSDSSsection.tex <==

%\section{New Masses and scaling relations}
\section{Mass analysis of the SDSSRM-XCS sample}
%comment:  It would be ironic, but have we inadvertently introduced some miscentering effect of our own by not re-measuring richness around the X-ray centre
\label{sec:results}
Here we present hydrostatic masses for a subset of galaxy clusters in the SDSSRM-XCS sample presented by \cite{xcsgiles}.  

\subsection{Masses for a subset of the SDSSRM-XCS sample}
\label{subsec:newmasses}

We attempt to measure masses for all 150 galaxy clusters in the SDSSRM-XCS sample.  Measurements presented in this section are performed using \xga{}, within the $R_{500}$ and $R_{2500}$ values measured by G22. In Section~\ref{subsubsec:txtests} we demonstrated that the global \xga{} \tx{} measurements are consistent with the original G22 analysis when measured within identical apertures (see Fig.~\ref{fig:xcstempcomp}). 

%We do not expect to be able to measure masses for all of these clusters, as measuring temperature profiles requires significant X-ray counts, but we shall attempt measurements using \xga{}'s automated routines. This will demonstrate its robustness and ability to deal with failed measurements.

Temperature and density profiles were generated out to $R_{500}$ (from G22), with the hydrostatic masses estimated from these profiles at $R_{500}$ and $R_{2500}$. Density profiles were generated as described in Section~\ref{subsec:densityProf}. The temperature profile annuli are chosen so that each annuli has a minimum width of 20\arcsec and a minimum number of background subtracted counts per annulus of 1500. The minimum counts check is performed on the combined data for all relevant observations of a cluster.  %\xga{} enforces a minimum of 4 annuli, so annuli with signal to noises lower than {\color{red}} are possible. 
%comment: Has all this not been said before? PG

We are able to successfully measure hydrostatic masses for 102 of the 150 galaxy clusters in the SDSSRM-XCS sample. The temperature profiles used for these measurements have between 4 (the minimum number allowed, see Section~\ref{subsec:xgaspecs}) 
and 26 annuli. We perform visual examination of relevant data products for each cluster, as described in Section~\ref{subsec:dataverif}. This process flags any suspect or nonphysical results, and allows us to perform a deeper inspection and determine why a particular result has been measured.

This set of hydrostatic masses adds significant value to the SDSSRM-XCS sample, as well as representing one of the largest samples of cluster hydrostatic masses available. As each mass is measured individually, rather than derived through the stacking of different clusters (as is usually the case for weak lensing cluster masses), there are many possible uses for the sample. Also, as SDSSRM-XCS clusters were selected from optical/NIR via the SDSS redMaPPer catalogue \citep[][]{redmappersdss}, this sample allows for powerful multi-wavelength studies of how cluster mass is related to optical properties.

% \textcolor{cyan}{How about we move 4.1 to the end of section 3, so that becomes Section 3.5, and then we add a section 3.5.1 which includes the comparisons to existing lit hydro masses?  Putting plot here for now}.

\subsection{Comparison of SDSSRM-XCS masses with the literature}
\label{subsec:sdssrm_hydro_comp}

Here we compare the masses estimated for the SDSSRM-XCS sample in Section~\ref{subsec:newmasses} to values taken from the literature.  We compare the M$^{500}_{\rm hy}$ values to those given in \cite{locusshydro}, \cite{lovisarimasses} and \cite{2023MNRAS.520.6001P}.  The \cite{locusshydro} masses are from the LoCuSS sample as discussed in Section~\ref{subsec:samples}.  The \cite{lovisarimasses} sample contains 120 {\em XMM} derived hydrostatic masses from {\em Planck} detected clusters (spanning a redshift range of $0.059 < z < 0.546$).  Finally, \cite{2023MNRAS.520.6001P} estimate hydrostatic masses using {\em XMM} for 19 clusters contained in the Meta-Catalog of X-Ray Detected Clusters of Galaxies \citep[][]{mcxc_sample} within the Hyper Suprime-Cam Subaru Strategic Programme field \citep[][]{HSC_SSP}.  The \textcolor{red}{102}  SDSSRM-XCS clusters with M$^{500}_{\rm hy}$ values are matched to the samples of clusters used in the works listed, resulting in 21, 16 and 9 clusters matched to \cite{locusshydro}, \cite{lovisarimasses} and \cite{2023MNRAS.520.6001P} respectively.  The comparison of the masses is plotted in Figure~\ref{fig:sdssrm_mass_comp}(a).  The black line represents the 1:1 relation, highlighting a broad consistency of the masses measured in this work and those reported in the literature.

In Figure~\ref{fig:sdssrm_mass_comp} (b), we show the number of SDSSRM-XCS clusters per M$^{500}_{\rm hy}$ bin (given by the blue histogram).  The M$^{500}_{\rm hy}$ distributions from \cite{locusshydro} and \cite{lovisarimasses} are given by the brown and green spline curves respectively.  While the SDSSRM-XCS sample clearly contains more masses than the \cite{locusshydro} sample, clusters in \cite{locusshydro} are selected by imposing a luminosity limit on clusters detected in the RASS, reducing the number of available clusters for study.  The \cite{lovisarimasses} sample contains a larger number of masses overall, the SDSSRM-XCS sample provides many more low-mass cluster estimates.  However, we note that this is likely due to the {\em Planck} selection of the clusters in \cite{lovisarimasses}, which will select higher mass clusters.  Additionally, \cite{lovisarimasses} provide masses for 17 clusters for which their masses were estimated using $<$4 temperature profile bins.  For the analysis of the SDSSXCS-RM sample, we required a minimum of 4 bins in the temperature profile for a mass determination.

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/sdssrm_mass_comp.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/mass_histogram.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[mass comparison]{(a) A one-to-one comparison of hydrostatic masses measured for the SDSSRM-XCS cluster sample using \xga{}, compared to \citet[][brown diamonds]{locusshydro}, \citet[][green triangles]{lovisarimasses} and \citet[][cyan crosses]{2023MNRAS.520.6001P}. (b) Mass distribution of the 102 SDSSRM-XCS clusters with M$^{500}_{\rm hy}$ values (lightblue histogram).  Mass distributions from \citet[][brown histogram, using only the {\em XMM} based masses]{locusshydro} and \citet[][green]{lovisarimasses} are given for comparison.}
    \label{fig:sdssrm_mass_comp}
\end{figure*}




==> OldSections/OldSections30Jan2024/ValidationSection.tex <==

\section{Validation Tests}
\label{sec:validation}

We have tested the validity of the \xga{} approach described in Section~\ref{sec:methodology} by comparing the \xga{} outputs to those presented in the literature. For this we have used three different cluster samples. The samples used for validation are  described in Section~\ref{subsec:samples}. In Sections~\ref{subsubsec:txtests}, \ref{subsec:compgasmasses}, \ref{subsec:mhydrocomp} we compare the \xga{} measurements of $T_{\rm X}$, $M_{\rm{gas}}$, $M_{\rm{hydro}}$ respectively to literature values. 



%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/samps_prop_dists.pdf}
%    \caption[Sample Historgrams]{Published properties of the samples re-analysed here in and described in Table~\ref{tab:samplesummary}. X-ray properties presented in this figure have been measured in different regions, indicated in the legend of each plot. 
    %comment: maybe switch to a definition of the terms, e.g. _500 means... KR
 %   a) global X-ray  temperature, b) redshift, 
    %from spectroscopic follow-up 
    %comment:  not needed, we are taking the info from the publication KR |  might be worth mentioning RM redshifts in the new results section though KR
    %(XXL-100-GC), from the RASS catalogues the sample was selected from (LoCuSS High-\lx{}), and from the redMaPPer cluster finder (SDSSRM-XCS) c) bolometric X-ray luminosities. taken from literature, measured within $R_{500}$ (LoCuSS High-\lx{} and SDSSRM-XCS) and 300~kpc (XXL-100-GC)
%}
%    \label{fig:samp_sum}
%\end{figure*}

%%Taken out of table description as we are no longer publishing extra locuss clusters
%\newline $^{\ddagger}$ In Table~\ref{tab:locussmeasurements}, we present \xga{} $T_{\rm X}$ values for an additional \extraLOCUSSTx{} clusters observed with \xmm{} since \cite{locusshydro} was published.

\begin{table*}
\centering
\caption[]{{The published galaxy cluster samples used to validate the \xga{} methodology. We use the sample names in this table to refer to the samples throughout this work, and provide a summary of each sample, as well as the number of clusters.}
\label{tab:samplesummary}
}
\vspace{1mm}

%In addition to a comparison to the \xmm{} derived properties of {\color{red} 32XX} LoCuSS clusters presented in (add refXX),

\begin{tabular}{|ll| p{0.4\linewidth} | p{0.30\linewidth}}
% \begin{tabular}{l|lc}
\hline
\hline
 Sample Name & N$_{\rm{CL}}$, $z$ & Brief description\\ 
\hline
\hline
SDSSRM-XCS & 
150, $0.1{<}z{<}0.35$ 
& 
SDSS redMaPPer clusters \citep[][]{redmappersdss} with available \xmm{} observations. Section~\ref{sec:validation} presents a comparison to results presented in \cite{xcsgiles}.
%with $\Delta T_{\rm{X}}$<25\% 
%more needed to explain XMM connection
%& Ensuring \xga{} $L_{\rm{X}}$ and $T_{\rm{X}}$ measurements are consistent with existing XCS results. New measurements of masses of this sample are presented.
\\
\hline
XXL-100-GC & 99, {$0.05<z<0.9$} & Drawn from a sample of the 100  X-ray brightest clusters in the XXL survey regions \citep[][]{xxl1,gc100}.
Section~\ref{sec:validation} presents a comparison to results presented in \cite{xxllt} and \cite{xxlbaryon}.
%& Testing whether \xga{} $L_{\rm{X}}$, $T_{\rm{X}}$, and $M_{\rm{gas}}$ measurements are consistent with external results.
\\
\hline
LoCuSS High-$L_{\rm{X}}$ (a) & 33, $0.15<z<0.3$ & Drawn from clusters detected in the the ROSAT All Sky Survey \citep{rass_ebeling}.  The sample contains 50 clusters satisfying the following conditions; $n_{H}<7\times10^{20}$~cm$^{2}$, $-25^{\circ} < \delta < 65^{\circ}$ and $L_{X}[0.1 - 2.4~{\rm keV}]E(z)^{-2.7} \geq 4.2\times10^{44}$ erg s$^{-1}$.  All clusters have subsequent observations by \xmm{} or \chandra{}. Section~\ref{sec:validation} presents a comparison to 33 clusters with \xmm{} derived results presented in \cite{locusshydro}.
%& Testing whether \xga{} $L_{\rm{X}}$ and $T_{\rm{X}}$ (global and core-excised) and $M_{\rm{gas}}$ and $M_{\rm{hy}}$ measurements are consistent with external results.
\\
LoCuSS High-$L_{\rm{X}}$ (b) & 32, $0.15<z<0.3$ & As above, but for clusters satisfying $L_{X}[0.1 - 2.4~{\rm keV}]E(z)^{-1} \geq 4.4\times10^{44}$ erg s$^{-1}$ between $0.15 < z < 0.24$, and $L_{X}[0.1 - 2.4~{\rm keV}]E(z)^{-1} \geq 7.0\times10^{44}$ erg s$^{-1}$ between $0.24 < z < 0.3$.  Resulting in a sample of 41 clusters. Section~\ref{sec:validation} presents a comparison to 32 clusters with \xmm{} derived results presented in \cite{locusstemps}.
\\
\hline
\end{tabular}
\end{table*}

\subsection{Validation Samples}
\label{subsec:samples}
%comment: add the description of the samples - or is this in intro? KR

%comment: this paragraph needs to go in, but somewhere else KR
%The SDSSRM-XCS sample contains 99 (66\%) objects with at least one on-axis observation, the XXL-100-GC sample contains 33 (34\%; lower because of the contiguous survey nature of XXL), and LoCuSS High-$L_{\rm{X}}$ 43 (96\%). Our final analysis of the three samples makes use of ${\sim}400$ unique \xmm{} observations, not including observations that were removed due to data quality issues.

The validation samples are SDSSRM-XCS \citep{xcsgiles}, XXL-100-GC \citep[][]{gc100}, and LoCuSS High-$L_{\rm{X}}$ \citep{locusshydro}. The properties of the validation samples are summarised in Table~\ref{tab:samplesummary}. We note that although both \xmm{} and \chandra{} based measurements are presented in \cite{locusshydro},
%comment: and in Mulroy? KR
we only make comparisons herein with \xmm{}, because there is a known discrepancy between \xmm{} and \chandra{} derived  temperature estimates \cite[e.g.,][]{schellenbergertcal}. Excluding duplicates,
a total of 268 clusters have been used in the validation tests. Duplicate clusters were identified by cross-matching the samples; to be considered a match, two sources needed to be within a projected distance of 500~kpc (at the cluster redshift) and with $\lvert\Delta z\rvert \leq 0.05$. For each test, we adjusted the \xga{} initiation values (Section~\ref{subsec:xcsdata}) to follow those used in the published works as closely as possible (see Sections~\ref{subsubsec:SDSSRMsim}, \ref{subsubsec:XXLsim}, \ref{subsubsec:LoCuSSsim}).
A companion GitHub repository (see Appendix~\ref{app:companionrepo} for a summary of the structure and contents) contains the exact sample files used in this section. 

%XCS and LoCuSS samples (\S?? and ??), and $\Omega_{\rm{M}}$=0.282, $\Omega_{\Lambda}$=0.719, and, for the XXL sample (\S??), $H_{0}$=69.7 km s$^{-1}$ Mpc$^{-1}$ \citep[i.e. the WMAP9 values in ][]{wmap9cosmo}.  In Section \ref{sec:results}, we again use $\Omega_{\rm{M}}$=0.3, $\Omega_{\Lambda}$=0.7, and $\rm{H}_{0}$=70 km s$^{-1}$ Mpc$^{-1}$.


\subsubsection{SDSSRM-XCS}
\label{subsubsec:SDSSRMsim}

We have used \xga{} to re-analyse a sample of 150 clusters presented in \citep[][hereafter G22]{xcsgiles}. These clusters are referred to as the SDSSRM-XCS$T_{\rm X,vol}$ sub-sample in G22 (see Table 2 therein), but hereafter will be referred to as SDSSRM-XCS for simplicity. The SDSSRM-XCS clusters in the sample were originally selected from SDSS photometry using the redMaPPer (RM) algorithm \citep[][]{redmappersdss}. The 150 SDSSRM-XCS clusters represent the subset of the original $\simeq$66,000 SDSSRM cluster catalogue, that meet the following criteria: they lie within the footprint of the the \xmm{} archive, were successfully processed by the XCS imaging anf spectroscopic pipelines ($\Delta T_{\rm X}<25\%$), and have redshifts in the range $0.1<z<0.35$. 

Our analysis of the SDSSRM-XCS clusters included these elements in common with G22:


\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
\item[$\bullet$] The cosmological model; flat $\Lambda$CDM, assuming $\Omega_{\rm{M}}$=0.3, $\Omega_{\Lambda}$=0.7, and $\rm{H}_{0}$=70 km s$^{-1}$ Mpc$^{-1}$.  
% \item[$\bullet$] The input \xmm{} observations. Even though \xmm{} observations are added to the public archive on a regular basis, {\color{red} no new, compared to G22, observations were used in the validation tests.} In total {\color{red}\sdssrmobsids} were used.
\item[$\bullet$] The \xmm{} data reduction, image generation, and source detection
%comment: and calibration? KR
(Section~\ref{subsec:xcsdata}).
%comment: correct? needs better explanation KR
This was performed outside of \xga{}, exactly following the G22 approach. 
%comment: is the same? is it? did we use all observations? KR
This meant that the automatically masked regions (Section~\ref{subsec:xgacontam})  were the same in both analyses. 
\item[$\bullet$] The UDCs$^{\ref{foot:udc}}$, redshifts, $R_{500}$, and $R_{2500}$ values. Therefore, the source apertures, and the background annuli (either 1.05-1.5$R_{500}$ or 2-3$R_{2500}$) were the same (i.e. size, shape, and location) during the global spectral fits (\S\ref{subsec:xgaspecs}), and construction of surface brightness profiles (\S\ref{subsec:SBandEm}).
\item[$\bullet$] The model used during the \xspec{} fits. Both analyses used an absorbed APEC plasma model with the column density, redshift, and metal abundance fixed during the fit. 
%Where nH came from.... and Z was fixed at ....
\end{itemize}

%\setlength{\parindent}{0pt}
Differences include:

\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
\item[$\bullet$] The choice of manually adjusted source masks and excluded \xmm{} 
observations (Section~\ref{subsec:manualdetreg}).
%comment: this contradicts what we say above about using exactly the same OBSids, so maybe brush over it? KR
\item[$\bullet$] Different versions of certain software packages; G22 used SAS v14.0.0 and \xspec{} v12.10.1f, whereas this work uses SAS {v18.0.0} and  \xspec{} {v12.11.0}.
\item[$\bullet$] The pipeline used for the global spectral analysis (there was no radial spectral analysis G22). Herein we use \xga{}, whereas G22 used XCS3P. One important difference between the two pipelines is the treatment of \xmm{} sub-exposures. Some \xmm{} observations contain multiple sub-exposures by the same instruments. The analyses performed by \xga{} only make use of the longest individual sub-exposure for a particular instrument of a particular observation, whereas XCS3P makes use of all of the sub-exposures. 
%comment: is XCS3P explained in Intro? If so, do section ref. If not, we need to do that here. KR.
\end{itemize}

\subsubsection{XXL-100-GC}
\label{subsubsec:XXLsim}

We have used \xga{} to re-analyse 99 of the 100 clusters first described in \cite{gc100}. (We did not include XLSSC-504 because it was excluded from the \cite{xxllt} study.) Two of the 99 did not successfully pass the \xga{} data checks, and so are not included in the comparison:  \texttt{backscale} errors were encountered during spectral generation for XLSSC-11, and, for  XLSSC-527, no observation fulfils the \xga{} criterion that the 300~kpc coverage (\S~\ref{subsec:xcsdata}) fraction should be $>70\%$. We compare the \xga{} derived global temperature measurements of the remaining 97 to those presented in 
\cite{xxllt}\footnote{\href{http://vizier.u-strasbg.fr/viz-bin/VizieR-3?-source=IX/49/xxl100gc}{http://vizier.u-strasbg.fr/viz-bin/VizieR-3?-source=IX/49/xxl100gc}}, and the \xga{} derived gas mass measurements to those presented in \cite{xxlbaryon}\footnote{One part of the XXL-100-GC sample information is not retrieved from the VizieR catalogue, the uncertainties on $R_{500}$ values. These are used in Section~\ref{subsec:compgasmasses}, and are only available in \cite{xxlbaryon}.}. 

Our analysis of the XXL-100-GC clusters included these elements in common with the published works:

\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
\item[$\bullet$] The cosmological model: $\Omega_{\rm{M}}$=0.28, $\Omega_{\Lambda}$=0.72, and $H_{0}$=70 km s$^{-1}$ Mpc$^{-1}$, the WMAP9 results \citep[][]{wmap9cosmo}.
% (H0 =70 km s−1 Mpc−1, Ωm = 0.28, ΩΛ = 0.72, Ωb = 0.046, σ8 =0.82, ns = 0.965). [quote from XXL paper]
\item[$\bullet$] The UDCs$^{\ref{foot:udc}}$, redshifts, and analysis regions ($r=300$~kpc) of the clusters. Therefore, the source apertures were the same (i.e. size, shape, and location) during the global spectral fits (\S\ref{subsec:xgaspecs}), and construction of surface brightness (SB) profiles (\S\ref{subsec:SBandEm}) of both analyses. 
\item[$\bullet$] The model used during the \xspec{} fits was the same. Both analyses used an absorbed APEC plasma model with the column density, redshift, and metal abundance fixed (at 0.3~$Z_{\odot}$, using  \cite{andgrev} abundance tables) during the fit. 
\item[$\bullet$] A fixed metallicity of 0.3~$Z_{\odot}$, and the \cite{andgrev} abundance tables.
\item [$\bullet$] \xspec{} fitting within an energy range of 0.4-7.0~keV.
\item [$\bullet$] Surface brightness profiles were derived from images generated in the 0.5–2.0keV energy band.
\item [$\bullet$] Surface brightness profiles are generated out to $1.2R_{500}$.
\item[$\bullet$] The global temperature value from \citet[][$T_{\rm{X}}^{300\rm{kpc}}$]{xxllt} was used for the conversion from SB to emission measure (see Section~\ref{subsec:SBandEm}).
\item [$\bullet$] $M_{\rm gas}$ values, and errors, were estimated within R$_{500}$ taken from \cite{xxlbaryon}.  Additionally, $M_{\rm gas}$ uncertainties include the error on R$_{500}$ as performed in \cite{xxlbaryon}, see Section~\ref{subsec:measgasmass}.

% \xga{} uses \cite{nh} values; they have been shown to be consistent\footnote{\label{footnote:nh}\href{https://heasarc.gsfc.nasa.gov/Tools/w3nh_comp.html}{Comparisons of nH from different analyses}}.
%quote from XXl Pacuad16: All conversion from luminosities to count rates or fluxes in this paper use an average nH column density over the two XXL fields of 1.8 × 1020 cm−2 http://www.cfht.hawaii.edu/Science/CFHTLS/T0007
%quote from XXl Giles16: cluster spectra were extracted for each of the XMM cameras and fits were performed in the 0.4–7.0 keV band with an absorbed APEC (Smith et al. 2001) model (v2.0.2) with the absorbing column fixed at the Galactic value (Kalberla et al. 2005). 

\end{itemize}

%\setlength{\parindent}{0pt}
Differences include:

\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
\item[$\bullet$] The input \xmm{} observations. Our analysis includes some \xmm{} observations that entered the archive after the publication of \cite{xxllt}. 
%In total {\color{red}\xxlobsids} were used.
\item[$\bullet$] 
The approach to background subtraction for the global spectral analyses.  We used a local, in field, subtraction technique with an annulus of width $1.05-1.5R_{500}$ centered on the UDC$^{\ref{foot:udc}}$. By comparison, \citet[][]{xxllt}, used either: {\em (i)} an annulus centered on the aimpoint of the {\em XMM} observation, with a width determined by the diameter of the analysis region of the galaxy cluster \citep[see Figure~1 of][]{xxllt}; or {\em (ii)} an annulus centered on the cluster centroid with an inner radius equal to the extent of the cluster emission and an outer radius a factor 2$\times$ the inner radius.  
\item[$\bullet$] The approach to background subtraction used during the generation of surface brightness (and thus emission measure) profiles. Whereas we used a simple technique (see above), \cite{{xxlbaryon}} used a model for the non-X-ray background and a spatial fit for the X-ray background (see section 2.2 and 2.3 in \cite{{xxlbaryon}} for more detail).
\item[$\bullet$] The choice of manually adjusted source masks and excluded \xmm{} 
observations (Section~\ref{subsec:manualdetreg}).
\item[$\bullet$] Different versions of certain software packages.  
\citet[][]{gc100} used SAS v10.0.2, whereas we use SAS v18.0.0. \cite{xxllt} used \xspec{} v12.8.1i, whereas we use v12.11.0.
\item[$\bullet$] 
%\item[$\bullet$] The \xmm{} data reduction, image generation, and source detection. Whereas herein we followed the methods described in G22, the XXL results are based on methods presented in \citet[][]{gc100}.
The pipelines used to generate the various analysis products required to obtain $T_{\rm X}$ and $M_{\rm gas}(<r)$ estimates. Herein, we use \xga{} (Section~\ref{sec:methodology}), which differs in several ways to those used in \cite{gc100}, \cite{xxllt}, and/or \cite{xxlbaryon}.

\end{itemize}

\subsubsection{LoCuSS High-$L_{\rm{X}}$}
\label{subsubsec:LoCuSSsim}

%from Hydro paper:
% Surface brightness profiles are computed from soft energy ([0.5–2.5 keV]) photon images, corrected for background and effective area. The surface brightness profile is extracted in concentric annuli centred on the centroid of the cluster. The maximum radius is set to r500, which is estimated using the r–Yx scaling relation, if the field of view permits. The minimum radius is chosen to exclude the cool cores or internal regions with evidence of isophotal asymmetry, likely due to merger events.

%\footnote{The other 5 LoCuSS High-$L_{\rm{X}}$ clusters have been observed by \chandra{}, but have not yet been observed by \xmm{}.}

%\footnote{A further \extraLOCUSSTx{} \xmm{} based values were extracted by our \xga{} analysis, and can be found in Table~\ref{tab:locussmeasurements}. However, for these \extraLOCUSSTx{} clusters, only \chandra{} values were available in \cite{locusstemps} and \cite{locusshydro}, so they are not included in the comparison presented in Figure~\ref{fig:locusstxcomp}.}

We have used \xga{} to analyse the 50 LoCuSS clusters {\color{red}(see Table~\ref{app:locussresults})} presented in \cite{locusshydro}. For \LOCUSSTxvaluesorginal{} clusters, \cite{locusshydro} provide gas and hydrostatic masses as determined using only {\em XMM} observations.  These clusters form the first LoCuSS validation sample, referred to as LoCuSS High-$L_{\rm{X}}$ (a).  A modified version of the LoCuSS sample selection is given in \cite{locusstemps}, containing 41 clusters (see Table~\ref{app:locussresults}).  Of these, 32 clusters were analysed using only {\em XMM} observations\footnote{The data tables in \cite{locusstemps} did not specific which values were derived from {\em XMM} or {\em Chandra}. This information was provided by G. Smith, priv. comm.} to provide global temperature measurements. These clusters form the second LoCuSS validation sample, referred to as LoCuSS High-$L_{\rm{X}}$ (b). We note that we do not measure any results for `RXCJ1212.3-1816', as its sole \xmm{} observation (0652010201) was excluded during the inspection detailed in Section~\ref{subsec:manualdetreg} due to residual flaring. 
Our analysis of the LoCuSS High-$L_{\rm{X}}$ clusters included these elements in common with the published works:

\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
\item[$\bullet$]  The cosmological model: $\Omega_{\Lambda}$=0.7, and $\rm{H}_{0}$=70 km s$^{-1}$ Mpc$^{-1}$.  
%\item -energy band
\item[$\bullet$] 
The UDCs$^{\ref{foot:udc}}$ (i.e. choice of cluster centroid locations) and redshifts values were taken from \cite{locusshydro}. To compare global temperatures, we used the R$_{500}$ values given in \cite{locusstemps}.  To compare gas and hydrostatic masses, we used the R$_{500}$ values given in \cite{locusshydro}. Therefore, the source apertures were the same (i.e. size, shape, and location) in the relevant aspects (global spectral fits, \S\ref{subsec:xgaspecs}) of both analyses.
\item[$\bullet$] The model used during the \xspec{} fits was the same. Both analyses used an absorbed APEC plasma model with the column density and redshift fixed during the fit. The metallicity is left free to vary.  One small difference is that \cite{locusshydro} uses the {\tt wabs} model (rather than {\tt tbabs}) to account for absorption. 
\item We perform \xspec{} fits within an energy range of 0.7-10.0~keV.
%\item[$\bullet$] Metallicity is left free to vary during \xspec{} fits. 
\item [$\bullet$] Surface brightness profiles were derived from images generated in the 0.5–2.5~keV energy band.
\item [$\bullet$] Temperature profiles were constructed with a minimum number of background subtracted counts per annulus of 3000.
%comment: : mention core excised KR
\item [$\bullet$] Global temperature values were measured from core-excised (0.15-1$R_{500}$) spectra.
\item Errors on the gas masses do not include overdensity radius uncertainties (see Sect.~\ref{subsec:measgasmass}) as \cite{locusshydro} did not use this approach in their analysis.

\end{itemize}

%\setlength{\parindent}{0pt}
Differences include:

\begin{itemize}[leftmargin=*, labelindent=2pt, itemsep=1ex]
\item[$\bullet$] The input \xmm{} observations. Our analysis includes \xmm{} observations that entered the archive after the publication of \cite{locusshydro}. 
%In total \locussobsids{} were used.
%comment: mention this produces extra Tx's; KR
%\item[$\bullet$] The model used during the \xspec{} fits. Whereas \xga{} used used an absorbed APEC plasma model with the column density, redshift, and metal abundance fixed during the fit, \cite{locusshydro} use older models (\texttt{wabs} and \texttt{mekal}) \textcolor{red}{NEED TO CHECK, MARTINO STATE MEKAL for ACIS-S but APEC for ACIS-I AND XMM?}. %Though we have found that temperature and luminosity results are consistent with \texttt{tbabs*apec}.
%\item[$\bullet$] \cite{locusshydro} used \cite{locussnh} nH measurements, \xga{} uses \cite{nh} values; they have been shown to be consistent$^\ref{footnote:nh}$.
% \item[$\bullet$] The \cite{locusshydro} analysis left nH and $Z$ free in XSPEC fits. In our reanalysis using \xga{}, we keep them fixed. 
\item[$\bullet$] The choice of manually adjusted source masks and excluded \xmm{} 
observations (Section~\ref{subsec:manualdetreg}).
\item[$\bullet$]  The approach to background subtraction. Whereas we used a simple, in field, subtraction technique with an annulus of width $1.05-1.5R_{500}$ (1.05-1.5~$\theta_{\rm{outer}}'$) centered on the UDC$^{\ref{foot:udc}}$, for the global spectral and surface brightness (radial spectral) analyses, \citet[][]{locusshydro}, used a spectral modeling approach (see section 3.3.1 and 3.3.3 in \cite{{locusshydro}} for more detail). We note that specific information regarding the background subtraction methods used to derive the global $T_{\rm X}$ values provided in \cite{locusstemps} is not given, but we assume the same (spectral modelling) approach was used.
\item[$\bullet$] Different versions of certain software packages; the \cite{locusshydro} work uses SAS v11.0.0, we use SAS v18.0.0. It is not stated which version of \xspec{} was used by \cite{locusshydro}, but it will be a considerably older version than we use (v12.11.0).
\item[$\bullet$]  The pipelines used to generate the various analysis products required to obtain $T_{\rm X}$, $M_{\rm gas}(<r)$, $M_{\rm hydro}(<r)$ estimates. Herein, we use \xga{} (Section~\ref{sec:methodology}), which differs in several ways to those used in \cite{locusshydro}.
\item[$\bullet$] The equations to model the density and 3D temperature profiles differ between those used in this work {\color{red}(Equ.** and Equ.** for density and temperature respectively)} and the form used in \citet[][see their Equ. 4 and 5 for density and temperature respectively]{locusshydro}.
\end{itemize}



\subsection{Validation of derived properties}

\begin{table}           
\begin{center}
\caption[]{{\small Best fit parameters of fixed-slope models fit to comparisons between original published properties of our galaxy clusters, and the \xga{} derived properties. The first column indicates the property compared, the second the particular sample (either SDSSRM-XCS, XXL, or LoCuSS High-\lx{}), the third gives the value and uncertainty of the normalisation parameter of the fit, the fourth gives the value and uncertainty of the scatter of the fit, and the last column links to the relevant figure.}\label{tab:compfit}}
\vspace{1mm}
\begin{tabular}{ccccc}
\hline
\hline
 Comparison & Sample & Norm & Scatter & Figure \\
 & & $A$ & $\sigma$ & \\ \hline
\hline
\vspace{1mm}
$T_{\rm{X}}^{2500}$ & SDSSRM-XCS & 0.99$\pm$0.00 & 0.02$\pm$0.00 & \ref{fig:xcstempcomp}(a) \\
\vspace{1mm}
$T_{\rm{X}}^{500}$ & SDSSRM-XCS & 1.00$\pm$0.01 & 0.04$\pm$0.01 & \ref{fig:xcstempcomp}(b) \\
\vspace{1mm}
$T_{\rm{X}}^{\rm 300kpc}$ & XXL-100-GC & 0.99$\pm$0.01 & 0.04$\pm$0.01 & \ref{fig:xxltxcomp} \\
\vspace{1mm}
$T_{\rm{X}}^{\rm 500ce}$ & LoCuSS High-\lx{} & 1.01$\pm$0.01 & 0.04$\pm$0.01 & \ref{fig:locusstxcomp} \\

\hline
\vspace{1mm}
$M_{\rm{gas}}^{500}$ & XXL-100-GC & 0.89$\pm$0.06 & 0.59$\pm$0.05 & \ref{fig:compxxlgm} \\
\vspace{1mm}
$M_{\rm{gas}}^{2500}$ & LoCuSS High-\lx{} & 0.97$\pm$0.02 & 0.08$\pm$0.01 & \ref{fig:complocussgm}(a) \\
\vspace{1mm}
$M_{\rm{gas}}^{500}$ & LoCuSS High-\lx{} & 0.93$\pm$0.02 & 0.13$\pm$0.02 & \ref{fig:complocussgm}(b) \\
\hline
\vspace{1mm}
$M_{\rm{hy}}^{2500}$ & LoCuSS High-\lx{} & 1.10$\pm$0.03 & 0.08$\pm$0.03 & \ref{fig:complocusshym}(b) \\
$M_{\rm{hy}}^{500}$ & LoCuSS High-\lx{} & 1.19$\pm$0.07 & 0.24$\pm$0.05 & \ref{fig:complocusshym}(b) \\
\hline
\end{tabular}
\end{center}
\end{table}


The validation of the derived properties takes the form of 1:1 comparisons to the validation sample described above, and are quantified by fitting a power-law with the slope fixed at unity. The fits were performed in log space using the R package LInear Regression in Astronomy\citep[{\sc lira}\footnote{\href{https://cran.r-project.org/web/packages/lira/index.html}{LInear Regression in Astronomy}}, ][]{softlira}, fully described in \cite{LIRA}. The validations are visualised via 1:1 plots for each property compared, and in each case the best-fit is given by a lightblue solid line and the 68\% confidence interval by the lightblue shaded region.  The 1, 2 and 3-$\sigma$ intrinsic scatter is given by the grey shaded regions.  A summary of fit results can be found in Table~\ref{tab:compfit}. In the following sections we discuss the comparisons of each property for each sample in more detail.  The results can be reproduced using public \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/sdss_comparisons.ipynb}{Jupyter notebooks}


\subsubsection{Validation of \xga{} derived global $T_{\rm X}$ values}
\label{subsubsec:txtests}


%number returned (why some missing or added)
%comparison of best fit values
%comparison of errors

%KR: add something about the adaptability of XGA

\textbf{SDSSRM-XCS:}
%\label{subsubsec:xcs3ptx}
The temperature comparison is shown in Figure~\ref{fig:xcstempcomp} for both the $R_{2500}$ (a) and $R_{500}$ (b) apertures.  The best-fit normalisations are 0.99$\pm$0.00 and 1.00$\pm$0.01 for T$_{\rm X}^{500}$ and T$_{\rm X}^{2500}$ respectively.  This highlights that the \xga{} and G22 values are in excellent agreement. This is expected, given the similarities in the input data and the methodology.
There is some small amount of scatter around the 1:1 relation, which can be attributed to the small differences in the method (see Section~\ref{subsubsec:SDSSRMsim}). 
%These results can be reproduced using the linked public \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/sdss_comparisons.ipynb}{Jupyter notebook}. 
%comment: we should do a comparison of the errors as well as of the values |  mention that XGA delivered results for the whole sample KR
%There are a small number of significant outliers. These have been investigated 
%%comment: have they?
%and can be explained by different decisions made during the eyeball step (Section ??). 

%{\color{red} GRABBED THIS FROM MY THESIS - CAN PARE IT DOWN AND MAYBE WOULD BE GOOD FOR THIS -
%It is interesting to note that, for three of the four high-\xga{}-luminosity outliers in Figure~\ref{fig:xcstemplumcomp}b, the \xga{} results reduce the scatter of luminosity with temperature compared to the original XCS results. This may indicate that these re-analysis measurements are more consistent with the actual physical properties of the clusters. The fourth high-luminosity outlier does not exhibit the same dramatic improvement in consistency with the luminosity-temperature relation, as it was already a low scatter point. This fourth cluster in particular is right on the edge of the field-of-view, making reliable measurements of properties more challenging. All four of these luminosity outliers correspond to temperature outliers in Figure~\ref{fig:xcstemplumcomp}a, as their constrained temperatures are also different to the original XCS measurements.}


\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/temp_comp_xcs_xga_slope_fix.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/temp_comp_xcs_xga_slope_fix_r2500.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Tx SDSSRM]{The \xga{} APEC temperatures versus the \texttt{XCS3P} 
    APEC temperatures within $R_{500}$ (a) and $R_{2500}$ (b) for the SDSSRM-XCS sample \citep[as taken from][]{xcsgiles}.  The red dashed line represents the 1:1 relation. }
    \label{fig:xcstempcomp}
\end{figure*}

%Published measurements were made using the \texttt{XCS3P} pipeline \citep[fully described in][]{xcsmethod, xcsgiles} that measures properties within the overdensity radii, found through an iterative process.  An initial temperature and luminosity are measured within the \xapa{} defined source radius, then uses the temperature to estimate R$_{500}$ (or R$_{2500}$) using the $R_{\Delta}-T_{\rm{X}}$ relation of \cite{arnaudmt}, and repeats until the radius converges.
%comment: does XGA do this iteration? KR
%To account for the background, local background annuli were constructed between 1.05-1.5$R_{500}$ or between 2-3$R_{2500}$.  \xga{} does not re-use any code from \texttt{XCS3P}, but the \xga{} analysis matches as close as possible that performed in \cite{xcsgiles} (e.g., the same source and background regions).



\noindent \textbf{XXL-100-GC:}
%\label{subsubsec:xxltx}
The \xga{} analysis yielded T$_{\rm X}^{\rm 300kpc}$ values for \XXLTxvalues{} of the 99 clusters in the input sample. The temperature comparison is shown in Figure~\ref{fig:xxltxcomp}.
%These results can be reproduced using the linked public \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/xxl_comparisons.ipynb}{Jupyter notebook}. 
The best-fit normalisation of 0.99$\pm$0.01 shows that the \xga{} and \cite{xxllt} values are in excellent agreement, despite the large number of differences between the two approaches (see Section~\ref{subsubsec:XXLsim}).
%With regard to the three XXL clusters that \xga{} failed to measure global $T_{\rm X}$ values for: In two cases (XLSSC-61 and XLSSC-527), the data did not pass the \xga{} cleaning step (whereby at least 70\% of the analysis region must be present on an observation, see Section \S~\ref{subsec:xcsdata}).  In the case of XLSSC-11, the cluster is too extended ($z=0.054$) for the \xga{} background aperture to fit in the XMM field of view.
%comment: correct? if so, say what z was KR




\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images/temp_comp_xxl_xga_slope_fix.pdf}
    \caption[T comp XXL]{A comparison of global X-ray temperature values measured by \xga{} and XXL analyses \citep[as taken from][]{xxllt}, for the XXL-100-GC sample (see Section~\ref{subsubsec:txtests} for details).  The 1:1 relation is highlighted by the red dashed line.
    %comment: task: remove the Lx figure
    % b) shows the equivalent for the 0.5-2.0keV luminosity measurements.
    }
    \label{fig:xxltxcomp}
\end{figure}

\noindent \textbf{LoCuSS High-$\pmb{L_{\rm{X}}}$}:
%\label{subsubsec:locusstx}
The \xga{} analysis yielded global, core-excised, temperatures values for all 32
of the input sample with \xmm{} results in \cite{locusstemps}. The temperature comparison is shown in Figure~\ref{fig:locusstxcomp}.  The best-fit normalisation is 1.01$\pm$0.01, showing that the \xga{} and \cite{locusstemps} values are in excellent agreement, despite the large number of differences between the two approaches (see Section~\ref{subsubsec:LoCuSSsim}).
%All 45 (\LOCUSSTxvaluesorginal+\extraLOCUSSTx) $T_{\rm X}$ values can be reproduced using the linked public \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/locuss_comparisons.ipynb}{Jupyter notebook}.




\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images/locuss_temp_comp_wl.pdf}
    \caption[T comp Locuss]{A comparison of global, core-excised, X-ray $R_{500}$ temperatures measured by \xga{} and LoCuSS analyses, for a subset of the LoCuSS High-$L_{\rm{X}}$ sample. The temperatures are measured within core excluded weak-lensing $R_{500}$ values (within [0.15-1]$R_{500}$), presented in \cite{locusstemps}.}
    \label{fig:locusstxcomp}
\end{figure} 



%The temperatures which we compare to for these clusters are core-excised (measured within 0.15-1R$_{500}$), 


% The cluster spectra are centered on RASS positions reported in \cite{locusshydro}.




%From the tests presented above, 
%(\S\ref{subsubsec:xcs3ptx}, \ref{subsubsec:xxltx}, \ref{subsubsec:locusstx})
%we can conclude that the \xga{} (almost\footnote{The data checks described in Section~\ref{subsec:manualdetreg} require human intervention.}) automated approach to extracting global cluster temperatures is robust. Occasional offsets ($\Delta T_{\rm X}>1 \sigma$) between \xga{} measured and previously published $T_{\rm X}$ values can be explained by the differing approaches taken during the analyses.
%could add more to say that we will look into individual clusters woth offsets in future work?
%The three sets of results can be reproduced using public \href{https://github.com/DavidT3/XCS-Mass-Paper-I-Analysis/blob/fe7c5ef9163d530a4f2d4e2124a01e2048f25999/notebooks/temp_lum_comparisons/sdss_comparisons.ipynb}{Jupyter notebooks}. 

\subsubsection{Validation of \xga{} derived $M_{\rm gas}$ values}
\label{subsec:compgasmasses}

The gas mass uncertainties presented for XXL-100-GC and LoCuSS High-\lx{} samples are derived from slightly different methods, as radius uncertainties are available for the XXL-100-GC sample, but not for the LoCuSS High-\lx{} sample. We discuss this in depth in Section~\ref{subsec:measgasmass}.

%From the tests presented below (\S\ref{subsubsec:xxlgasmass},\ref{subsubsec:locussgasmasses}), we can conclude that the \xga{} almost\footnotemark[\value{footnote}] automated approach to extracting gas masses delivers results similar to those in the literature. Where there are offsets, these are likely explained by the differing approaches taken during the analyses. In future work, we will further optimise the \xga{} method using mock observations of clusters extracted from hydrodynamic simulations extracted from hydrodynamic simulations \citep[such as e.g.,][]{300sims,milleniumTNGclusters}, i.e. where the ``true'' baryonic mass is known. This will also allow us to estimate the systematic errors introduced from simplifying assumptions, such as spherical symmetry and isothermality.


%comment: make sure the resolution of the SB profile, in pixels, is mentioned for each KR

%\newcommand{\XXLTxvalues}{99}
%\newcommand{\XXLgasmassvalues}{91}
%\newcommand{\LOCUSSTxvaluesorginal}{39}
%\newcommand{\LOCUSSgasmassvalues}{39}
%\newcommand{\extraLOCUSSTx}{6}

\noindent\textbf{XXL-100-GC:}
The \xga{} analysis yielded M$_{\rm gas}^{500}$ values for \XXLgasmassvalues{} (of the 99) clusters contained in the XXL-100-GC sample. 
%Each cluster's neutral hydrogen column density is used in the conversion factor calculation, as is its redshift, and we assume a metallicity of 0.3~$Z_{\odot}$. 
Figure~\ref{fig:compxxlgm} shows the comparison between \xga{} measured and gas mass estimates published in \cite{xxlbaryon}.  While the best-fit normalisation of 0.89$\pm$0.06 highlights the \xga{} values are $\sim$10\% lower than those measured by \cite{xxlbaryon}, the difference is $<$2$\sigma$. Therefore, there is broad agreement between the two analyses. This is encouraging considering the significant differences in density measurement between the two samples (see Section~\ref{subsubsec:XXLsim}). 

\noindent \textbf{LoCuSS High-$\pmb{L_{\rm{X}}}$}:
The \xga{} analysis yielded M$_{\rm gas}^{500}$ values for \LOCUSSgasmassvaluesxga{} (of \LOCUSSgasmassvaluesoriginal{}) LoCuSS High-$L_{\rm{X}}$ clusters.  Note that the one cluster missing (RXCJ1212) Comparisons of the gas masses calculated within R$_{2500}$ ($M_{\rm gas}^{2500}$) and R$_{500}$ ($M_{\rm gas}^{500}$) are presented in Figure~\ref{fig:complocussgm} (a) and (b) respectively.  The normalisations of the fits are 0.97$\pm$0.02 and 0.93$\pm$0.02 for $M_{\rm gas}^{2500}$ and $M_{\rm gas}^{500}$ respectively.  This highlights that the $M_{\rm gas}^{2500}$ values are consistent, however, the XGA measured $M_{\rm gas}^{500}$ values are on average 7\% lower than the LoCuSS values (significant at the 3.5$\sigma$ level).  

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images/xxl_mgas_comp.pdf}
    \caption[mgas comparison XXL]{A one-to-one comparison of gas masses measured for the XXL-100-GC cluster sample, within $R_{500}$, by \cite{xxlbaryon} and an \xga{} reanalysis. $S_B$ profiles were fitted with Beta profiles, density profiles with King profiles. Contains measurements for 91 of 96 XXL-100-GC clusters analysed with \xga{}.}
    \label{fig:compxxlgm}
\end{figure}

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/locuss_mgas_comp_r2500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/locuss_mgas_comp_r500.pdf} \\
    a) & b) \\
    \end{tabular}
    \caption[mgas comparison, locuss]{A one-to-one comparison of gas masses measured for the LoCuSS High-$L_{\rm{X}}$ cluster sample, within LoCuSS measured $R_{2500}$ (a) and $R_{500}$ (b) values, by \cite{locusshydro} and an \xga{} reanalysis.}
    \label{fig:complocussgm}
\end{figure*}

\subsubsection{Validation of \xga{} derived $M_{\rm hydro}$ values}
\label{subsec:mhydrocomp}
%comment:  make sure the minimum counts per spectral annulus is mentioned KR


%As a consistency check, we use \xga{} to measure hydrostatic masses for the LoCuSS High-$L_{\rm{X}}$ sample.

%mention that there aren't any other samples to test against (Lovasari?)

%To minimise differences with the original LoCuSS High-$L_{\rm{X}}$ hydrostatic mass analysis, we leave the metallicity of each annulus free to vary during the spectral fits.
%Density and temperature profiles are generated with an outer radius of $R_{500}$, fitted with models as described in Section~\ref{subsec:densityProf} and Section~\ref{subsec:gastempprof}. 
%Mass profiles are constructed (see Section~\ref{subsec:hydromassprof}) and used to measure hydrostatic masses within R$_{500}$ ($M^{\rm{hy}}_{500}$) and R$_{2500}$ ($M^{\rm{hy}}_{2500}$).  The background regions are taken from the 1.05-1.5$R_{\rm{outer}}$ annulus, where $R_{\rm{outer}}$ is the outer radius of the $N^{\rm{th}}$ annulus, which will likely be very slightly larger than $R_{500}$ (as described in Section~\ref{subsec:xgaspecs}, the outer radius must be an integer multiple of the minimum annulus width).

\textbf{LoCuSS High-$\pmb{L_{\rm{X}}}$}:
Figure~\ref{fig:complocusshym} shows a comparison between the \xga{} and LoCuSS hydrostatic masses for $M_{\rm{hy}}^{2500}$ (a) and $M_{\rm{hy}}^{500}$ (b). We successfully measure masses for \LOCUSShydromassvaluesxga{} galaxy clusters (of \LOCUSSTxvaluesorginal{}) in the LoCuSS High-$L_{\rm{X}}$ sample, \LOCUSShydromassvaluesoriginalxgaoverlap{} of which have \xmm{} hydrostatic masses measured by LoCuSS (which are compared in Fig.~\ref{fig:complocusshym}). When compared to the LoCuSS masses (specifically those measured by \xmm{}), we find \xga{} measured masses 10\% and 19\% higher than LoCuSS for $M_{\rm{hy}}^{2500}$ and $M_{\rm{hy}}^{500}$ respectively.  While the difference is significant at the 3.3$\sigma$ level for $M_{\rm{hy}}^{2500}$, the difference is $<$3$\sigma$ for $M_{\rm{hy}}^{500}$.

%The agreement between the measured masses is not perfectly one-to-one; this is expected, since the number of components involved in measuring hydrostatic mass make it difficult to exactly match measurement methods between analyses (see Section~\ref{subsubsec:LoCuSSsim}). For example, \xga{} and LoCuSS take different approaches to measuring density profiles.  Furthermore, additional \xmm{} data is available for these clusters than there was at the time of the original \cite{locusshydro} analysis, which may have an effect on the constraints. 

%From the test presented above, we can conclude that the \xga{} (almost\footnote{The steps described in Sections~\ref{subsec:manualdetreg} and \ref{subsec:dataverif} do require human intervention.}) automated approach to extracting hydrostatic masses delivers results similar to those in the literature. Where there are offsets, these are likely explained by the differing approaches taken during the analyses. In future work, we will further optimise the \xga{} method using mock observations of clusters extracted from hydrodynamic simulations \citep[such as e.g.,][]{300sims,milleniumTNGclusters}, i.e. where the ``true'' halo mass is known. This will also allow us to estimate the systematic errors introduced from simplifying assumptions such as spherical symmetry.
%can we add any refs where hydro mass tests have been done on sims, e.g. https://arxiv.org/pdf/0912.1343.pdf



\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/locuss_mass_comp_r2500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/locuss_mass_comp_r500.pdf} \\
    a) & b) \\
    \end{tabular}
    \caption[hmass comparison]{A one-to-one comparison of hydrostatic masses measured for the LoCuSS High-$L_{\rm{X}}$ cluster sample, within LoCuSS measured $R_{2500}$ (a) and $R_{500}$ (b) values, by \cite{locusshydro} and an \xga{} reanalysis.}
    \label{fig:complocusshym}
\end{figure*}


%Many of the same caveats discussed in Section~\ref{subsubsec:locusslt} (where we presented \tx{} and \lx{} comparisons for an \xga{} reanalysis of LoCuSS High-$L_{\rm{X}}$ clusters) also apply to these mass measurements. We use slightly different models than LoCuSS for the \texttt{XSPEC} fitting process, though we have found results to be consistent between them. We also use a different XSPEC fitting method, in terms of how the spectra are tied together, and our approach to the background annulus is different. Finally, there is more \xmm{} data available for these clusters now than there was at the time of the original \cite{locusshydro} analysis, which may have an effect on the constraints.



%\subsection{scaling relation test}
%comment: not needed KR

%{\color{red} compare to Giles+ | this could be with same input data, to remove any inconsistencies with Tx's, Lx's}

\subsection{Discussion}

% Best-fit parameters of the cluster scaling relations (see $\S$\ref{sec:ltrelation} and $\S$\ref{sec:xray_richness} for details).  For each relation, parameters are given for the SDSSRM-XCS$_{T_{X},vol}$ ($T_{X,err}<25\%$ and 0.1$\le$z$\le$0.35) cluster sample.  Best-fit parameters are given for the $L_{X}-T_{X}$, $L_{X}-\lambda_{\rm RM}$ and $T_{X}-\lambda_{\rm RM}$ relations, given by equations~\ref{equ:lt},~\ref{equ:l-lambda} and~\ref{equ:t-lambda} respectively.

{\color{red} add some more commentary here (see list below)?}


From the tests presented above, 
%(\S\ref{subsubsec:xcs3ptx}, \ref{subsubsec:xxltx}, \ref{subsubsec:locusstx})
we can conclude that the \xga{} (almost\footnote{The data checks described in Section~\ref{subsec:manualdetreg} require human intervention.}) automated batch approaches to extracting estimates of $T_{\rm X}, M_{\rm gas}$ and $M_{\rm hydro}$ are robust, see Figures??-?? and Table ??. In only ?? (of ??) of the tests was the normalisation more than $3\sigma$ from unity. 
Where there are offsets, these are likely explained by the differing approaches taken during the analyses. In future work, we will further optimise the \xga{} method using mock observations of clusters extracted from hydrodynamic simulations \citep[such as e.g.,][]{300sims,milleniumTNGclusters}, i.e. where the ``true'' gas and halo masses are known. This will also allow us to estimate the systematic errors introduced from simplifying assumptions, such as spherical symmetry and isothermality. 

%say something about one or more of following...
%future improvements
%flexibility of XGA in terms of method and s;n variation (XXL vs LOCUSS)
% we have illustrated that we can easily analyse large samples of galaxy clusters with \xga{}.
% over wide range of Tx's and do core excision
%n Martino, they have a fiddle if there is not a T profile: When the low number of counts do not allow us to have a temperature profile with more than two annuli, we assume a constant profile with a = c = rt = 0 in the formula (5).

%stuff commented out from much earlier version, worth checking for useful snippets

%Summary information for these samples is presented in Table~\ref{tab:samplesummary}.  Comparisons of the distributions of the X-ray temperature ($T_{X}$), redshift and X-ray luminosity ($L_{X}$) for the samples are shown in Figures~\ref{fig:samp_sum}a), b) and c) respectively.  The temperature distribution shows the XXL-100-GC mostly contains clusters below 6~keV, the SDSSRM-XCS peaks at a similar temperature to XXL-100-GC but extends to higher temperatures, and the LoCuSS High-$L_{\rm{X}}$ sample contains higher temperature clusters (similar to the tail of the SDSSRM-XCS distribution) due to its selection from highly luminous systems.  The redshift distribution for the XXL-100-GC sample contains higher redshift clusters than the other samples, however, the SDSSRM-XCS and LoCuSS High-$L_{\rm{X}}$ samples includes redshift cuts, introducing artificial limits. Finally, the luminosity distributions highlights that the XXL-100-GC is similar to the lower end of the SDSSRM-XCS distribution, whereas the LoCuSS High-$L_{\rm{X}}$ sample is similar to the high luminosity tail of SDSSRM-XCS. 


% The full LoCuSS sample of 165 clusters was derived from the RASS catalogues by applying the cuts to various values; 0.15 < $z$ < 0.3, $n_{H}$ < $7\times 10^{20}\rm{cm}^{-2}$, and $-70^{\circ}$ < $\delta$ < $70^{\circ}$. The High-$L_{\rm{x}}$ sample was then selected from this larger sample by a harsher cut on the allowed declination values ($-25^{\circ}$ < $\delta$ < $65^{\circ}$), and a cut on the cluster luminosities measured within the $0.1-2.4$keV band ($L_{\rm{X}}$E($z$)$^{-2.7}$ $\geq$ $4.2\times10^{44}\rm{erg\:s^{-1}}$).
 

==> OldSections/ResultsSDSSsection4Augsut30.tex <==

%\section{New Masses and scaling relations}
\section{Mass analysis and scaling relations for the SDSSRM-XCS sample}
%comment:  It would be ironic, but have we inadvertently introduced some miscentering effect of our own by not re-measuring richness around the X-ray centre
\label{sec:results}
Here we present hydrostatic masses for a subset of galaxy clusters in the SDSSRM-XCS sample presented by \cite{xcsgiles}.  With these masses, we present a series of mass-observable relations.

\subsection{Masses for a subset of the SDSSRM-XCS sample}
\label{subsec:newmasses}

We attempt to measure masses for all 150 galaxy clusters in the SDSSRM-XCS sample.  Measurements presented in this section are performed using \xga{}, though we use $R_{500}$ values measured by G22. In Section~\ref{subsubsec:xcs3ptx} we demonstrated that the \xga{} \tx{} measurements are almost completely consistent with the original G22 analysis when measured within identical apertures. 

%We do not expect to be able to measure masses for all of these clusters, as measuring temperature profiles requires significant X-ray counts, but we shall attempt measurements using \xga{}'s automated routines. This will demonstrate its robustness and ability to deal with failed measurements.

Temperature and density profiles were generated out to $R_{500}$, where the $R_{500}$ used was measured by G22 using the radius-temperature relation of \cite{arnaudmt}. Density profiles were generated as described in Section~\ref{subsec:densityProf}. The temperature profile annuli are chosen so that each annuli has a minimum width of 20\arcsec and a minimum number of background subtracted counts per annulus of 1500. The minimum counts check is performed on the combined data for all relevant observations of a cluster. %\xga{} enforces a minimum of 4 annuli, so annuli with signal to noises lower than {\color{red}} are possible. 
%comment: Has all this not been said before? PG

We are able to successfully measure hydrostatic masses for \textcolor{red}{102} of the 150 galaxy clusters in the SDSSRM-XCS sample. The temperature profiles used for these measurements have between 4 (the minimum number allowed, see Section~\ref{subsec:xgaspecs}) 
and 26 annuli. We perform visual examination of relevant data products for each cluster, as described in Section~\ref{subsec:dataverif}. This process flags any suspect or blatantly nonphysical results, and allows us to perform a deeper inspection and determine why a particular result has been measured.

This set of hydrostatic masses adds significant value to the SDSSRM-XCS sample, as well as representing one of the largest samples of cluster hydrostatic masses available. As each mass is measured individually, rather than derived through the stacking of different clusters (as is usually the case for weak lensing cluster masses), there are many possible uses for the sample. Also, as SDSSRM-XCS clusters were selected from optical/NIR via the SDSS redMaPPer catalogue \citep[][]{redmappersdss}, this sample allows for powerful multi-wavelength studies of how cluster mass is related to optical properties.

{\color{red} we need to show the Mhydro results before doing scaling relations, e.g. a histogram? Ideally doing comparison to previous results, as per Giles Fig 8a. We should also do the comparisons to exisiting Hydro results for these clusters, as per Giles Fig 8b}

\textcolor{cyan}{How about we move 4.1 to the end of section 3, so that becomes Section 3.5, and then we add a section 3.5.1 which includes the comparisons to existing lit hydro masses?  Putting plot here for now}.

\subsubsection{Comparison of SDSSRM-XCS masses with the literature}
\label{sec:sdssrm_hydro_comp}

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/mass_histogram.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/sdssrm_mass_comp.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[mass comparison SDSSRM]{A one-to-one comparison of hydrostatic masses measured for the SDSSRM-XCS cluster sample using \xga{}, and values taken from the literature.}
    \label{fig:sdssrm_mass_comp}
\end{figure*}



\subsection{Construction of scaling relations}
\label{subsec:mors}

{\color{red} NOTE THAT COLOURS OF PLOTS ARE NOT NECESSARILY FINAL, ALSO I NEED TO SETTLE ON NORMALISING VALUES}

{\color{red} ALSO TITLES AND LEGENDS OF PLOTS MAY CHANGE}


{\color{red} KR added: for each relation subsection, we need a formula for the presentation:  figures, values, comparison to literature, implications e.g. for cosmo studies and/or hydro sims. Ordering is a bit random at the moment. Maybe split into Mgas relations and MHydro relations?}


{\color{red} KR added: I vote to drop the XGA plots in Section 4 and go with Paul's versions, since those have the scatter bands.}

We use the properties derived during the mass analysis process, namely the gas mass and total hydrostatic mass, for the SDSSRM-XCS sample to construct scaling relations between these properties and other X-ray and optical properties (e.g., the X-ray luminosity and temperature and the optical richness). These are compared to examples taken from literature. In all cases we perform the fits in log space using the R package LInear Regression in Astronomy\citep[{\sc lira}\footnote{\href{https://cran.r-project.org/web/packages/lira/index.html}{LInear Regression in Astronomy}},][]{softlira}, fully described in \cite{LIRA}.

Scaling relations are determined by fitting a power-law of the form, 

\begin{align}
Y = A + B\cdot Z \pm \epsilon
\label{morel}
\end{align}
where ${\rm var}(\epsilon)=\sigma^{2}_{Y|Z}$ and $Z$ is the intrinsic cluster property.  In the subsequent sections that follow, the scaling relations are simply denoted by the cluster properties in question and the scatter given by $\sigma$ (for example, see Equation~\ref{equ:mt}).  For each of the scaling relations presented, we consider relation with X-ray properties measured within two different overdensity radii, where $\Delta$=500 and 2500.  The relevant information for all our scaling relations is presented in Table~\ref{tab:scalingrelations}. 

\subsubsection{$M^{\rm{hy}}_{\rm{\Delta}}$-$T_{\rm{X,\Delta}}$ scaling relation}
\label{subsubsec:newMT}

Here, we present the scaling relation between hydrostatic mass and temperature ($M^{\rm{hy}}_{\rm{\Delta}}$-$T_{\rm{X,\Delta}}$). Figures~\ref{fig:mtsdssrm}(a) and (b) displays the $M^{\rm{hy}}_{\rm{\Delta}}$-$T_{\rm{X,\Delta}}$ for $\Delta$=500 and 2500 respectively.  A power law relation is fit to the data, which we express as:
\begin{align}
{\rm log}\left(\frac{M^{\rm hy}_{\Delta}}{E(z)^{y_{MT}}M_{0}}\right) &= {\rm log}(A_{MT}) + B_{MT}{\rm log}\left(\frac{T_{X,\Delta}}{T_{0}}\right) \pm \sigma_{M|T},
\label{equ:mt}
\end{align}
where $A_{MT}$ denotes the normalisation, $B_{MT}$ the slope, $y_{MT}$ the evolution with redshift and $\sigma_{L|T}$ the intrinsic scatter.  We assumed an $M_{0}$=\textcolor{red}{***} and $T_{0}$=\textcolor{red}{***}~keV and a self-similar evolution where $y_{MT}$=1.  The fit to the data is given by the cyan line, with the shaded region highlighting the 1$\sigma$ uncertainty.  Table~\ref{tab:scalingrelations} gives the best-fit value parameters of the relations.

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/sdssmt_r500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/sdssmt_r2500.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Mhydro T]{The hydrostatic mass to temperature relation constructed using masses measured from \sdssrmmasses{} clusters from the SDSSRM-XCS sample (black crosses). Masses and temperatures are measured within $R_{500}$ (a) and $R_{2500}$ (b).  In each case, the fits to the data (see Section~\ref{subsubsec:newMT}) are given by the cyan solid line, with the cyan shaded region representing the 1$\sigma$ uncertainty.}

    \label{fig:mtsdssrm}
\end{figure*}

\subsubsection{$M^{\rm{hy}}_{\rm{\Delta}}$-$M^{\rm gas}_{\Delta}$ scaling relation}
\label{subsubsec:newMg}

Here, we present the scaling relation between hydrostatic mass and gas mass ($M^{\rm{hy}}_{\rm{\Delta}}$-$M^{\rm gas}_{\Delta}$).  The $M^{\rm{hy}}_{\rm{\Delta}}$-$M^{\rm gas}_{\Delta}$ relation, measured for $\Delta$=500 and 2500, are given in Figure~\ref{fig:mgas_sdssrm}(a) and (b) respectively.  A power law relation is fit to the data, which we express as:
\begin{align}
{\rm log}\left(\frac{M^{\rm hy}_{\Delta}}{M_{0}}\right) &= {\rm log}(A_{MM_{g}}) + B_{MM_{g}}{\rm log}\left(\frac{M^{\rm gas}_{\Delta}}{M_{g,0}}\right) \pm \sigma_{M|M_{g}},
\label{equ:mmg}
\end{align}
where $M_{0}$=\textcolor{red}{***~M$_{\odot}$} and $M_{g,0}$=\textcolor{red}{***~M$_{\odot}$}.

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/sdssmhymg_r500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/sdssmhymg_r2500.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Mhydro T]{The hydrostatic mass to gas mass relation constructed using masses measured from \sdssrmmasses{} clusters from the SDSSRM-XCS sample (black crosses). Masses are measured within $R_{500}$ (a) and $R_{2500}$ (b).  In each case, the fits to the data (see Section~\ref{subsubsec:newMg}) are given by the cyan solid line, with the cyan shaded region representing the 1$\sigma$ uncertainty.}

    \label{fig:mgas_sdssrm}
\end{figure*}

\subsubsection{$L_{\rm{X,\Delta}}$-$M^{\rm{gas}}_{\rm{\Delta}}$ scaling relations}
\label{subsubsec:newMgasL}

We present here the scaling between $L_{\rm{X,\Delta}}$ and $M^{\rm{gas}}_{\rm{\Delta}}$.  It is expected that there should exist a strong correlation between these two quantities since they are both dependent on the electron density.  Previous literature studies of the $L_{\rm{X,\Delta}}$-$M^{\rm{gas}}_{\rm{\Delta}}$ relation have found a strong, low scatter, correlation \cite[e.g.,][]{hiflugcs_relations,WtG_mgas_lambda,efeds_scaling}.  The $L_{\rm{X,\Delta}}$-$M^{\rm{gas}}_{\rm{\Delta}}$ relation is plotted in Figure~\ref{fig:Lmgas_sdssrm}, for $\Delta$=500 (a) and $\Delta$=2500 (b).  The fit to the data is expressed as:
\begin{align}
{\rm log}\left(\frac{L_{X,\Delta}}{E(z)^{y_{LM_{g}}}L_{0}}\right) &= {\rm log}(A_{LM_{g}}) + B_{LM_{g}}{\rm log}\left(\frac{M^{\rm gas}_{\Delta}}{M_{g,0}}\right) \pm \sigma_{L|M},
\label{equ:lm}
\end{align}
where we assume $L_{0}$=\textcolor{red}{***~erg s$^{-1}$} and $M_{g,0}$=\textcolor{red}{***~M$_{\odot}$}.  We assume self-similar evolution where $y_{LM}=7/3$ when considering the bolometric luminosity and $y_{LM}=2$ when considering the 0.5-2.0~keV luminosity (\textcolor{red}{WHAT Lx BANDS ARE WE GOING TO USE?}).  We find a slope of the $\Delta$=500 soft-band relation of \textcolor{red}{$B_{LM_{g}}$=1.16$\pm$0.06}, which while steeper than the self-similar expectation (where we expect $L_{\rm{X,\Delta}}$ $\propto$ $M^{\rm{gas}}_{\rm{\Delta}}$), only represents a \textcolor{red}{2.6$\sigma$} deviation.  The slope of the relation when using bolometric luminosities (\textcolor{red}{1.31$\pm$0.06}) is entirely consistent with the self-similar expectation of 4/3. However, when we consider the $\Delta$=2500 relation, the slope of the soft-band relation, \textcolor{red}{$B_{LM_{g}}$=1.34$\pm$0.05}, represents a significant deviation from the self-similar expectation (at the 6.8$\sigma$ level).  The same is found for the $\Delta$=2500 bolometric luminosity relation, although the tension is reduced (at the 3.9$\sigma$ level).

When comparing our results to the literature, the slope of our relation is in good agreement with recent results from clusters detected in the eFEDS survey \textcolor{red}{CITED BEFORE?}.  \cite{efeds_scaling} found a slope of the soft-band  $L_{\rm{X,500}}$-$M^{\rm{gas}}_{500}$ relation of 1.07$\pm$0.02.  Note that the \cite{efeds_scaling} results are derived from {\em eROSITA} observation, and while \cite{efedsxcs} found that luminosities measured between {\em eROSITA} and {\em XMM} were in excellent agreement, no such comparisons of gas masses have been performed.  None-the-less, we highlight the comparison due to the lack of previous $L_{\rm{X,\Delta}}$-$M^{\rm{gas}}_{\rm{\Delta}}$ scaling studies. Our result is also consistent with \cite{hiflugcs_relations}, who used 62 clusters from the HIFLUGCS sample to investigate scaling relations.  Based upon the core-included $\Delta$=500 relations, they found a slope of 1.09$\pm$0.05.  However, when we compare the scatter of our relation to the literature, we find the intrinsic scatter of the relation is significantly different.  \cite{efeds_scaling} report a scatter of 0.30$\pm$0.02 and \cite{hiflugcs_relations} a value of 0.14$\pm$0.01, both of which are significantly less than our measured value of 0.57$\pm$0.04.  One potential reason for the increased scatter is the mix of targeted and serendipitously detected clusters in the SDSSRM sample \citep[see Section 5.1][for a discussion]{xcsgiles}.  \cite{xcsgiles} found that the scatter of the serendipitous clusters was less than the targeted clusters when considering relations involving X-ray luminosity.  \textcolor{red}{DO WE WANT TO GO FURTHER?}.

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/placeholder.jpg} &
    \includegraphics[width=1.0\columnwidth]{images/placeholder.jpg} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Mhydro T]{The luminosity to gas mass relation constructed using masses measured from \sdssrmmasses{} clusters from the SDSSRM-XCS sample (black crosses). Luminosities and gas masses are measured within $R_{500}$ (a) and $R_{2500}$ (b).  In each case, the fits to the data (see Section~\ref{subsubsec:newMgasL}) are given by the cyan solid line, with the cyan shaded region representing the 1$\sigma$ uncertainty.}

    \label{fig:Lmgas_sdssrm}
\end{figure*}

\subsubsection{$L_{\rm{X,\Delta}}$-$M^{\rm{hy}}_{\rm{\Delta}}$ scaling relations}
\label{subsubsec:newML}

The Luminosity-Mass ($L_{\rm{X,\Delta}}$-$M^{\rm{hy}}_{\rm{\Delta}}$) scaling relation is of great interest as it offers a way of estimating a clusters' mass from a simple X-ray observable.  This is of particular importance to the ongoing \erosita{} All-Sky Survey cosmology efforts since many more luminosity than temperature measurements will be acquired. Figure~\ref{fig:mlsdssrm} plots the $L_{\rm{X,\Delta}}$-$M^{\rm{hy}}_{\rm{\Delta}}$ scaling relations, for an overdesnity of $\Delta$=500 (Fig~\ref{fig:mlsdssrm}a) and 2500 (Fig~\ref{fig:mlsdssrm}b).  A fit to the data uses the same form as Equation~\ref{equ:lm}, but simply substituting $M^{\rm{gas}}_{\rm{\Delta}}$ with $M^{\rm hy}_{\rm{\Delta}}$ and $M_{g}$ with $M$.  We assume $L_{0}$=\textcolor{red}{***~erg s$^{-1}$} and $M_{0}$=\textcolor{red}{***~M$_{\odot}$}

We compare our relations to {\color{red}.... \erosita{} WL mass to L relation?, make one from Lovisari?}

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/sdsslm_r500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/sdsslm_r2500.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Mhydro L]{A luminosity to hydrostatic mass relation constructed using masses measured from \sdssrmmasses{} clusters from the SDSSRM-XCS sample. Masses and luminosities are measured within $R_{2500}$. Luminosities are unabsorbed and measured within the soft band (0.5-2.0~keV).}
    \label{fig:mlsdssrm}
\end{figure*}

\subsubsection{$M^{\rm{gas}}_{\rm{\Delta}}$-$\lambda$ scaling relation}
\label{subsubsec:newMgaslambda}

Here we focus on scaling relations involving the optical richness of the clusters.  Figures~\ref{fig:mgaslambdasdss}(a) and (b) gives the $M^{\rm{gas}}_{\rm{\Delta}}$-$\lambda$ scaling relation for $\Delta$=500 and 2500 respectively.

Literature constraints on the $M^{\rm{gas}}_{\rm{\Delta}}$-$\lambda$ relation are somewhat limited.  We compare to the relation presented in \cite{WtG_mgas_lambda}, who used a sample of \textcolor{red}{***} clusters from the Weighing the Giants cluster sample \citep{WtG_sample} to place constraints on the $M^{\rm{gas}}_{\rm{\Delta}}$-$\lambda$ relation.  While the gas masses calculated in \cite{WtG_mgas_lambda} were based upon {\em Chandra} observations, \cite{chandraxmmdensprofs} found that gas masses estimated from both {\em Chandra} and {\em XMM} were in good agreement. \cite{WtG_mgas_lambda} find a slope of 0.75$\pm$0.12 and a log-normal intrinsic scatter of 0.35$\pm$0.04.  

Next we construct a $M^{\rm{gas}}_{\rm{\Delta}}$-$\lambda$ relation from LoCuSS clusters using $M^{\rm{gas}}$ data from \cite{locusshydro} and richness data from \cite{locusstemps}.  Using 20 LoCuSS clusters with available data, we fit for the $M^{\rm{gas}}_{\rm{\Delta}}$-$\lambda$ relation as described in Section~\ref{subsec:mors}, finding a slope of 0.70$\pm$0.21 and a residual intrinsic scatter of 0.41$\pm$0.08.   

\subsubsection{$M^{\rm{hy}}_{\rm{\Delta}}$-$\lambda$ scaling relation}
\label{subsubsec:newMlambda}

Finally, we construct multi-wavelength scaling relations between hydrostatic mass and optical richness. Richness ($\lambda$) is a probabilistic measure of the number of galaxies in a galaxy cluster, and cannot be measured using X-ray observations. It is one of the outputs of the redMaPPer galaxy cluster finder, which was run on SDSS photometry \citep[][]{redmappersdss} and was used to construct the SDSSRM-XCS sample \citep[][]{xcsgiles}.

As in Section~\ref{subsubsec:newMgaslambda} above, comparisons to the literature are limited, with the majority of previous mass-richness relations using WL based masses \citep[e.g.,][]{WtG_mgas_lambda,2017MNRAS.466.3103S,desy1_wl_mor,locusstemps}. Our scaling relations are compared to {\color{red}... Bleem maybe? Or one constructed from the Lovisari sample}


\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/sdssgmr_r500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/sdssgmr_r2500.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Mhydro R]{A gas mass to richness relation constructed using masses measured from \sdssrmmasses{} clusters from the SDSSRM-XCS sample. Masses are measured within $R_{500}$. Richnesses are taken from the SDSS redMaPPer catalogue.}
    \label{fig:mgaslambdasdss}
\end{figure*}

\begin{figure*}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=1.0\columnwidth]{images/sdssmr_r500.pdf} &
    \includegraphics[width=1.0\columnwidth]{images/sdssmr_r2500.pdf} \\
    (a) & (b) \\
    \end{tabular}
    \caption[Mhydro R]{A hydrostatic mass to richness relation constructed using masses measured from \sdssrmmasses{} clusters from the SDSSRM-XCS sample. Masses are measured within $R_{500}$. Richnesses are taken from the SDSS redMaPPer catalogue.}
    \label{fig:masslambdasdss}
\end{figure*}

\begin{table}
\begin{center}
\caption[]{{The normalisation, slope, and residual scatter values for the mass-observable scaling relations measured using the new SDSSRM-XCS mass sample. Mass and observable normalisation values are also included.}\label{tab:scalingrelations}}
\vspace{1mm}
\begin{tabular}{lccccc}
\hline
\hline
Relation Name & $M_{0}$ & $O_{0}$ & $A_{MO}$ & $B_{MO}$ & $\sigma_{M|O}$\\
\hline
\hline
$E(z)M^{\rm{hy}}_{\rm{500}}$-\tx{}_{,500} & 0 & 0 & $0^{+0}_{-0}$ & $0^{+0}_{-0}$ & $0^{+0}_{-0}$\\
\hline 
$E(z)M^{\rm{hy}}_{\rm{2500}}$-\tx{}_{,2500} & 0 & 0 & $0^{+0}_{-0}$ & $0^{+0}_{-0}$ & $0^{+0}_{-0}$\\
\hline 
${\color{red}E(z)}M^{\rm{hy}}_{\rm{500}}$-$L^{\rm{0.5-2.0}}_{\rm{X,500}}$ & 0 & 0 & $0^{+0}_{-0}$ & $0^{+0}_{-0}$ & $0^{+0}_{-0}$\\
\hline 
${\color{red}E(z)}M^{\rm{hy}}_{\rm{2500}}$-$L^{\rm{0.5-2.0}}_{\rm{X,2500}}$ & 0 & 0 & $0^{+0}_{-0}$ & $0^{+0}_{-0}$ & $0^{+0}_{-0}$\\
\hline
${\color{red}E(z)}M^{\rm{hy}}_{\rm{500}}$-\lambda & 0 & 0 & $0^{+0}_{-0}$ & $0^{+0}_{-0}$ & $0^{+0}_{-0}$\\
\hline 
${\color{red}E(z)}M^{\rm{hy}}_{\rm{2500}}$-\lambda & 0 & 0 & $0^{+0}_{-0}$ & $0^{+0}_{-0}$ & $0^{+0}_{-0}$\\
\hline
\end{tabular}
\end{center}
\end{table}


==> OldSections/archive.tex <==
%\begin{figure*}
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/samps_prop_dists.pdf}
%    \caption[Sample Historgrams]{Histograms of properties of samples used in this work, taken from literature. X-ray properties presented in this figure have been measured in different regions, indicated in the legend of each plot. a) Intra-cluster medium average temperatures, b) cluster redshifts from spectroscopic follow-up (XXL-100-GC), from the RASS catalogues the sample was selected from (LoCuSS High-\lx{}), and from the redMaPPer cluster finder (SDSSRM-XCS), c) bolometric X-ray luminosities taken from literature, measured within $R_{500}$ (LoCuSS High-\lx{} and SDSSRM-XCS) and 300~kpc (XXL-100-GC).}
%   \label{fig:samp_sum}
%\end{figure*}

%{\em Chandra}'s smaller FoV and lower sensitivity make it a less effective instrument for probing hydrostatic masses, and though {\em eROSITA} has a very large FoV and similar sensitivity to {\em XMM}, its current use as a survey telescope precludes the possibility of gathering enough photons to determine temperature profiles. As such, while {\em eROSITA} is predicted to detect ${\sim}$100000 \citep[][]{erass_numclusters} galaxy clusters over the full eRASS survey, older X-ray telescopes (especially {\em XMM}) have an important part to play in the future of X-ray cluster mass measurements. Enough X-ray data exists in the telescope archives that we will be able to measure hundreds of masses at once, but a new, self-consistent, method is required.

%First, we measure projected temperature profiles by generating spectra in annuli centered on the cluster coordinates, then performing spectral fits to each annulus to determine a temperature. Previous XCS work \citep[][]{xcsmethod} has indicated that around 1000 counts are required to measure well constrained temperatures (with percentage uncertainties of 10-30\%, depending on the temperature of the cluster). That means that all annuli need to have that many counts to achieve a well constrained projected temperature profile. We make use of the method described in Section~\ref{subsec:annspec} to generate annular radii, centered on the supplied cluster coordinates, that have a minimum number of counts defined by the user (3000 for the LoCuSS analysis, 1500 for the SDSSRM-XCS analysis).
